FDFB: Full Domain Functional Bootstrapping Towards Practical Fully Homomorphic Encryption

Computation on ciphertexts of all known fully homomorphic encryption (FHE) schemes induces some noise, which, if too large, will destroy the plaintext. Therefore, the bootstrapping technique that re-encrypts a ciphertext and reduces the noise level remains the only known way of building FHE schemes for arbitrary unbounded computations. The bootstrapping step is also the major efficiency bottleneck in current FHE schemes. A promising direction towards improving concrete efficiency is to exploit the bootstrapping process to perform useful computation while reducing the noise at the same time. We show a bootstrapping algorithm, which embeds a lookup table and evaluates arbitrary functions of the plaintext while reducing the noise. Depending on the choice of parameters, the resulting homomorphic encryption scheme may be either an exact FHE or homomorphic encryption for approximate arithmetic. Since we can evaluate arbitrary functions over the plaintext space, we can use the natural homomorphism of Regev encryption to compute affine functions without bootstrapping almost for free. Consequently, our algorithms are particularly suitable for circuits with many additions and scalar multiplication gates. We achieve record speeds for such circuits. For example, in the exact FHE setting, we achieve a speedup of a factor of over 3000x over state-of-the-art methods. Effectively, we bring the evaluation time from weeks or days down to a few hours or minutes. Furthermore, we note that the speedup gets more significant with the size of the affine function. We provide a tight error analysis and show several parameter sets for our bootstrapping. Finally, we implement our algorithm and provide extensive tests. We demonstrate our algorithms by evaluating different neural networks in several parameter and accuracy settings.

==> sections/alternative-packing.tex <==



\begin{definition}[Key Switching LWE to GLWE]\label{def:packing-lwe-to-rlwe-ordinary}
We define the key generation algorithm $\KeySwitchSetup$ and  LWE to RLWE switching $\KeySwitch$ as follows.

\begin{description} 
\item[$\KeySwitchSetup(\bound_{\keySwitchKey}, n, n', \deg, q, \vec{s}, \vec{s}', \basis_{\keySwitchKey}):$]
Takes as input 
bound $\bound_{\keySwitchKey} \in \NN$, dimensions $n, n' \in \NN$, a degree $\deg \in \NN$ and
a modulus $q \in \NN$ that define $\R_{\deg, q}$,  vectors  $\vec{s} \in \ZZ_q^n$, $\vec{s}' \in \R_{\deg, q}^{n'}$ and a basis $\basis_{\keySwitchKey} \in \NN$.  
\begin{enumerate}
\item Set $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$. 
\item For $i \in [n]$,  $j \in [\ell_{\keySwitchKey}]$ set  
\begin{align*}
\keySwitchKey[i,j] \exec \GLWE_{\bound_{\keySwitchKey}, n', \deg, q}(\vec{s}', \vec{s}[i] \cdot \basis_{\keySwitchKey}^{j-1}).
\end{align*}

\item Output $\keySwitchKey \in \GLWE_{\bound_{\keySwitchKey}, n', \deg, q}(\vec{s}', .)^{n \times \ell_{\keySwitchKey}}$. 
\end{enumerate}

\item[$\KeySwitch(\vec{c}, \keySwitchKey):$]
Takes as input a LWE ciphertext $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \LWE_{\bound_{\vec{c}}, n, q}(\vec{s}, .)$
and a packing key $\keySwitchKey \in \GLWE_{\bound_{\keySwitchKey}, n', \deg, q}(\vec{s}', .)^{n \times \ell_{\keySwitchKey} \times \basis_{\keySwitchKey}}$.
\begin{enumerate}
\item Denote $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$.
%\item  Set $\fr{b}' \exec b \cdot X^{d - 1} \in \R_{\deg, q}$.   
\item Compute $\ma{A} \exec \Decomp_{\basis_{\keySwitchKey}, q}(\vec{a}) \in \R_{\basis_{\keySwitchKey}}^{n \times \ell_{\keySwitchKey}}$.    
\item Compute $c_{\out} \exec [\fr{b}, 0]^{\top} - \sum_{i=1}^n \sum_{j=1}^{\ell_{\keySwitchKey}} , \ma{A}[i,j] \cdot \keySwitchKey[i,j]$.  
\end{enumerate}
\end{description} 
 \end{definition}
 
  
 

 
 
 

==> sections/ap-blind-rotate.tex <==
 
 
 Here we recall the intuition behind the blind rotation algorithm of Alperin-Sheriff and Peikert \cite{C:AlpPei14}.
In short, the AP bootstrapping, uses a similar blind rotation procedure as FHEW, with the following exceptions.
Instead of having the $\brKey$ consisting of RGSW samples of $X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot (k - 1)}$,
it consists of a matrix of RGSW of bits representing a permutation which encoded 
$2^{i-1} \cdot \vec{s}[i]$. 
Then in blind rotation
instead of computing the external product on the accumulator with a RGSW sample of the $\brKey$,
we compute RGSW matrix multiplication, depending on the corresponding bits of the decomposed ciphertexts.
Note that the accumulator in this case is also an RGSW encrypted permutation matrix
representing the $b$ part of the ciphertext. We note that the permutation matrices, encode elements
$\ZZ_q$ by defining a shift on a vector, similarly to our shift based blind rotation scheme.


For completeness we will recall the permutation matrix encoding scheme, and briefly summarize the error.

\begin{definition}[Encryption of Permutation Matrices]
The scheme is defined as follows.
\begin{description}
\item[$\MatEnc(\fr{s}, \basis_{\RGSW}, \bound_{\MatEnc}, \ma{P}):$] 
On input a secret key $\fr{s} \in \R_{\deg, q}$, a basis $\basis_{\RGSW}$, a error distribution $\bound_{\MatEnc}$ and
a permutation matrix $\ma{P} \in \{0, 1\}^{p \times p}$, proceed as follows.
\begin{enumerate}
\item For all $i, j \in [p]$, set $\ma{C}_{\out}[i, j]\exec \RGSW_{\bound_{\MatEnc}, \deg, q, \basis_{\RGSW}}(\fr{s}, \ma{P}[i, j])$.
\item Return $\ma{C}_{\out}$.
\end{enumerate} 

\item[$\MatProd(\ma{C}_c, \ma{C}_d):$]
Takes as input $\ma{C}_c \in \RGSW_{\bound_{c}, \deg, q, \basis_{\RGSW}}(\fr{s}, \msg_c)^{p_1 \times p}$
and $\ma{C}_d \in \RGSW_{\bound_{d}, \deg, q, \basis_{\RGSW}}(\fr{s}, \msg_d)^{p \times p_2}$.
\begin{enumerate}
\item For all $i \in [p_1]$ set $\ma{C}_{\out}[i, j] \exec \sum_{j=1}^{p_2} \intProd(\ma{C}_c[i, j], \ma{C}_d[j, i])$.
\item Output $\ma{C}_{\out}$.
\end{enumerate}

\item[$\BlindRotate(\brKey, \vec{acc}, \ct):$]
The procedure takes as input a blind rotation key $\brKey \in \RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{p \times p \times n \times \ell_{\brKey} \times \basis_{\brKey}}$, and a vector $\vec{acc} \in \RLWE_{\bound_{\brKey}, \deg, Q}(\fr{s}, .)^{p}$, and a ciphertext $\ct \in \LWE_{\bound_{\ct}, n, q}$.
\begin{enumerate}
\item $\vec{c} \ModSwitch(\ct, q, p)$.
\item Let $\vec{c} \in [b, \vec{a}^\top]^\top \in \ZZ_p^{(n+1) \times 1}$.
\item Run $\ma{A} \exec \Decomp_{\basis_{\brKey}, q}(\vec{a}) \in \ZZ_q^{n \times \ell_{\brKey}}$.
\item For $i \in [n]$,
\begin{enumerate}
\item For $j \in [\ell_{\brKey}]$, compute $\vec{acc} \exec \MatProd(\ma{A}[i, j] \cdot \brKey[i, j], \vec{acc})$.
\end{enumerate}
\item Return $\vec{acc}$.
\end{enumerate}
\end{description}
\end{definition}

Note that in the above blind rotation we may actually use the internal product instead of the external product.
Furthermore, from correctness of the internal product, we have that the error induced by a single encrypted matrix multiplication 
is bounded by $\bound \leq \bound_d + p \cdot \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_c$,
where $\bound_d$ and $\bound_c$ are the error bounds on $\ma{C}_d$ and $\ma{C}_c$ respectively.
Hence, if we start blind rotation with an accumulator with error bounded by $\bound_{\vec{acc}}$,
then the error after blind rotation is $\bound_{\out} \leq \bound_{\acc}  + n \cdot \ell_{\brKey} \cdot p \cdot \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$. Finally, we note that the scheme requires   a
blind rotation key consisting of $n \cdot \ell_{\brKey} \cdot p^2$ RGSW samples and blind rotation requires 
$n \cdot \ell_{\brKey} \cdot p^2$
external products and $n \cdot \log_2{q} \cdot p^2$ additions of RLWE samples.

==> sections/bootstrapping-integers.tex <==
 
In this section, we show how to use the cyclic shifting of our packing technique to build an efficient functional bootstrapping algorithm.
 
\subsection{The Shift Based Blind Rotation Algorithm}
 
Now we are ready to define our blind rotation algorithm.
The main difference between our algorithm and the TFHE blind rotation algorithm is that we use our cyclic shift to update the accumulator. 
Therefore, we can evaluate arbitrary functions using our blind rotation, in contrast to only negacyclic functions, as it is the case for TFHE and FHEW style blind rotation.
 
\begin{definition}[Shifting Based Blind Rotation]
We define a the shifting based blind rotation $\BlindRotate_{\Shift}$ as follows.
\begin{description} 
\item[$\BRKeyGen_{\Shift}(n, \vec{s}, \vec{u}, \errDist_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s}):$]
 
Takes as input a dimension $n \in \NN$, a secret key $\vec{s} \in \ZZ_q^{n \times 1}$ and a vector $\vec{u} \in \ZZ^{u}$,
an error distribution $\errDist_{\brKey}$,
 a degree $\deg \in \NN$ and a modulus $Q$ defining the ring $\R_Q$, 
 a basis $\basis_{\RGSW} \in \NN$, and a secret key $\fr{s} \in \R_Q$.
 
\begin{enumerate}
\item  Set a matrix $\ma{Y} \in \BB^{n \times u}$ as follows:  
\begin{enumerate}
\item For $i \in [n]$ set the $i$-th row of $\ma{Y}$, to satisfy 
$\vec{s}[i] = \sum_{j=1}^{u} \ma{Y}[i, j] \cdot \vec{u}[j]$, 
\end{enumerate} 
\item For $i \in [n]$, $j \in [u]$ set $\brKey[i,j] = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, \ma{Y}[i,j])$. 
\item Output  $\brKey$. 
\end{enumerate}



\item[$\BlindRotate_{\Shift}(\brKey, \acc, \ct, \vec{u}, \packKey):$]
The algorithm takes as input a blind rotation key $\brKey = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{n \times u}$,  
  an accumulator $\acc \in \RLWE_{\errDist_{\acc}, \deg, Q}(\fr{s}, .)$, 
 a LWE sample $\ct = \in  \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)$,  a vector $\vec{u} \in \ZZ^{u}$, 
 a packing key $\packKey \in \RLWE_{\errDist_{\packKey}, \deg, Q}(\fr{s}, .)^{\deg \times \ell_{\packKey} \times \basis_{\packKey}}$.
\begin{enumerate}
\item $\vec{c} \exec \ModSwitch(\ct, q, \deg)$.
\item Let $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \ZZ_{\deg}^{(n+1) \times 1}$.
\item For $i \in [n]$ do: 
\begin{enumerate}
\item  For $j \in [u]$ do:
 \begin{align*}
 \acc \exec \CMux(\brKey[i, j], \Shift(\acc, - \vec{a} \cdot \vec{u}[j] \mod \deg), \acc)
\end{align*}   
\end{enumerate} 
\item Output $\acc$. 
\end{enumerate}
\end{description} 
\end{definition}

 
\begin{lemma}[Correctness of Shift-Based Blind Rotation]
\label{lemma:correctness-shift-based-blind-rotate}
Let  $\vec{u} \in \ZZ^u$ be a vector 
 that for all $y \in \ZZ_q$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod q$.
 Let  $\ct \in \LWE_{\errDist_{\bound_{\ct}}, n, q}(\vec{s}, .)$ to be a LWE sample and denote $\ct = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
Let   $\deg \in \NN$ be the degree and $Q \in \NN$ be the modulus defining the ring $\R_Q$.
Let $\fr{s} \in \R_Q$, $\basis_{\packKey} \in \NN$,  $\basis_{\RGSW} \in \NN$,  $\errDist_{\bound_{\brKey}}$ be a $\bound_{\brKey}$-Bounded distribution,
and $\acc \in \RLWE_{\errDist_{\bound_{\acc}}, \deg, Q}(\fr{s}, \msg_{\acc})$,
where $\errDist_{\bound_{\acc}}$ is a $\bound_{\acc}$-Bounded distribution.
Furthermore, let $\brKey \exec \BRKeyGen_{\Shift}(n, \vec{s}, \vec{u}, \errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}, \fr{s})$,
$\vec{s}' \exec \KeyExtract(\fr{s}) \in \ZZ_q^{\deg \times 1}$
and $\packKey \exec \PackSetup(\errDist_{\bound_{\packKey}},\deg, \deg, Q, \vec{s}', \fr{s}, \basis_{\packKey})$,
where $\errDist_{\bound_{\packKey}}$ is a $\bound_{\packKey}$-Bounded distribution.  
If $\acc_{\out} \exec \BlindRotate_{\Shift}(\brKey, \acc, \ct, \vec{u}, \packKey)$,
then $\acc_{\out} \in \RLWE_{\errDist_{\bound_{\out}}, \deg, Q}(\fr{s}, \msg_{\acc}^{\out})$,
where $\msg_{\acc}^{\out} = \Shift(\msg_{\acc}, - \vec{a}^{\top} \cdot \vec{s} \mod q) \in \R_Q$ and 
$\errDist_{\bound_{\out}}$ is a $\bound_{\out}$-Bounded distribution
with  
\begin{align*}
\bound_{\out} \leq \bound_{\acc} + n \cdot u \cdot (\deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}), 
\end{align*} 
where $\ell_{\RGSW} = \roundUp{\log_{\basis_{\RGSW}}{Q}}$ and $\ell_{\packKey} = \roundUp{\log_{\basis_{\packKey}}{Q}}$.
\end{lemma}




\begin{proof}[of lemma \ref{lemma:correctness-shift-based-blind-rotate} - Correctness of Shift-Based Blind Rotation]
The proof partially follows the reasoning of the proof of lemma \ref{lemma:correctness-tfhe-blind-rotate},
thus we will reuse some sentences from it. 
For brevity we will refer to calls of $\Shift$ omitting all parameters except
the polynomial to be shifted and the number of positions.
Let us first note that the blind rotation key $\brKey$ consists of RGSW samples of bits:
$\RGSW_{\errDist, \deg, Q, \basis_{\RGSW}}(\fr{s}, \ma{Y}[i,j])$, where $\ma{Y}[i,j] \in \BB$ for $i \in [n]$ 
and $j \in [u]$.
Denote the current accumulator as $\acc_{curr} \in \RLWE_{\errDist_{\bound_{\curr}}, \deg, Q}(\fr{s}, \msg_{\curr})$ for some $\msg_{\curr} \in \R_Q$.
If we increment 
$\acc_{\next} \exec \CMux(\brKey[i,j], \Shift(\acc_{\curr}, - \vec{a}[i] \cdot \vec{u}[j] \mod \deg), \acc_{\curr})$  
for some $i \in [n]$ and $j \in [u]$, then from correctness  
of the $\CMux$ gate
we have that $\acc_{\next} \in \RLWE_{\errDist_{\bound_{\next}}, \deg, Q}(\fr{s}, \msg_{\next})$,
where $\msg_{\next} = \Shift(\msg_{\curr}, d)$, where the number of shifts is
$d = -\vec{a}[i] \cdot \vec{u}[j] \cdot \ma{Y}[i, j] \mod \deg$. In other words, the next message
is shifted if $\ma{Y}[i,j] = 1$, or stays the same otherwise.
Let $\msg_{\out}$ be the message in the accumulator after the blind rotation loop (i.e. after $n \cdot u$ shifts).
Overall, we can represent the total output number of shifts $d_{\out}$ on the output message $\msg_{\out}$ as 
\begin{align*}
d_{\out} &=  \sum_{i=1}^n \sum_{j=1}^{u} -\vec{a}[i] \cdot \vec{u}[j] \cdot K[i, j] \mod \deg \\
 &= \sum_{i=1}^n -\vec{a}[i] \cdot \vec{s}[i] \mod \deg \\
 &=  -\vec{a}^{\top} \cdot \vec{s} \mod \deg.
\end{align*}
 
Furthermore, let $\errDist_{\bound_{\curr}}$ (resp. $\errDist_{\bound_{\next}}$) be a $\bound_{\curr}$-Bounded
(resp. $\bound_{\next}$-Bounded) distribution.
Let us also denote as $\bound_{\Shift, \curr}$ the
error bound on the shifted $\acc_{\curr}$.
From correctness of the $\Shift$ algorithm we have $\bound_{\Shift, \curr} \leq \bound_{\curr} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Then
from correctness of $\CMux$ we have $\bound_{\next}$ is given by
\begin{align*}
\bound_{\next} &\leq \max(\bound_{\curr}, \bound_{\Shift, \curr}) + \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey} \\
 &\leq    \bound_{\curr} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey} +   \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}
\end{align*}

Let us denote as $\bar{e} = \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey} +   \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$.
Then the error bound after $x$ iterations is given by the recursive function $T$ defined by
$T(0) = \bound_{\acc}$ and $T(x) = T(x-1) + \bar{e}$.
The explicit function for the formula is $T(x) = \bound_{\acc} + x \cdot \bar{e}$.
It is easy to verify the formula for $x=0$ and $x=1$.
Let us thus assume it holds from $x$, then
\begin{align*}
T(x+1) = \bound_{\acc} + (x + 1) \cdot \bar{e} = \bound_{\acc} + x \cdot \bar{e} + \bar{e} = T(x) + \bar{e}.
\end{align*}

To sum up, the error bound $\bound_{\out}$ after $n \cdot u$ iterations
satisfies
\begin{align*}
\bound_{\out} \leq \bound_{\acc} + n \cdot u \cdot (\deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}), 
\end{align*} 
  
\end{proof}


 
\subsection{Shift Based Bootstrapping}

 Below we describe the shift-based bootstrapping algorithm.
  
\begin{definition}[Shift-Based Bootstrapping]
\label{def:pre-rotation-bootstrapping}
The bootstrapping procedure is defined as follows:
\begin{description}
\item[$\BootstrapPreRot(\rKey, \ct, \preRotPoly):$]
Takes as input a bootstrapping key $\rKey$ which includes the blind rotation key $\brKey = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\brKey}}(\fr{s}, .)^{n \times u}$, 
a vector $\vec{u} \in \ZZ^{u}$,
a packing key $\packKey \in \RLWE_{\errDist_{\packKey}, \deg, Q}(\fr{s}, .)^{\deg \times \ell_{\packKey} \times \basis_{\packKey}}$,
 and a keyswitch key $\keySwitchKey \in \LWE_{\errDist_{\keySwitchKey}, n, q}(\vec{s}, .)^{\deg \times \ell_{\keySwitchKey}}$. 
The algorithm also takes as input a LWE sample $\ct = \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)(\msg) = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$,  
and a polynomial $\preRotPoly \in \R_Q$.

\begin{enumerate}
\item Set $\preRotPoly_b \exec \Shift(\preRotPoly, b)$.
\item Set $\acc \exec \RLWE_{\errDist_{\acc}, \deg, Q}(\fr{s}, 0) + [\preRotPoly_b, 0]^{\top}$.  
\item Run $\acc_{\BR} \exec \BlindRotate_{\Shift}(\brKey, \acc, \ct, \vec{u}, \packKey)$.   
\item Run $\vec{c}_{Q} \exec \SampleExtract(\acc_{\BR}, 1)$.
\item Run $\vec{c}_{q} \exec \ModSwitch(\vec{c}_Q, Q, q)$.
\item Run $\ct_{\out} \exec \KeySwitch(\vec{c}_q, \keySwitchKey)$.
\item Return $\ct_{\out}$.
\end{enumerate}
\end{description}
\end{definition}
  
 
 
\begin{theorem}[Correctness of the Bootstrapping]
\label{thm:bootstrapping-pre-rotation}
Let  $\vec{u} \in \ZZ^u$ be a vector 
 that for all $y \in \ZZ_q$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod q$.
 Let $\ct = \LWE_{\errDist_{\ct}, n, q}(\vec{s},\msg) = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
 Let $\deg, Q \in \NN$ and $\basis_{\RGSW}, \basis_{\brKey}, \basis_{\packKey}, \basis_{\keySwitchKey} \in \NN$.
 Let
 and $\fr{s} \in \R_q$ and $\vec{s}_{\fr{s}} \exec \KeyExtract(\fr{s})$.
 Let $\errDist_{\bound_{\brKey}}$, $\errDist_{\bound_{\packKey}}$ and $\errDist_{\bound_{\keySwitchKey}}$,
 be respectively $\bound_{\brKey}$, $\bound_{\packKey}$ and $\bound_{\keySwitchKey}$-Bounded distributions.
  Let
 $\brKey \exec \BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}, \fr{s})$, 
 $\packKey \exec \PackSetup(\errDist_{\bound_{\packKey}}, \deg, \deg, \allowbreak q, \vec{s}_{\fr{s}}, \fr{s}, \basis_{\packKey})$, 
 and  $\keySwitchKey \exec \KeySwitchSetup(\errDist_{\bound_{\keySwitchKey}}, \deg, \deg, q, \vec{s}_{\fr{s}}, \vec{s}, \basis_{\keySwitchKey})$.
 Finally, let $\preRotPoly \in \R_Q$ and $\rKey$ be the bootstrapping key which includes $\vec{u}$, $\brKey$,
 $\packKey$ and $\keySwitchKey$.
 
 If $\ct_{\out} \exec \BootstrapPreRot(\rKey, \ct, \preRotPoly)$, then
 $\ct_{\out} \in \LWE_{\errDist_{\bound}, \deg, q}(\vec{s}, \msg_{\out})$, where
 $\msg_{\out} = (\frac{q}{t}) \cdot \msg_{F}$ and $\msg_{F} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)))[1]$ for $Q = q = 0 \mod t$,
 and $\errDist_{\bound}$ is a $\bound$-Bounded distribution with
 \begin{align*} 
\bound \leq (\frac{q}{Q}) \cdot  \bound_{\BR}   + \bound_{\skDist} + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1),
\end{align*}
where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$, $\norm{\vec{s}}_2 \leq \bound_{\skDist}$
and  
 $\bound_{\BR}$ is the bound on RLWE accumulator after blind rotation according to lemma \ref{lemma:correctness-shift-based-blind-rotate}.
 Furthermore, we have that
 if $\bound \le  \frac{q}{2 \cdot t}$, then
 $\round{\Phase(\ct_{\out})}_t^q = \msg_{F}$.
\end{theorem}
 

\begin{proof}[of theorem \ref{thm:bootstrapping-pre-rotation} - Correctness of the Shift-Based Bootstrapping]
The correctness of the bootstrapping follows from the correctness of the underlying algorithms.
In particular, on the beginning we set the accumulator $\acc$ to the $\preRotPoly$ shifted by $b$.
From correctness of blind rotation we have 
$\acc_{\BR} \in \RLWE_{\bound_{\BR}}(\fr{s}, \msg_{\BR})$, where
$\msg_{\BR} = \Shift(\preRotPoly, \Phase(\ct)) \in \R_Q$
and $\errDist_{\bound_{\BR}}$ is a $\bound_{\BR}$-Bounded distribution
where the bound is given by lemma \ref{lemma:correctness-shift-based-blind-rotate}. 
Then from correctness of sample extract we have that $\vec{c}_Q \in \LWE_{\errDist_{\bound_{\BR}}, \deg, Q}(\vec{s}_{\fr{s}}, \msg_{\BR})$, where $\msg_{\vec{c}_Q} = \coefs(\msg_{\BR})[1]$.
From correctness of modulus switching we have that 
$\vec{c}_q \in \LWE_{\errDist_{\bound_{\vec{c}_q}}, \deg, q}(\vec{s}_{\fr{s}}, (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q})$,
where $\errDist_{\bound_{\vec{c}_q}}$ is a $\bound_{\vec{c}_q}$-Bounded distribution
with $\bound_{\vec{c}_q} \leq (\frac{q}{Q}) \cdot   \bound_{\BR} + \bound_{\skDist}$.
From correctness of key switching
we have that $\ct_{\out} \in \LWE_{\errDist_{\bound}, \deg, q}(\vec{s}, \msg_{\out})$,
where $\msg_{\out} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q}$ and
 $\errDist_{\bound}$ is a $\bound$-Bounded distribution
with 
\begin{align*}
\bound &\leq \bound_{\vec{c}_q} + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) \\
 &\leq (\frac{q}{Q})   \cdot  \bound_{\BR}   + \skDist + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1),
\end{align*}
where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$. 

Finally, denote $\msg_{\vec{c}_Q} = (\frac{Q}{t}) \cdot \msg_{F}$, so that
$$\msg_{F} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)))[1].$$
Then we have 
$\msg_{\out} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q} = (\frac{q}{Q}) \cdot  (\frac{Q}{t}) \cdot \msg_{F} = (\frac{q}{t}) \cdot \msg_{F}$,
and if $\bound \le  \frac{q}{2\cdot t}$, then $\round{\Phase(\ct_{\out})}_t^q = \msg_{F} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)))[1]$.
\end{proof}




==> sections/correctness-for-packing.tex <==






\begin{proof}[of lemma \ref{lemma:correctness-lwe-to-rlwe-packing} - Correctness of LWE to RLWE Packing]
Note that the packing algorithm proceeds similarly as the keyswitch algorithm from LWE to LWE, with the exception 
that we represent
$\vec{c}$ as a polynomial of degree $X^{d-1}$ in $\R_q$.
For completeness we will mostly restate the proof for this case.

Let us first note that for all $i \in [n]$ we have 
\begin{align*}
\vec{c}_i &= \sum_{j=1}^{\ell_{\packKey}}  \packKey[i,j, \vec{A}[i,j]+1] \\
&= \sum_{j=1}^{\ell_{\packKey}}  \RLWE_{\bound_{\packKey}, \deg, q}(\fr{s}, \vec{s}[i] \cdot \basis_{\packKey}^{j-1} \cdot \vec{A}[i,j]) \\
&=  \RLWE_{\bound_{1}, \deg, q}(\fr{s}, \vec{a}'[i] \cdot \vec{s}[i]) \\
&= \RLWE_{\bound_{1}, \deg, q}(\fr{s}, \vec{a}[i] \cdot X^{d-1} \cdot \vec{s}[i])
\end{align*}
where $\bound_{1}$ is a $\bound_1$-Bounded distribution with 
$\bound_1 \leq \ell_{\packKey} \cdot \bound_{\packKey}$.
Then  note that
\begin{align*}
[\fr{b}'', \fr{a}'']^{\top} &= X^{d-1} \sum_{i=1}^{n} \vec{c}_i \\
 &= \sum_{i=1}^{n} \RLWE_{\bound_{1}, \deg, q}(\fr{s},  \vec{a}[i] \cdot X^{d-1} \cdot \vec{s}[i]) \\ 
 &=  \RLWE_{\bound_{2}, \deg, q}(\fr{s}, \sum_{i=1}^{n} \vec{a}[i] \cdot X^{d-1} \cdot \vec{s}[i])  \\
 &= \RLWE_{\bound_{2}, \deg, q}(\fr{s},  \vec{a}^{\top}  \cdot \vec{s}  \cdot X^{d-1}),
\end{align*}
where  
$\bound_{2} \leq n \cdot \bound_1 \leq n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Let us denote $\fr{b}' = X^{d-1} \cdot (\vec{a}^{\top} \cdot \vec{s} + \msg + e)$ and
$\fr{b}'' = \fr{a}'' \cdot \fr{s} + \vec{a}^{\top} \cdot \vec{s} \cdot X^{d-1} + \fr{e}''$,
then
\begin{align*}
\vec{c}_{\out} = [\fr{b}', 0]^{\top} - [\fr{b}'', \fr{a}'']^{\top} = [\fr{b}' - \fr{b}'', -\fr{a}'']^{\top} = [- \fr{a}'' \cdot \fr{s} + X^{d-1} \cdot \msg +  e \cdot X^{d - 1} - \fr{e}''].
\end{align*}
Hence, $\vec{c}_{\out}$ is a valid RLWE sample of $X^{d-1} \cdot \msg$ with respect to key $\fr{s}$ 
and $\norm{\Var(\Error(c))}_{\infty}   \leq \bound_{\vec{c}} + \bound_{2} \leq \bound_{\vec{c}} + n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
 
 For the ordinary packing algorithm given by Definition~\ref{def:packing-lwe-to-rlwe-ordinary}, 
the proof is analogous.
The only change is that in we multiply $\ma{A}[i,j] \cdot \packKey[i,j]$ instead of having
a packing key with the the $\ma{A}[i,j]$ multiple precomputed.
We assume that the entries of $\ma{A}$ are distributed uniformly in $[0, \basis_{\packKey}-1]$.
Therefore, the bound is 
$\bound \leq  \bound_{\vec{c}} + (\frac{7}{12}) \cdot n \cdot \ell_{\packKey} \cdot \basis_{\packKey}^2 \cdot  \bound_{\packKey}$. 
\end{proof}





\begin{proof}[of lemma \ref{lemma:correctness-of-vector-packing} - Correctness of Vector Packing]
For $i \in [m]$ us denote $\vec{v}[i] = [b_i, \vec{a}_i] \in \ZZ_q^{(n+1) \times 1}$,
where $b_i = \vec{a}_1^{\top}\cdot \vec{s} + \msg_i + e_i$, 
and let $\vec{d}[i] = [\fr{b}_i, \fr{a}_i]$.
Then from the the proof of lemma \ref{lemma:correctness-lwe-to-rlwe-packing}, we can write
$\fr{b}_i'' = \fr{a}_i'' \cdot \fr{s} + X^{i-1} \cdot \msg_i + \fr{e}_i'' + X^{i-1} \cdot e_i$,
for some $\fr{a}'' \in \R_q$ and $\fr{e}_i''$ from the packing key.
Note also that, as in the proof of lemma  \ref{lemma:correctness-lwe-to-rlwe-packing},
for all $i \in [m]$
we have  $\norm{\Var(\fr{e}_i'')}_{\infty} \leq \bound_{2} \leq n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Now we can denote
$
\ct_{\out} = \begin{bmatrix}
\fr{a}_{\out} \\
\fr{b}_{\out}
\end{bmatrix}
$
where $\fr{a}_{\out} = \sum_{i=1}^m$ and 
\begin{align*}
\fr{b}_{\out} = \sum_{i=1}^m \fr{b}_i'' = \fr{a}_{\out}^{\top} \cdot \fr{s} + \sum_{i=1}^m \msg_{i} \cdot X^{i-1} + \sum_{i=1}^m \fr{e}_i'' + \sum_{i=1}^{m} e_i \cdot X^{i-1}.
\end{align*}
Furthermore we have
that $\norm{\Var(\Error(\ct_{\out}))}_{\infty} = \norm{\Var(\sum_{i=1}^m \fr{e}_i'' + \sum_{i=1}^{m} e_i \cdot X^{i-1})}_{\infty} = \norm{\Var(\sum_{i=1}^m \fr{e}_i'')}_{\infty} + \norm{\Var(\sum_{i=1}^{m} e_i \cdot X^{i-1})}_{\infty} \leq \bound \leq m \cdot \bound_{2} + \bound_{\vec{v}} \leq \bound_{\vec{v}} + m \cdot n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$ for the precomputed packing version.

For the ordinary packing version the bound on the error is
$\bound \leq \bound_{\vec{v}} + (\frac{7}{12}) \cdot m \cdot n \cdot \ell_{\packKey} \cdot \basis_{\packKey}^2 \cdot \bound_{\packKey}$.
 

To conclude the proof we have that $\ct_{\out} \in \RLWE_{bound, \deg, q}(\msg_{\out})$, 
where $\msg_{\out} = \sum_{i=1}^m \msg_{i} \cdot X^{i-1}$. 
\end{proof}


 
%
%\begin{proof}[of lemma \ref{lemma:correctness-shift} - Correctness Shifting]
%Let us first start with the case $1 \leq d \leq \frac{\deg}{2}$.
%Let us denote
%$\ct = [\fr{b}, \fr{a}]^{\top} \in \R_q^2$, where $\fr{b} = \fr{a} \cdot \fr{s} + \sum_{i=1}^{\deg} \msg_i \cdot X^{i-1} + \sum_{i=1}^{\deg} e_{i} \cdot X^{i-1} \in \R_q$.
%Then, let us denote $\vec{c}_s = \ct \cdot X^d = [\fr{b}_s, \fr{a}_s] \in \R_q^2$,
%where $\fr{a}_s = \fr{a} \cdot X^d$ and 
%$\fr{b}_s = \fr{a}_s \cdot \fr{s} + \sum_{i=1}^{\deg} \msg_{i} \cdot X^{d + i-1} - \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} + \sum_{i=1}^{\deg} e_{i} \cdot X^{d + i - 1} - \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1}$.
%
%Let us also denote $\vec{c}_p = [\fr{b}_p, \fr{a}_p] \in \R_q^2$,
%where $\fr{b}_p = \fr{a}_p \cdot \fr{s} + \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1}  + \sum_{i=1}^{d} \fr{e}_{i}'' + \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1}$,
%where $\sum_{i=1}^{d} \fr{e}_i''$ is the error as in vector packing in the proof of lemma 
%\ref{lemma:correctness-of-vector-packing}. 
%Recall that  $\norm{\sum_{i=1}^{d} \fr{e}_i''}_2 \leq d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%
%Now let $\ct_{\out} = \vec{c}_s + 2 \cdot \vec{c}_p = [\fr{b}_{\out}, \fr{a}_{\out}] \in \R_q^2$.
%Then we have  $\fr{a}_{\out} = \fr{a}_s + 2 \cdot \fr{a}_p$
%and  
%$\fr{b}_{\out}  = \fr{a}_{\out} \cdot \fr{s} + \msg_{\out} + \fr{e}'' + \fr{e}_{\ct}$
%where $\fr{e}'' = 2 \cdot \sum_{i=1}^{d} \fr{e}_i''$,
%\begin{align*}
%\msg_{\out} &=  \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i-1} - \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} + 2 \cdot \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} \\
% &= \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i-1} + \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1},
%\end{align*}  
%and
%\begin{align*}
%\fr{e}_{\ct} &=  \sum_{i=1}^{\deg - d} e_{i} \cdot X^{d + i - 1} - \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1} + 2 \cdot \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1} \\
% &=  \sum_{i=1}^{\deg - d} e_{i} \cdot X^{d + i - 1} + \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1}
%\end{align*}
%Hence we have 
%$\norm{\fr{e}''}_2 \leq  2 \cdot d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$,
%$\norm{\fr{e}_{\ct}}_2 \leq \bound_{\ct}$.
%and,
%$\norm{\Error(\ct_{\out})}_2   \leq  \norm{\fr{e}_{\ct}}_2 + \norm{\fr{e}''}_2 \leq \bound_{\ct} + 2 \cdot d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%Since, in this case $d \leq \frac{\deg}{2}$, we have
%$\bound \leq \bound_{\ct} +   \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%
%Now we will turn to the case with $\frac{N}{2} \leq d \leq \deg$.
%In this case we have
%$\vec{c}_p = \vec{c}_p = [\fr{b}_p, \fr{a}_p] \in \R_q^2$,
%where $\fr{b}_p = \fr{a}_p \cdot \fr{s} + \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{i-1}  + \sum_{i=1}^{\deg - d} \fr{e}_{i}'' + \sum_{i=1}^{\deg - d} e_{i} \cdot X^{i-1}$.
%Let us denote 
%$\vec{c}_{\out} = [\fr{b}_{\out}, \fr{a}_{\out}]^{\top} = (2 \cdot \vec{c}_p + \ct) \cdot X^{d} \in \R_q^2$.
%Then $\fr{a}_{\out} = 2 \cdot (\fr{a}_p - \fr{a}_p) \cdot X^d \in \R_q$
%and
%$\fr{b}_{\out} = (2 \cdot \fr{b}_{p} + \fr{b}) \cdot X^d = \fr{a}_{\out} \cdot \fr{s} + \msg_{\out} + \fr{e}_{\out}$,
%where
%\begin{align*}
%\msg_{\out} &= (2 \cdot \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{i-1} -  \sum_{i=1}^{\deg} \msg_i \cdot X^{i-1}) \cdot X^d \\
% &= (2 \cdot \sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} - \sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} -
% \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{\deg - d + i} ) \cdot X^{d} \\
% &= (\sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} - \sum_{i=1}^d \msg_{\deg - d + i} \cdot X^{\deg - d + i} ) \cdot X^d \\
% &= \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i - i} + \sum_{i=1}^d \msg_{\deg - d + i} \cdot X^{i-1}
%\end{align*}
%and
%\begin{align*}
%\fr{e}_{\out} &= (2 \cdot (\sum_{i=1}^{\deg - d} \fr{e}_{i}'' + \sum_{i=1}^{\deg - d} e_{i} \cdot X^{i-1}) - \sum_{i=1}^{\deg} e_{i} \cdot X^{i-1}) \cdot X^d \\
% &= 2 \cdot X^d \cdot \sum_{i=1}^{\deg - d} \fr{e}_i'' + \sum_{i=1}^{\deg - d} e_i \cdot X^{d + i - 1} + \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1}.
%\end{align*}
%Hence, as earlier
%we have that 
%$\norm{\Error(\ct_{\out})}_2  \leq \bound_{\ct} + 2 \cdot (\deg - d) \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%Finally, since $\deg - d \leq \frac{\deg}{2}$,  we have
%$\bound \leq \bound_{\ct} +  \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
% 
%\end{proof}
%
%

 


 

==> sections/correctness-for-shift-blind-rotate.tex <==



\begin{proof}[of lemma \ref{lemma:correctness-shift-based-blind-rotate} - Correctness of Shift-Based Blind Rotation]
The proof partially follows the reasoning of the proof of lemma \ref{lemma:correctness-tfhe-blind-rotate},
thus we will reuse some sentences from it. 
For brevity we will refer to calls of $\Shift$ omitting all parameters except
the polynomial to be shifted and the number of positions.
Let us first note that the blind rotation key $\brKey$ consists of RGSW samples of bits:
$\RGSW_{\errDist, \deg, Q, \basis_{\RGSW}}(\fr{s}, \bf{Y}[i,j])$, where $\bf{Y}[i,j] \in \BB$ for $i \in [n]$ 
and $j \in [u]$.
Denote the current accumulator as $\acc_{curr} \in \RLWE_{\errDist_{\bound_{\curr}}, \deg, Q}(\fr{s}, \msg_{\curr})$ for some $\msg_{\curr} \in \R_Q$.
If we increment 
$\acc_{\next} \exec \CMux(\brKey[i,j], \Shift(\acc_{\curr}, - \vec{a}[i] \cdot \vec{u}[j] \mod \deg), \acc_{\curr})$  
for some $i \in [n]$ and $j \in [u]$, then from correctness  
of the $\CMux$ gate
we have that $\acc_{\next} \in \RLWE_{\errDist_{\bound_{\next}}, \deg, Q}(\fr{s}, \msg_{\next})$,
where $\msg_{\next} = \Shift(\msg_{\curr}, d)$, where the number of shifts is
$d = -\vec{a}[i] \cdot \vec{u}[j] \cdot \bf{Y}[i, j] \mod \deg$. In other words, the next message
is shifted if $\bf{Y}[i,j] = 1$, or stays the same otherwise.
Let $\msg_{\out}$ be the message in the accumulator after the blind rotation loop (i.e. after $n \cdot u$ shifts).
Overall, we can represent the total output number of shifts $d_{\out}$ on the output message $\msg_{\out}$ as 
\begin{align*}
d_{\out} &=  \sum_{i=1}^n \sum_{j=1}^{u} -\vec{a}[i] \cdot \vec{u}[j] \cdot K[i, j] \mod \deg \\
 &= \sum_{i=1}^n -\vec{a}[i] \cdot \vec{s}[i] \mod \deg \\
 &=  -\vec{a}^{\top} \cdot \vec{s} \mod \deg.
\end{align*}
 
Furthermore, let $\errDist_{\bound_{\curr}}$ (resp. $\errDist_{\bound_{\next}}$) be a $\bound_{\curr}$-Bounded
(resp. $\bound_{\next}$-Bounded) distribution.
Let us also denote as $\bound_{\Shift, \curr}$ the
error bound on the shifted $\acc_{\curr}$.
From correctness of the $\Shift$ algorithm we have $\bound_{\Shift, \curr} \leq \bound_{\curr} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Then
from correctness of $\CMux$ we have $\bound_{\next}$ is given by
\begin{align*}
\bound_{\next} &\leq \max(\bound_{\curr}, \bound_{\Shift, \curr}) + \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey} \\
 &\leq    \bound_{\curr} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey} +   \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}
\end{align*}

Let us denote as $\bar{e} = \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey} +   \deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$.
Then the error bound after $x$ iterations is given by the recursive function $T$ defined by
$T(0) = \bound_{\acc}$ and $T(x) = T(x-1) + \bar{e}$.
The explicit function for the formula is $T(x) = \bound_{\acc} + x \cdot \bar{e}$.
It is easy to verify the formula for $x=0$ and $x=1$.
Let us thus assume it holds from $x$, then
\begin{align*}
T(x+1) = \bound_{\acc} + (x + 1) \cdot \bar{e} = \bound_{\acc} + x \cdot \bar{e} + \bar{e} = T(x) + \bar{e}.
\end{align*}

To sum up, the error bound $\bound_{\out}$ after $n \cdot u$ iterations
satisfies
\begin{align*}
\bound_{\out} \leq \bound_{\acc} + n \cdot u \cdot (\deg \cdot \ell_{\RGSW} \cdot (\basis_{\RGSW} - 1) \cdot \bound_{\brKey} + \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}), 
\end{align*} 
  
\end{proof}



\begin{proof}[of theorem \ref{thm:bootstrapping-pre-rotation} - Correctness of the Shift-Based Bootstrapping]
The correctness of the bootstrapping follows from the correctness of the underlying algorithms.
In particular, on the beginning we set the accumulator $\acc$ to the $\preRotPoly$ shifted by $b$.
From correctness of blind rotation we have 
$\acc_{\BR} \in \RLWE_{\bound_{\BR}}(\fr{s}, \msg_{\BR})$, where
$\msg_{\BR} = \Shift(\preRotPoly, \Phase(\ct)) \in \R_Q$
and $\errDist_{\bound_{\BR}}$ is a $\bound_{\BR}$-Bounded distribution
where the bound is given by lemma \ref{lemma:correctness-shift-based-blind-rotate}.
%Then we compute $\vec{c} \exec \acc_{\BR} \cdot \postRotPoly$,
%so from linear homomorphism of RLWE samples we have  that
%$\vec{c} \in \RLWE_{\errDist_{\bound_{\vec{c}}}, \deg, Q}(\fr{s}, \msg_{\vec{c}})$,
%where $\msg_{\vec{c}} = \msg_{\BR} \cdot \postRotPoly \in \R_Q$, and
%$\errDist_{\bound_{\vec{c}}}$ is a $\bound_{\vec{c}}$-Bonded distribution with 
%$\bound_{\vec{c}} \leq \expFact_{\R_Q} \cdot  \bound_{\BR} \cdot \postRotPoly \leq \sqrt{\deg} \cdot  \bound_{\BR} \cdot \postRotPoly$.
Then from correctness of sample extract we have that $\vec{c}_Q \in \LWE_{\errDist_{\bound_{\BR}}, \deg, Q}(\vec{s}_{\fr{s}}, \msg_{\BR})$, where $\msg_{\vec{c}_Q} = \coefs(\msg_{\BR})[1]$.
From correctness of modulus switching we have that 
$\vec{c}_q \in \LWE_{\errDist_{\bound_{\vec{c}_q}}, \deg, q}(\vec{s}_{\fr{s}}, (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q})$,
where $\errDist_{\bound_{\vec{c}_q}}$ is a $\bound_{\vec{c}_q}$-Bounded distribution
with $\bound_{\vec{c}_q} \leq (\frac{q}{Q}) \cdot   \bound_{\BR}   + \bound_{\skDist}$.
From correctness of key switching
we have that $\ct_{\out} \in \LWE_{\errDist_{\bound}, \deg, q}(\vec{s}, \msg_{\out})$,
where $\msg_{\out} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q}$ and
 $\errDist_{\bound}$ is a $\bound$-Bounded distribution
with 
\begin{align*}
\bound &\leq \bound_{\vec{c}_q} + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) \\
 &\leq (\frac{q}{Q})   \cdot  \bound_{\BR}   + \skDist + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1),
\end{align*}
where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$. 

Finally, denote $\msg_{\vec{c}_Q} = (\frac{Q}{t}) \cdot \msg_{F}$, so that $\msg_{F} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)))[1]$.
Then we have 
$\msg_{\out} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_Q} = (\frac{q}{Q}) \cdot  (\frac{Q}{t}) \cdot \msg_{F} = (\frac{q}{t}) \cdot \msg_{F}$.
What follows is that if $\bound \le  \frac{q}{2\cdot t}$, then $\round{\Phase(\ct_{\out})}_t^q = \msg_{F} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)))[1]$.
\end{proof}



==> sections/cyclic-shift-and-permutations.tex <==
 
 
 
 
\subsection*{Efficient Cyclic Shift on the Coefficient Vector.}
  
Below we give our shifting algorithm. As explained in the introduction, our algorithm exploits the underlying ring structure to avoid excessive use of the relatively more expensive key switch.

\begin{definition}[Shifting]
We define a coefficient shifting algorithm $\Shift$ as follows.
\begin{description}
\item[$\Shift(\ct, \packKey, d):$]
Takes as input a ciphertext $\ct \in \RLWE_{\errDist_{\ct}, \deg, q}(\fr{s}, .)$, a packing key $\packKey \in \RLWE_{\errDist_{\packKey}, \deg, q}(\fr{s}, .)^{\deg \times \ell_{\packKey} \times \basis_{\packKey}}$ and the number of positions $d \in [\deg-1]$.
\begin{enumerate}
\item If $d \leq \frac{\deg}{2}$, then
\begin{enumerate}
\item For $i \in [d]$ set $\vec{v}[i] \exec \SampleExtract(\ct, \deg + 1 - i)$. 
\item Run $\vec{c}  \exec \PackLWEtoRLWE(\vec{v}, \packKey)$.   
\item Output $\vec{c}_{\out} \exec \ct  \cdot X^{d} + 2 \cdot \vec{c}$.
\end{enumerate}
\item If $d \ge \frac{\deg}{2}$, then
\begin{enumerate}
\item For $i \in [\deg - d]$ set $\vec{v}[i] \exec \SampleExtract(\ct, i)$. 
\item Run $\vec{c}  \exec \PackLWEtoRLWE(\vec{v}, \packKey)$.   
\item Output $\vec{c}_{\out} \exec  (2 \cdot \vec{c} - \ct) \cdot X^{d}$.
\end{enumerate}
\end{enumerate}
\end{description} 
\end{definition}
 

\begin{lemma}[Correctness of Shift]
\label{lemma:correctness-shift}
Let $\ct = \RLWE_{\errDist_{\bound_{\ct}}, \deg, q}(\fr{s}, \msg)$, where 
$\msg = \sum_{i=1}^{\deg} \msg_i \cdot X^{i - 1} \in \R_q$
and $\errDist_{\bound_{\ct}}$ is a $\bound_{\ct}$-Bounded distribution.
Let $\vec{s} \exec \KeyExtract(\fr{s}) \in \ZZ_q^{\deg}$, and  
$\packKey \exec \PackSetup(\errDist_{\bound_{\packKey}}, \deg, \deg, q, \vec{s}, \fr{s}, \basis_{\packKey})$, 
where $\basis_{\packKey} \in \NN$ and $\errDist_{\bound_{\packKey}}$ is a $\bound_{\packKey}$-Bounded distribution.
If $\ct_{\out} \exec \Shift(\ct, \packKey, d)$ for some $d \in [\deg]$,
then $\ct_{\out} \in \RLWE_{\errDist_{\bound}, \deg, q}(\fr{s}, \msg_{\out})$,
where  
\begin{align*}
\msg_{\out} = \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} + \sum_{i=1}^{\deg-d} \msg_{i} \cdot X^{d + i - 1} \in \R_q
\end{align*}
and $\errDist_{\bound}$ is a $\bound$-Bounded distribution with 
$\bound \leq \bound_{\ct} +  \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
\end{lemma}
 
 

\begin{proof}[of lemma \ref{lemma:correctness-shift} - Correctness Shifting]
Let us first start with the case $1 \leq d \leq \frac{\deg}{2}$.
Let us denote
$\ct = [\fr{b}, \fr{a}]^{\top} \in \R_q^2$, where $\fr{b} = \fr{a} \cdot \fr{s} + \sum_{i=1}^{\deg} \msg_i \cdot X^{i-1} + \sum_{i=1}^{\deg} e_{i} \cdot X^{i-1} \in \R_q$.
Then, let us denote $\vec{c}_s = \ct \cdot X^d = [\fr{b}_s, \fr{a}_s] \in \R_q^2$,
where $\fr{a}_s = \fr{a} \cdot X^d$ and 
$\fr{b}_s = \fr{a}_s \cdot \fr{s} \cdot X^d + \sum_{i=1}^{\deg} \msg_{i} \cdot X^{d + i-1} - \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} + \sum_{i=1}^{\deg} e_{i} \cdot X^{d + i - 1} - \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1}$.

Let us also denote $\vec{c}_p = [\fr{b}_p, \fr{a}_p] \in \R_q^2$,
where $\fr{b}_p = \fr{a}_p \cdot \fr{s} + \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1}  + \sum_{i=1}^{d} \fr{e}_{i}'' + \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1}$,
where $\sum_{i=1}^{d} \fr{e}_i''$ is the error as in vector packing in the proof of lemma 
\ref{lemma:correctness-of-vector-packing}. 
Recall that  $\norm{\sum_{i=1}^{d} \fr{e}_i''}_2 \leq d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.

Now let $\ct_{\out} = \vec{c}_s + 2 \cdot \vec{c}_p = [\fr{b}_{\out}, \fr{a}_{\out}] \in \R_q^2$.
Then we have  $\fr{a}_{\out} = \fr{a}_s + 2 \cdot \fr{a}_p$
and  
$\fr{b}_{\out}  = \fr{a}_{\out} \cdot \fr{s} + \msg_{\out} + \fr{e}'' + \fr{e}_{\ct}$
where $\fr{e}'' = 2 \cdot \sum_{i=1}^{d} \fr{e}_i''$,
\begin{align*}
\msg_{\out} &=  \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i-1} - \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} + 2 \cdot \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1} \\
 &= \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i-1} + \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{i-1},
\end{align*}  
and
\begin{align*}
\fr{e}_{\ct} &=  \sum_{i=1}^{\deg - d} e_{i} \cdot X^{d + i - 1} - \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1} + 2 \cdot \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1} \\
 &=  \sum_{i=1}^{\deg - d} e_{i} \cdot X^{d + i - 1} + \sum_{i=1}^d e_{\deg - d + i} \cdot X^{i-1}
\end{align*}
Hence we have 
$\norm{\fr{e}''}_2 \leq  2 \cdot d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$,
$\norm{\fr{e}_{\ct}}_2 \leq \bound_{\ct}$.
and,
$\norm{\Error(\ct_{\out})}_2   \leq  \norm{\fr{e}_{\ct}}_2 + \norm{\fr{e}''}_2 \leq \bound_{\ct} + 2 \cdot d \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Since, in this case $d \leq \frac{\deg}{2}$, we have
$\bound \leq \bound_{\ct} +   \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.

Now we will turn to the case with $\frac{N}{2} \leq d \leq \deg$.
In this case we have
$\vec{c}_p = [\fr{b}_p, \fr{a}_p] \in \R_q^2$,
where $\fr{b}_p = \fr{a}_p \cdot \fr{s} + \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{i-1}  + \sum_{i=1}^{\deg - d} \fr{e}_{i}'' + \sum_{i=1}^{\deg - d} e_{i} \cdot X^{i-1}$.
Let us denote 
$\vec{c}_{\out} = [\fr{b}_{\out}, \fr{a}_{\out}]^{\top} = (2 \cdot \vec{c}_p + \ct) \cdot X^{d} \in \R_q^2$.
Then $\fr{a}_{\out} = 2 \cdot (\fr{a}_p - \fr{a}_p) \cdot X^d \in \R_q$
and
$\fr{b}_{\out} = (2 \cdot \fr{b}_{p} + \fr{b}) \cdot X^d = \fr{a}_{\out} \cdot \fr{s} + \msg_{\out} + \fr{e}_{\out}$,
where
\begin{align*}
\msg_{\out} &= (2 \cdot \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{i-1} -  \sum_{i=1}^{\deg} \msg_i \cdot X^{i-1}) \cdot X^d \\
 &= (2 \cdot \sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} - \sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} -
 \sum_{i=1}^{d} \msg_{\deg - d + i} \cdot X^{\deg - d + i} ) \cdot X^{d} \\
 &= (\sum_{i=1}^{\deg - d} \msg_i \cdot X^{i-1} - \sum_{i=1}^d \msg_{\deg - d + i} \cdot X^{\deg - d + i} ) \cdot X^d \\
 &= \sum_{i=1}^{\deg - d} \msg_{i} \cdot X^{d + i - i} + \sum_{i=1}^d \msg_{\deg - d + i} \cdot X^{i-1}
\end{align*}
and
\begin{align*}
\fr{e}_{\out} &= (2 \cdot (\sum_{i=1}^{\deg - d} \fr{e}_{i}'' + \sum_{i=1}^{\deg - d} e_{i} \cdot X^{i-1}) - \sum_{i=1}^{\deg} e_{i} \cdot X^{i-1}) \cdot X^d \\
 &= 2 \cdot X^d \cdot \sum_{i=1}^{\deg - d} \fr{e}_i'' + \sum_{i=1}^{\deg - d} e_i \cdot X^{d + i - 1} + \sum_{i=1}^{d} e_{\deg - d + i} \cdot X^{i-1}.
\end{align*}
Hence, as earlier
we have that 
$\norm{\Error(\ct_{\out})}_2  \leq \bound_{\ct} + 2 \cdot (\deg - d) \cdot \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
Finally, since $\deg - d \leq \frac{\deg}{2}$,  we have
$\bound \leq \bound_{\ct} +  \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
 
\end{proof}
 
 

\subsection*{Coefficient Permutation}
Below, we give an algorithm to compute
any permutation of the RLWE slots.

\begin{definition}[Coefficient Permutation]
 We define a coefficient permutation algorithm $\Permute$ as follows.
\begin{description}
\item[$\Permute(\ct, \packKey, \pi):$]
Takes as input a ciphertext $\ct \in \RLWE_{\errDist_{\ct}, \deg, q}(\fr{s}, .)$, a packing key $\packKey \in \RLWE_{\errDist_{\packKey}, \deg, q}(\fr{s}, .)^{\deg \times \ell_{\packKey} \times \basis_{\packKey}}$ and a permutation $\pi:[\deg] \mapsto [\deg]$.
\begin{enumerate}
\item For all $i \in [\deg]$,
\begin{enumerate}
\item If $\pi(i) = j$,  and $i \neq j$, then $\vec{v}[j] \exec \LWEtoRLWE(\SampleExtract(\ct, j), \packKey, j)$.  
\end{enumerate} 
\item Set $\ct_{\out} = \ct$.
\item For all $i \in [\deg]$,
\begin{enumerate}
\item if $\pi(i) = j$ and $i \neq j$, then $\ct_{\out} \exec \ct_{\out} + (\vec{v}[j] - \vec{v}[i]) \cdot X^{i-1}$.
\end{enumerate}
\item Output $\ct_{\out}$.
\end{enumerate}
\end{description} 
\end{definition}


\begin{lemma}[Correctness of Permute]
\label{lemma:correctness-shift}
Let $\ct = \RLWE_{\errDist_{\bound_{\ct}}, \deg, q}(\fr{s}, \msg)$, where 
$\msg = \sum_{i=1}^{\deg} \msg_i \cdot X^{i - 1} \in \R_q$
and $\errDist_{\bound_{\ct}}$ is a $\bound_{\ct}$-Bounded distribution.
Let $\vec{s} \exec \KeyExtract(\fr{s}) \in \ZZ_q^{\deg}$, and  
$\packKey \exec \PackSetup(\errDist_{\bound_{\packKey}}, \deg, \deg, q, \vec{s}, \fr{s}, \basis_{\packKey})$, 
where $\basis_{\packKey} \in \NN$ and $\errDist_{\bound_{\packKey}}$ is a $\bound_{\packKey}$-Bounded distribution.
Let $\pi:\deg \mapsto \deg$ be a permutation.
If $\ct_{\out} \exec \Permute(\ct, \packKey)$,
then $\ct_{\out} \in \RLWE_{\errDist_{\bound}, \deg, q}(\fr{s}, \msg_{\out})$,
where  
\begin{align*}
\msg_{\out} = \sum_{i=1}^{\deg} \msg_{\pi(i)} \cdot X^{i-1} \in \R_q
\end{align*}
and $\errDist_{\bound}$ is a $\bound$-Bounded distribution with 
$\bound \leq \bound_{\ct} + 2 \cdot \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
\end{lemma}

\begin{proof}[Sketch]
The proof follows the reasoning of the proof of lemma \ref{lemma:correctness-shift}.
In particular, we extract all coefficients which need to be moved.
Furthermore, at each iteration of step 3.1, we subtract a $i$th message from the $i$th coefficient
from the packed ciphertext, effectively cleaning the slot.
Then add the $j$th message to the $i$th coefficient, effectively setting it the message.
For error analysis note that, subtracting the $i$th message, also subtracts the extracted error from the coefficient, just as described in the proof of lemma \ref{lemma:correctness-shift}.
Hence, if $d$ is the number of moves we need to perform, then
the error is bounded by $\bound \leq \bound_{\ct} + 2 \cdot d \cdot \deg  \cdot \ell_{\packKey} \cdot \bound_{\packKey} \leq \bound_{\ct} + 2 \cdot \deg^2 \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
\end{proof}


==> sections/fhew-blind-rotate.tex <==
 
  
\begin{definition}[FHEW Blind Rotation]
The blind rotation consists of a   key generation algorithm $\BRKeyGen_{\FHEW}$,
and the blind rotation algorithm $\BlindRotate_{\FHEW}$ defined as follows.

\begin{description}

\item[$\BRKeyGen_{\FHEW}(n, \vec{s}, \basis_{\brKey}, \bound_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s}):$]

Takes as input a dimension $n \in \NN$, a secret key $\vec{s} \in \ZZ_{2\cdot \deg}^{n \times 1}$ and a basis $\basis_{\brKey} \in \NN$,
a bound $\bound_{\brKey} \in \NN$,
 a degree $\deg \in \NN$ and a modulus $Q$ defining the ring $\R_{\deg, Q}$, 
 a basis $\basis_{\RGSW} \in \NN$, and a secret key $\fr{s} \in \R_{\deg, Q}$.

\begin{enumerate}
\item  Denote $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$.
\item For $i \in [n]$, $j \in [\ell_{\brKey}]$ and $k \in [\basis_{\brKey}]$, 
set a three dimensional matrix $\brKey$ as follows.  
\begin{enumerate} 
\item If $k-1 = 0$, then set  $\brKey[i, j, k] \exec 1$. 
\item Otherwise set  $\brKey[i, j, k] \exec \RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot (k - 1)})$. 

\end{enumerate}
\item Output $\brKey$.  
\end{enumerate}

\item[$\BlindRotate_{\FHEW}(\brKey, \acc, \ct):$]
The algorithm takes as input a blind rotation key $\brKey \in \RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{n \times \ell_{\brKey} \times \basis_{\brKey}}$,  
  an accumulator $\acc \in \RLWE_{\bound_{\acc}, \deg, Q}(\fr{s}, .)$, and
  a LWE sample $\ct  \in  \LWE_{\bound_{\ct}, n, q}(\vec{s}, .)$.  
\begin{enumerate} 
\item $\vec{c} \exec \ModSwitch(\ct, q, 2\cdot \deg)$.
\item Let $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \ZZ_{2\cdot \deg}^{(n+1) \times 1}$.

\item Run $\ma{A} \exec \Decomp_{\basis_{\brKey}, q}(\vec{a}) \in \ZZ_q^{n \times \ell_{\brKey}}$, where $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$.  
\item  For $i \in [n]$  do  
\begin{enumerate}
\item  For $j \in [\ell_{\brKey}]$  do
\begin{enumerate}
\item   $\acc \exec \extProd(\brKey[i, j, \ma{A}[i, j]+1], \acc)$.  
\end{enumerate}
\end{enumerate} 
\item  Output $\acc$.  
\end{enumerate}

\end{description} 
\end{definition}


\begin{lemma}[Correctness of FHEW-Style Bind-Rotation]
\label{lemma:correctness-fhew-blind-rotate}
 Let us define  $\ct \in \LWE_{\bound_{\ct}, n, q}(\vec{s}, .)$ to be a LWE sample and denote $\ct = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
Let $\basis_{\brKey} \in \NN$ be a basis, $\deg \in \NN$ be the degree and $Q \in \NN$ be the modulus defining the ring $\R_{\deg, Q}$.
Furthermore, let $\fr{s} \in \R_{\deg, Q}$,  $\basis_{\RGSW} \in \NN$,  $\bound_{\brKey} < Q$  
and $\acc \in \RLWE_{\bound_{\acc}, \deg, Q}(\fr{s}, \msg_{\acc})$.
%where $\errDist_{\bound_{\acc}}$ is a $\bound_{\acc}$-Bounded distribution.
If $\brKey \exec \BRKeyGen_{\FHEW}(n, \vec{s}, \basis_{\brKey}, \bound_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s})$
and $\acc_{\out} \exec \BlindRotate_{\FHEW}(\brKey, \acc, \ct, \basis_{\brKey})$,
then $\acc_{\out} \in \RLWE_{\bound_{\out}, \deg, Q}(\fr{s}, \msg_{\acc}^{\out})$,
where $\msg_{\acc}^{\out} = \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s} \mod 2\deg} \in \R_{\deg, Q}$ 
%and  $\bound_{\out}$ is a $\bound_{\out}$-Bounded distribution with 
\begin{align*}
\bound_{\out} \leq  \bound_{\acc}  +  n \cdot \ell_{\brKey} \cdot \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey},
\end{align*} 
where $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$. 
\end{lemma}




\begin{proof}[of lemma \ref{lemma:correctness-fhew-blind-rotate} - Correctness of FHEW-Style Bind-Rotation]
The proof follows from the correctness of the external product.
The message $\msg_{\acc}^{\out}$ is given by
\begin{align*}
\msg_{\acc}^{\out} &= \msg_{\acc} \cdot \prod_{i=1}^n \prod_{j=1}^{\ell_{\brKey}} X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot \ma{A}[i,j] \mod 2\deg}  \\
 &= \msg_{\acc} \cdot  \prod_{i=1}^n X^{- \vec{s}[i] \cdot \vec{a}[i] \mod 2\deg}\\
 &= \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s}\mod 2\deg}.
\end{align*}

Furthermore, for all $i \in [n]$, $j \in \ell_{\brKey}$ and $k \in [\basis_{\brKey}]$ we can denote 
$\brKey[i,j,k] = \RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(s, \msg_{\brKey[i,j,k]})$
and $\norm{\msg_{\brKey[i,j,k]}}_2 \leq \norm{X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot \ma{A}[i,j]}}_2 \leq 1$.
From the analysis of the external product
  we have that, if $\bound_{\acc_{\curr}}$ is the bound of the current accumulator, 
then multiplying it with the next RGSW sample from the blind rotation key,
results in a RLWE sample with bound $\bound_{\acc_{\next}} \leq \bound_{\acc_{\curr}}  +  \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$.
Hence, after $n \cdot \ell_{\brKey}$ iterations, we obtain
\begin{align*}
\bound_{\out} \leq  \bound_{\acc}  +  n \cdot \ell_{\brKey} \cdot \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}
\end{align*} 
\end{proof}


==> sections/fhew-tfhe-blind-rotate.tex <==
 
  
  
We recall two version of blind rotate. 
We specify those algorithms under the same names, as our scheme can be instantiated using both methods.
First we recall the version from FHEW.


\begin{definition}[FHEW Blind Rotation]
The blind rotation consists of a   key generation algorithm $\BRKeyGen_{\FHEW}$,
and the blind rotation algorithm $\BlindRotate_{\FHEW}$ defined as follows.

\begin{description}

\item[$\BRKeyGen_{\FHEW}(n, \vec{s}, \basis_{\brKey}, \errDist_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s}):$]

Takes as input a dimension $n \in \NN$, a secret key $\vec{s} \in \ZZ_{2\cdot \deg}^{n \times 1}$ and a basis $\basis_{\brKey} \in \NN$,
an error distribution $\errDist_{\brKey}$,
 a degree $\deg \in \NN$ and a modulus $Q$ defining the ring $\R_Q$, 
 a basis $\basis_{\RGSW} \in \NN$, and a secret key $\fr{s} \in \R_Q$.

\begin{enumerate}
\item  Denote $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$.
\item For $i \in [n]$, $j \in [\ell_{\brKey}]$ and $k \in [\basis_{\brKey}]$, 
set a three dimensional matrix $\brKey$ as follows.  
\begin{enumerate} 
\item If $k-1 = 0$, then set  $\brKey[i, j, k] \exec 1$. 
\item Otherwise set  $\brKey[i, j, k] \exec \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot (k - 1)})$. 

\end{enumerate}
\item Output $\brKey$.  
\end{enumerate}

\item[$\BlindRotate_{\FHEW}(\brKey, \acc, \ct):$]
The algorithm takes as input a blind rotation key $\brKey \in \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{n \times \ell_{\brKey} \times \basis_{\brKey}}$,  
  an accumulator $\acc \in \RLWE_{\errDist_{\acc}, \deg, Q}(\fr{s}, .)$, and
  a LWE sample $\ct  \in  \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)$.  
\begin{enumerate} 
\item $\vec{c} \exec \ModSwitch(\ct, q, 2\cdot \deg)$.
\item Let $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \ZZ_{2\cdot \deg}^{(n+1) \times 1}$.

\item Run $\ma{A} \exec \Decomp_{\basis_{\brKey}, q}(\vec{a}) \in \ZZ_q^{n \times \ell_{\brKey}}$, where $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$.  
\item  For $i \in [n]$  do  
\begin{enumerate}
\item  For $j \in [\ell_{\brKey}]$  do
\begin{enumerate}
\item   $\acc \exec \extProd(\brKey[i, j, \ma{A}[i, j]+1], \acc)$.  
\end{enumerate}
\end{enumerate} 
\item  Output $\acc$.  
\end{enumerate}

\end{description} 
\end{definition}


\begin{lemma}[Correctness of FHEW-Style Bind-Rotation]
\label{lemma:correctness-fhew-blind-rotate}
 Let us define  $\ct \in \LWE_{\errDist_{\bound_{\ct}}, n, q}(\vec{s}, .)$ to be a LWE sample and denote $\ct = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
Let $\basis_{\brKey} \in \NN$ be a basis, $\deg \in \NN$ be the degree and $Q \in \NN$ be the modulus defining the ring $\R_Q$.
Furthermore, let $\fr{s} \in \R_Q$,  $\basis_{\RGSW} \in \NN$,  $\errDist_{\bound_{\brKey}}$ be a $\bound_{\brKey}$-Bounded distribution
and $\acc \in \RLWE_{\errDist_{\bound_{\acc}}, \deg, Q}(\fr{s}, \msg_{\acc})$,
where $\errDist_{\bound_{\acc}}$ is a $\bound_{\acc}$-Bounded distribution.
If $\brKey \exec \BRKeyGen_{\FHEW}(n, \vec{s}, \basis_{\brKey}, \errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}, \fr{s})$
and $\acc_{\out} \exec \BlindRotate_{\FHEW}(\brKey, \acc, \ct, \basis_{\brKey})$,
then $\acc_{\out} \in \RLWE_{\errDist_{\bound_{\out}}, \deg, Q}(\fr{s}, \msg_{\acc}^{\out})$,
where $\msg_{\acc}^{\out} = \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s} \mod 2\deg} \in \R_Q$ and 
$\errDist_{\bound_{\out}}$ is a $\bound_{\out}$-Bounded distribution
with 
\begin{align*}
\bound_{\out} \leq  \bound_{\acc}  +  n \cdot \ell_{\brKey} \cdot \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey},
\end{align*} 
where $\ell_{\brKey} = \roundUp{\log_{\basis_{\brKey}}{2\cdot \deg}}$. 
\end{lemma}




\begin{proof}[of lemma \ref{lemma:correctness-fhew-blind-rotate} - Correctness of FHEW-Style Bind-Rotation]
The proof follows from the correctness of the external product.
The message $\msg_{\acc}^{\out}$ is given by
\begin{align*}
\msg_{\acc}^{\out} &= \msg_{\acc} \cdot \prod_{i=1}^n \prod_{j=1}^{\ell_{\brKey}} X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot \ma{A}[i,j] \mod 2\deg}  \\
 &= \msg_{\acc} \cdot  \prod_{i=1}^n X^{- \vec{s}[i] \cdot \vec{a}[i] \mod 2\deg}\\
 &= \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s}\mod 2\deg}.
\end{align*}

Furthermore, for all $i \in [n]$, $j \in \ell_{\brKey}$ and $k \in [\basis_{\brKey}]$ we can denote 
$\brKey[i,j,k] = \RGSW_{\errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}}(s, \msg_{\brKey[i,j,k]})$
and $\norm{\msg_{\brKey[i,j,k]}}_2 \leq \norm{X^{- \basis_{\brKey}^{j-1} \cdot \vec{s}[i] \cdot \ma{A}[i,j]}}_2 \leq 1$.
From the analysis of the external product
  we have that, if $\bound_{\acc_{\curr}}$ is the bound of the current accumulator, 
then multiplying it with the next RGSW sample from the blind rotation key,
results in a RLWE sample with bound $\bound_{\acc_{\next}} \leq \bound_{\acc_{\curr}}  +  \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$.
Hence, after $n \cdot \ell_{\brKey}$ iterations, we obtain
\begin{align*}
\bound_{\out} \leq  \bound_{\acc}  +  n \cdot \ell_{\brKey} \cdot \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}
\end{align*} 
\end{proof}



%  
%
%\begin{definition}[TFHE Blind Rotation]
%The blind rotation consists of a key   generation algorithm $\BRKeyGen_{\TFHE}$,
%and the blind rotation algorithm $\BlindRotate_{\TFHE}$ defined as follows.
%
%\begin{description}
%
%\item[$\BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \errDist_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s}):$]
%
%
%Takes as input a dimension $n \in \NN$, a secret key $\vec{s} \in \ZZ_t^{n \times 1}$ and a vector $\vec{u} \in \ZZ^{u}$,
%an error distribution $\errDist_{\brKey}$,
% a degree $\deg \in \NN$ and a modulus $Q$ defining the ring $\R_Q$, 
% a basis $\basis_{\RGSW} \in \NN$, and a secret key $\fr{s} \in \R_Q$.
%
% 
%\begin{enumerate}
%\item  Set a matrix $\ma{Y} \in \BB^{n \times u}$ such as follows:  
%\begin{enumerate}
%\item For $i \in [n]$ set the $i$-th row of $\ma{Y}$, to satisfy 
%$\vec{s}[i] = \sum_{j=1}^{u} \ma{Y}[i, j] \cdot \vec{u}[j]$, 
%\end{enumerate} 
%\item For $i \in [n]$, $j \in [u]$ set $\brKey[i,j] = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, \ma{Y}[i,j])$. 
%\item Output  $\brKey$. 
%\end{enumerate}
%
%\item[$\BlindRotate_{\TFHE}(\brKey, \acc, \ct, \vec{u}):$]
%The algorithm takes as input a blind rotation key $\brKey = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{n \times u}$,  
%  an accumulator $\acc \in \RLWE_{\errDist_{\acc}, \deg, Q}(\fr{s}, .)$, 
% a LWE sample $\ct \in  \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)$, where $\vec{s} \in \ZZ_t^{n}$ with $t \leq q$, and a vector $\vec{u} \in \ZZ^{u}$.
%\begin{enumerate}
%\item $\vec{c} \exec \ModSwitch(\ct, q, \deg)$.
%\item Let $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \ZZ_{\deg}^{(n+1) \times 1}$. 
%\item For $i \in [n]$ do: 
%\begin{enumerate}
%\item  For $j \in [u]$ do:
% \begin{align*}
% \acc \exec \CMux(\brKey[i, j], \acc \cdot X^{-\vec{a}[i] \cdot \vec{u}[j]}), \acc)
%\end{align*}   
%\end{enumerate} 
%\item Output $\acc$. \\
%\end{enumerate} 
%\end{description} 
%\end{definition}
% 
% 
% 
%\begin{lemma}[Correctness of TFHE-Style Bind-Rotation]
%\label{lemma:correctness-tfhe-blind-rotate}
%Let  $\vec{u} \in \ZZ^u$ be a vector 
% that for all $y \in \ZZ_q$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod q$.
% Let   $\ct \in \LWE_{\errDist_{\bound_{\ct}}, n, q}(\vec{s}, .)$ to be a LWE sample and denote $\ct = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
%Let $\deg \in \NN$ be the degree and $Q \in \NN$ be the modulus defining the ring $\R_Q$.
%Furthermore, let $\fr{s} \in \R_Q$,  $\basis_{\RGSW} \in \NN$,  $\errDist_{\bound_{\brKey}}$ be a $\bound_{\brKey}$-Bounded distribution
%and $\acc \in \RLWE_{\errDist_{\bound_{\acc}}, \deg, Q}(\fr{s}, \msg_{\acc})$,
%where $\errDist_{\bound_{\acc}}$ is a $\bound_{\acc}$-Bounded distribution.
%If $\brKey \exec \BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}, \fr{s})$
%and $\acc_{\out} \exec \BlindRotate_{\TFHE}(\brKey, \acc, \ct, \vec{u})$,
%then $\acc_{\out} \in \RLWE_{\errDist_{\bound_{\out}}, \deg, Q}(\fr{s}, \msg_{\acc}^{\out})$,
%where $\msg_{\acc}^{\out} = \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s}} \in \R_Q$ and 
%$\errDist_{\bound_{\out}}$ is a $\bound_{\out}$-Bounded distribution
%with  
%\begin{align*} 
%\bound_{\out} \leq  \bound_{\acc} +  n \cdot u \cdot  \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}
%\end{align*} 
%\end{lemma}
%  
%  
% 
%\begin{proof}[of lemma \ref{lemma:correctness-tfhe-blind-rotate} - Correctness of TFHE-Style Bind-Rotation]
%Note that the blind rotation key $\brKey$ consists of samples of bits:
%$\RGSW_{\errDist, \deg, Q, \basis_{\RGSW}}(\fr{s}, \ma{Y}[i,j])$, where $\ma{Y}[i,j] \in \BB$ for $i \in [n]$ 
%and $j \in [u]$.
%Denote the current accumulator as $\acc_{curr} \in \RLWE_{\errDist_{\bound_{\curr}}, \deg, Q}(\fr{s}, \msg_{\curr})$ for some $\msg_{\curr} \in \R_Q$.
%If we increment 
%$\acc_{\next} \exec \CMux(\brKey[i, j], \acc_{\curr} \cdot X^{-\vec{a}[i] \cdot \vec{u}[j]}), \acc_{\curr})$
%for some $i \in [n]$ and $j \in [u]$, then from correctness of the CMux gate 
%we have that $\acc_{\next} \in \RLWE_{\errDist_{\bound_{\next}}, \deg, Q}(\fr{s}, \msg_{\next})$,
%where $\msg_{\next} = \msg_{\curr} \cdot X^{-\vec{a}[i] \cdot \vec{u}[j] \cdot K[i, j]}$.
%Overall, we can represent the last message $\msg_{\out}$ as
%\begin{align*}
%\msg_{\out} &= \msg_{\acc} \cdot \prod_{i=1}^n \prod_{j=1}^{u}  X^{-\vec{a}[i] \cdot \vec{u}[j] \cdot K[i, j]} \\
% &=  \msg_{\acc} \cdot \prod_{i=1}^n X^{-\vec{a}[i] \cdot \vec{s}[i]} \\
% &= \msg_{\acc} \cdot X^{- \vec{a}^{\top} \cdot \vec{s}}.
%\end{align*}
% 
%Furthermore, let $\errDist_{\bound_{\curr}}$ be a $\bound_{\curr}$-Bounded distribution. 
%From the analysis of the internal product we have that 
%$\bound_{\next} \leq \bound_{\curr} +   \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}$.
%  
%Finally since we perform $n \cdot u$ iterations,
%we have that
%\begin{align*} 
%\bound_{\out} \leq  \bound_{\acc} +  n \cdot u \cdot  \deg \cdot \ell_{\RGSW} \cdot  (\basis_{\RGSW} - 1) \cdot \bound_{\brKey}.
%\end{align*} 
%\end{proof} 
%  
%  
%  

==> sections/functional-keyswitch-and-full-domain-gsw-product.tex <==
  
 
 
\begin{definition}[LWE to RLWE Functional Keyswitch]
Key-switching is specified by a setup algorithm $\KeySwitchSetup$ and
a key switch algorithm $\KeySwitch$ defined as follows.
\begin{description}
\item[$\FuncKeySwitchSetup(\errDist_{\keySwitchKey}, n, q, \deg, \vec{s}, \fr{s}, \fr{d}, \basis_{\keySwitchKey}):$]
Takes as input a error distribution $\errDist_{\keySwitchKey}$, $n \in \NN$,  $\deg \in \NN$, 
a vector  $\vec{s} \in \ZZ_q^{n \times 1}$,  ring elements  $\fr{s}, \fr{d} \in \R_q$, 
and a basis $\basis_{\keySwitchKey} \in \NN$.  
\begin{enumerate}
\item Denote $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$.
\item For $i \in [n]$ and $j \in [\ell_{\keySwitchKey}]$ set
 $\keySwitchKey_1[i,j] \exec \RLWE_{\errDist_{\keySwitchKey}, \deg, q}(\fr{s}, \fr{s} \cdot \vec{s}[i] \cdot \basis_{\keySwitchKey}^{j-1}) $. 
 
 \item For $j \in [\ell_{\keySwitchKey}]$ set
 $\keySwitchKey_2[i,j] \exec \RLWE_{\errDist_{\keySwitchKey}, \deg, q}(\fr{s}, \fr{s} \cdot \basis_{\keySwitchKey}^{j-1})$. 
\item Output $\keySwitchKey = (\keySwitchKey_1, \keySwitchKey_2)$. 
\end{enumerate}


\item[$\FuncKeySwitch(\vec{c}, \keySwitchKey):$]
Takes as input a sample $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \LWE_{\errDist_{\vec{c}}, n, q}(\vec{s}, \msg)$ and 
 a key-switching key $\keySwitchKey = (\keySwitchKey_1, \keySwitchKey_2)$, 
 where $\keySwitchKey_i \in \RLWE_{\errDist_{\keySwitchKey}, \deg, q}(\fr{s}, .)^{n \times \ell_{\keySwitchKey}}$
 for $i \in [2]$ and $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$.  
\begin{enumerate}
%\item Denote $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$.
\item  Compute $\ma{A} \exec \Decomp_{\basis_{\keySwitchKey}, q}(\vec{a}) \in \ZZ_{\basis_{\keySwitchKey}}^{n \times \ell_{\keySwitchKey}}$.

\item Compute $\vec{b} \exec \Decomp_{\basis_{\keySwitchKey}, q}(b) \in \ZZ_{\basis_{\keySwitchKey}}^{\ell_{\keySwitchKey}}$.

\item Set $\vec{c}_{\out} \exec \sum_{j=1}^{\ell_{\keySwitchKey}} \vec{b}[j] \cdot  \keySwitchKey_2[j] - \sum_{i=1}^{n} \sum_{j=1}^{\ell_{\keySwitchKey}} \ma{A}[i,j] \cdot \keySwitchKey_1[i,j]$.
\item Output $\vec{c}_{\out}$.  
\end{enumerate}
\end{description}
\end{definition}  


\begin{lemma}[Correctness of Key-Switching]
\label{lemma:correctness-of-key-switch}
Let  $\basis_{\keySwitchKey} \in \NN$,  $\deg \in \NN$, $\fr{s}, \fr{d} \in \R_q$ and
  $\vec{c} \in \LWE_{\errDist_{\bound_{\vec{c}}}, n, q}(\vec{s}, \msg)$,
where $\errDist_{\bound_{\vec{c}}}$ is a $\bound_{\vec{c}}$-Bounded distribution
and $\norm{\fr{d}}_2 \leq \bound_{\fr{d}}$.
Furthermore, let $\errDist_{\bound_{\keySwitchKey}}$, be a $\bound_{\keySwitchKey}$-Bounded distribution.
If we execute $\keySwitchKey \exec \KeySwitchSetup(\errDist_{\keySwitchKey}, n, q, \deg, \vec{s}, \fr{s}, \fr{d}, \basis_{\keySwitchKey})$ 
and $\vec{c}_{\out} \exec \KeySwitch(\vec{c}, \keySwitchKey, \basis_{\keySwitchKey})$,
then $\vec{c}_{\out} \in \RLWE_{\errDist_{\bound}, \deg, q}(\fr{s}, \msg \cdot \fr{d})$,
where $\errDist_{\bound}$ is a $\bound$-Bounded distribution with
$\bound \leq n \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) +  \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) + \bound_{\fr{d}} \cdot \bound_{\vec{c}}$, where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$.
\end{lemma}
 
   

\begin{proof}[of lemma \ref{lemma:correctness-of-key-switch} - Correctness of Key-Switching]
Let us first note that for all $i \in [n]$ we have
\begin{align*}
[\fr{b}_i, \fr{a}_i]^{\top} &= \sum_{j=1}^{\ell_{\keySwitchKey}} \ma{A}[i,j] \cdot \keySwitchKey_1[i,j] \\
&= \sum_{j=1}^{\ell_{\keySwitchKey}} \ma{A}[i,j] \cdot \RLWE_{\errDist_{\bound_{\keySwitchKey}}, \deg, q}(\fr{s}, \fr{d} \cdot \vec{s}[i] \cdot \basis_{\keySwitchKey}^{j}) \\
&=  \RLWE_{\errDist_{\bound_{1}}, \deg, q}(\fr{s}, \fr{d} \cdot \vec{a}[i] \cdot \vec{s}[i]),
\end{align*}
where $\errDist_{\bound_{1}}$ is a $\bound_1$-Bounded distribution with $\bound_1 \leq \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1)$.
Then  note that
\begin{align*}
[\fr{b}', \fr{a}']^{\top} &= \sum_{i=1}^{n} \RLWE_{\errDist_{\bound_{1}}, \deg, q}(\fr{s}, \fr{d} \cdot \vec{a}[i] \cdot \vec{s}[i]) \\ 
 &=  \RLWE_{\errDist_{\bound_{2}}, \deg, q}(\fr{s}, \fr{d} \cdot  \sum_{i=1}^{n} \vec{a}[i] \cdot \vec{s}[i])  \\
 &= \RLWE_{\errDist_{\bound_{2}}, \deg, q}(\fr{s}, \fr{d} \cdot \vec{a}^{\top} \cdot \vec{s}),
\end{align*}
where $\errDist_{\bound_{2}}$ is a $\bound_{2}$-Bounded distribution with 
$\bound_{2} \leq n \cdot \bound_1 \leq n \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1)$.

Similarly, we have
\begin{align*}
[\fr{b}'', \fr{a}'']^{\top} &= \sum_{j=1}^{\ell_{\keySwitchKey}} \vec{b}[j] \cdot  \keySwitchKey_2[j] \\
&= \sum_{j=1}^{\ell_{\keySwitchKey}} \vec{b}[j] \cdot  \RLWE_{\bound_{\keySwitchKey}, \deg, q}(\fr{s},  \fr{d} \cdot \basis_{\keySwitchKey}^{j-1}) \\
&= \RLWE_{\errDist_{\bound_{3}}, \deg, q}(\fr{s},  \fr{d} \cdot \sum_{j=1}^{\ell_{\keySwitchKey}} \vec{b}[j] \cdot \basis_{\keySwitchKey}^{j-1}) \\
&= \RLWE_{\errDist_{\bound_{3}}, \deg, q}(\fr{s},  \fr{d} \cdot b),
\end{align*}
where $\errDist_{\bound_{3}}$ is a $\bound_{3}$-Bounded distribution with $\bound_{3} \leq \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1)$.

Let us denote $b = \vec{a}^{\top} \cdot \vec{s} + \msg + e$ and
$b' = \vec{a}'^{\top} \cdot \vec{s} + \vec{a}^{\top} \cdot \vec{s} + e'$,
then
\begin{align*}
\vec{c}_{\out} &= [\fr{b}'', \fr{a}'']^{\top} - [\fr{b}', \fr{a}']^{\top} \\
 &= \RLWE_{\errDist_{\bound_{3}}, \deg, q}(\fr{s},  \fr{s} \cdot b) - \RLWE_{\errDist_{\bound_{2}}, \deg, q}(\fr{s}, \vec{a}^{\top} \cdot \vec{s}) \\
 &= \RLWE_{\errDist_{\bound_{4}}, \deg, q}(\fr{s}, \fr{d} \cdot (\msg + e)) \\
 &= \RLWE_{\errDist_{\bound_{5}}, \deg, q}(\fr{s}, \fr{d} \cdot \msg)
\end{align*}
Hence, $\vec{c}_{\out}$ is a valid RLWE sample of $\msg$ with respect to key $\fr{s}$ 
and $\norm{\Error(\vec{c})}_2  \leq \bound_{2} + \bound_{3} + \norm{\fr{d} \cdot e}_2 \leq
n \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) +  \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) + \bound_{\fr{d}} \cdot \bound_{\vec{c}}$.
\end{proof}


  
  
  
  
  
 
\begin{definition}[Gadget-LWE to RGSW Keyswitch]
 Key-switching is specified by a setup algorithm $\KeySwitchSetup$ and
a key switch algorithm $\KeySwitch$ defined as follows.
\begin{description}
\item[$\RGSWKeySwitchSetup(\errDist_{\keySwitchKey}, n, q, \deg, \vec{s}, \fr{s}, \basis_{\keySwitchKey})$:]
Takes as input a error distribution $\errDist_{\keySwitchKey}$, $n \in \NN$,  $\deg \in \NN$, 
a vector  $\vec{s} \in \ZZ_q^{n \times 1}$, a ring element $\fr{s} \in \R_q$, 
and a basis $\basis_{\keySwitchKey} \in \NN$.  
\begin{enumerate}
\item $\keySwitchKey_1 \exec \KeySwitchSetup(\errDist_{\keySwitchKey}, n, q, \deg, \vec{s}, \fr{s}, \fr{d}, \basis_{\keySwitchKey})$ - normal keyswitch

\item $\keySwitchKey_2 \exec \FuncKeySwitchSetup(\errDist_{\keySwitchKey}, n, q, \deg, \vec{s}, \fr{s}, \fr{d}, \basis_{\keySwitchKey})$ - functional keyswitch
\end{enumerate}

\item[$\RGSWKeySwitch(\ma{C}, \keySwitchKey)$:]
Takes as input a sample $\ma{C} =  [\LWE_{\errDist_{\vec{c}}, n, q}(\vec{s}, \msg \cdot \basis_{\keySwitchKey}^{j-1})]_{j \in [\ell_{\keySwitchKey}]}^{\top}$, where $\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$
and 
 a key-switching key $\keySwitchKey = (\keySwitchKey_1, \keySwitchKey_2)$.
\begin{enumerate}  
\item For all $j \in [\ell_{\keySwitchKey}]$ do
\begin{enumerate}
\item $\ma{C}_{\out}[i] \exec \KeySwitch(\ma{C}[j], \keySwitchKey_1)$ - Normal Keyswitch

\item $\ma{C}_{\out}[i + \ell_{\keySwitchKey}] \exec \FuncKeySwitch(\ma{C}[j], \keySwitchKey_2)$ - Functional Keyswitch
\end{enumerate}

\item Output $\ma{C}_{\out}$.
\end{enumerate}
\end{description}
 \end{definition}
 
 
 
 \begin{lemma}[Correctness of Gadget-LWE to RGSW Keyswitch]
TODO Its correct...
 \end{lemma}
 
 \begin{proof}
 Note that $\ma{C}_{\out}[i] = \RLWE(\msg \cdot 2^{i-1})$ for $i \in [\ell_{\keySwitchKey}]$
 and $\ma{C}_{\out}[i] = \RLWE(- \fr{s} \msg \cdot 2^{i-1})$ for $i \in [\ell_{\keySwitchKey}, 2 \cdot \ell_{\keySwitchKey}]$.
 Easy peasy.
 \end{proof}
 
  
 
 \begin{definition}[Full Domain $\GGSW$ Product]\label{def:full-domain-ggsw-product}
 We define the full domain $\GGSW$ product as follows.
 \begin{description}
 \item[$\FullDomainGGSWConstProduct(\ma{C}, \fr{a})$:]
 The algorithm takes as input a sample $\ma{C} = \GGSW_{\errDist_{\bound_{\ma{C}}}, n, \deg, q, \basis}(\vec{s}, \msg_{\ma{C}})$,
 and $\fr{a} \in \R_q$, the algorithm outputs $\ma{C}_{\out}$ defined as
 \begin{align*}
	\ma{C}_{\out} \exec \intProd(\ma{C}, \fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)}))
 \end{align*}
\end{description}  
 \end{definition}
 
 
 \begin{lemma}[Correctness of $\FullDomainGGSWConstProduct$]
 Let us denote $\ma{C} = \GGSW_{\errDist_{\bound_{\ma{C}}}, n, \deg, q, \basis}(\vec{s}, \msg)$,
 where $\msg \in \R_q$ and $\errDist_{\bound_{\ma{C}}}$ is a $\bound_{\ma{C}}$-bounded distribution.
 Let $\fr{a} \in \R_q$ and $\ma{C}_{\out} \exec \FullDomainGGSWConstProduct(\ma{C}, \fr{a})$.
 Then $\ma{C}_{\out} = \GGSW_{\errDist_{\bound_{\out}}, n, \deg, q, \basis}(\vec{s}, \fr{a} \cdot \msg)$
 where $\errDist_{\bound}$ is a $\bound_{\out}$-bounded distribution with 
 $\bound \leq  \deg \cdot  (n+1) \cdot \ell \cdot (\basis - 1) \cdot \bound_{\ma{C}}$ in general, and
 $\bound \leq  (n + 1) \cdot \ell \cdot (\basis - 1) \cdot \bound_{\ma{C}}$ when $\fr{a}$ is a monomial.
 \end{lemma}
 
 \begin{proof}
 Denote $\ma{C} = \ma{A} + \msg \cdot\ma{G}_{\ell, \basis, (n+1)}$, where  $\ma{A} \in \R_q^{(n+1) \cdot \ell \times (n+1)}$.
 From the definition of $\FullDomainGGSWConstProduct$,
 we have 
\begin{align*}
\ma{C}_{\out} &= \intProd(\ma{C}, \fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)})  \\
 &= \Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)})  \cdot \ma{C} \\
 &= \Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)})  \cdot \ma{A} + \msg \cdot \Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)})  \cdot \ma{G}_{\ell, \basis, (n+1)} \\
 &= \Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)}) \cdot \ma{A} + \fr{a} \cdot \msg \cdot \ma{G}_{\ell, \basis, (n+1)} \\
 &= \ma{A}_{\out} + \msg \cdot \ma{G}_{\ell, \basis, (n+1)}
\end{align*} 
 where $\ma{A}_{\out}[i, \ast] = \sum_{j=1}^{(n+1) \cdot \ell} \Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)}))[i, j] \cdot  \ma{A}[j, \ast]$. Note that $\ma{A}_{\out}[i, \ast]$ is the linear
 combination of $(n+1) \cdot \ell$ $\GLWE$ samples from $\ma{A}$ with polynomials from $\R_{\basis}$.
 Therefore, given that $\bound_{\ma{C}}$ is the bound on the error of $\ma{C}$, we have that $\bound \leq  \deg   \cdot  (n+1) \cdot \ell \cdot (\basis - 1) \cdot \bound_{\ma{C}}$. 
 Finally, if $\fr{a}$ is a monomial, then the matrix
 $\Decomp(\fr{a} \cdot \ma{G}_{\ell, \basis, (n+1)}))$ consists also of monomials. 
 Hence, in this case we have that  $\bound \leq (n+1) \cdot \ell \cdot (\basis - 1) \cdot \bound_{\ma{C}}$.
 
 \end{proof}
 
 
 
 

==> sections/impl-timings.tex <==
In this subsection we present the timings of our algorithm. 

Our system featured 32GB of ram and used an AMD processor RX 2700X with a clock speed of 3.7 GHZ and the measurements are averaged over 30 runs. 
We implemented our bootstrapping technique on top of the latest\footnote{\texttt{commit} 793405a6aed6879621c7f11947daeead95c93426} version of the PALISADE library \cite{PALISADE}  which
already featured an implementation of \cite{EPRINT:DucMic14b} and \cite{AC:CGGI16}. 

We test our implementation on three sets of parameters, depicted in Table~\ref{tbl:params}, which follow the recommendation of the library's developers. Additionally,
the table includes the security level provided by Albrecht et al's estimator\footnote{\url{https://bitbucket.org/malb/lwe-estimator/src/master/}} based on \cite{albrecht2015concrete}.




\begin{table}
	\setlength{\tabcolsep}{6pt}
	\centering
	\caption{Parameters sets and security according to Albrecht et al's estimator}
	\label{tbl:params}
	\begin{tabular}{c | c || c | c | c | c | c | c | c | c }
		\hline
		Set & $\lambda$ & $n$ & $N$ & $q$ & $Q$ & $\sigma$ & $\basis_{\brKey}$ & $\basis_{\packKey}$ & $\basis_{\keySwitchKey}$   \\
		\hline 
		1 & $40$ & $32$ & $512$ & $512$ & $4294957057$ & $3.19$ & $2^{11}$ & $2^{9}$ & $23$  \\
		2 & $98$ & $256$ & $1024$ & $512$ & $4294957057$ & $3.19$ & $2^{16}$ & $2^8$ & $23$  \\
		3 & $128$  & $512$ & $1024$ & $1024$ & $134215681$ & $3.19$ & $2^9$ & $2^8$ & $23$  \\
		\hline
	\end{tabular}
\end{table}

The parameter $\basis_{\packKey}$ was chosen based on the maximum speedup it provided. Figure~\ref{fig:impact} 
depicts how increasing the decomposition base affects the execution time of the bootstrapping, with regards to the first parameter set. We
chose powers of 2 bases due to efficient decomposition. From $\basis_{\packKey} = 512$ on, higher values no longer provided a speedup. In fact, using a 
base 1024 increased the bootstrapping time and utilized a large amount of memory (22GB). 
\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{graphics/baseimpact}
	\caption{Impact of $\basis_\packKey$ on execution time}
	\label{fig:impact}
\end{figure}

To choose a plaintext dimension $t$, we need to determine an appropriate bound $\bound$ and by extension $\Pr_{e \leftarrow \X_{\secpar}}[|e| \ge \bound]$. In practice,
$\X_{\secpar}$ will be a Gaussian distribution centered at $\mu=0$ and of standard deviation $\sigma$. Thus, we can use:
\begin{align*}
	\Pr_{e \leftarrow \X_{\secpar}}[|e| \ge \bound] &= 1 - \Pr_{e \leftarrow \X_{\secpar}}[|e| \leq \bound] \\
	&= 1 - \frac{1}{\sigma\sqrt{2 \pi}}\int_{-\bound}^\bound \exp\left(-\frac{1}{2}\left(\frac{e-\mu}{\sigma}\right)^2\right) de\\
	&= 1 - \int_{-\frac{\bound - \mu}{\sigma\sqrt{2}}}^{\frac{\bound - \mu}{\sigma\sqrt{2}}} \exp\left(-t^2\right) dt\\
	&= 1 - \mathsf{erf}\left(\frac{\bound - \mu}{\sigma\sqrt{2}}\right)\\
	&= 1 - \mathsf{erf}\left(\frac{\bound}{\sigma\sqrt{2}}\right)
\end{align*}

By picking $\bound$ sufficiently large so that $\epsilon(\bound) = \Pr_{e \leftarrow \X_{\secpar}}[|e| \ge \bound]$ is close to $0$, we can select the largest $t$ such that $t \leq \frac{q}{2\bound}$, following Theorem~\ref{thm:bootstrapping-pre-rotation}. In our tests, we picked $\bound = 16$ with $\epsilon(\bound) = 5.2 \cdot 10^{-7}$ resulting 
in plaintext moduli of $16$, $16$ and $32$ respectively for parameter sets 1,2 and 3. It possible to achieve larger plaintext space by setting smaller bounds. However,
this would increase the risk of a bootstrapping failure which can be observed in Table~\ref{tbl:bound-pt}. In our tests we chose a very conservative value for $\bound$ in order
to guarantee the accuracy of the procedure. One can easily double the maximum plaintext
by reducing the bound; in some application it might not matter whether the result differs by a small amount.

\begin{table}
	\setlength{\tabcolsep}{7pt}
	\centering
	\caption{Possible bounds and induced plaintext dimensions for all parameter sets}
	\label{tbl:bound-pt}
	\begin{tabular}{c | c | c | c  }
		\hline
		$\bound$ & $\epsilon(\bound)$ & $t$ (Set 1 and 2) & $t$ (Set 3)\\
		\hline
		1 & $0.75$ & $256$ & $512$ \\
		4 & $0.21$ & $64$ & $128$ \\
		8 & $1.21 \cdot 10^{-2}$& $32$ & $64$ \\
		12 & $1.6 \cdot 10^{-4}$ & $21$ &$43$ \\
		16 & $5.2 \cdot 10^{-7}$ & $16$ & $32$ \\
		20 & $3.61 \cdot 10^{-10}$ & $13$ & $26$ \\
		24 & $5.32 \cdot 10^{-14}$ & $11$ & $21$ \\
		\hline	
	\end{tabular}

\end{table}

Table~\ref{tbl:timings} shows the timing result of the bootstrapping procedure. We note that our implementation has not been optimized and more efficient packing and decomposition code might offer significant speedups. Moreover,
parameters were not aggressively optimized and thus may not offer an optimal relationship between security, efficiency
and maximum plaintext dimension.

The most expensive operation during bootstrapping is the packing algorithm $\LWEtoRLWE$, which on average
takes around 17ms with the weakest parameter set, and 115ms. with the strongest.
 We mitigate this to some extent by computing the individual packing operations required by $\PackLWEtoRLWE$ in
parallel. Nevertheless, the shift based bootstrapping procedure takes almost 10 minutes with the strongest parameter set. To some extent this may be attributed to the fact that
the classical TFHE/GINX style rotation only requires a product with a monomial within the $\CMux$. This can be achieved with little computation, by copying the coefficients in memory and
negating certain entries. On the other hand, our technique requires a large number of transformations, which
may not be very efficient in higher dimensions; successive entries are too large to be loaded into the cache and might
not even be accessed sequentially.

%\begin{table}
%	\setlength{\tabcolsep}{6pt}
%	\centering
%		\caption{Bootstrap Timing in seconds, and amortized values by $\log_2(t)$}
%	\label{tbl:timings}
%	\begin{tabular}{c || c | c || c }
%		\hline
%		Set & Shift based bootstrapping & $\Shift$ & \parbox{3.5cm}{\centering TFHE/GINX Bootstrap\\in $\ZZ_2$}  \\
%		\hline 
%		1 ($t=16$) & $5.9$ ($1.4$) & $0.24$ ($0.06$) & $0.023$  \\
%		2 ($t=16$) & $51.4$ ($12.85$) & $2.0$ ($0.5$) & $0.10$  \\
%		3 ($t=32$) & $472.3$ ($94.4$)  & $2.0$ ($0.4$) & $0.22$ \\
%		\hline
%	\end{tabular}
%\end{table}

\begin{table}
	\setlength{\tabcolsep}{6pt}
	\centering
	\caption{Bootstrap Timing in seconds, and amortized values by $\log_2(t)$}
	\label{tbl:timings}
	\begin{tabular}{c || c | c | c | c || c }
		\hline
		Set & \multicolumn{2}{c|}{Shift based bootstrapping} & \multicolumn{2}{c||}{$\Shift$} & \parbox{3.5cm}{\centering TFHE/GINX \\Bootstrap in $\ZZ_2$}  \\
		\hline 
		& CPU & GPU & CPU & GPU & \\
		1 ($t=16$) & $5.9$ ($1.4$) & $0.066$ ($0.0165$) & $0.24$ ($0.06$) & $1.0\cdot10^{-3} (2.5 \cdot 10^{-5})$ & $0.023$  \\
		2 ($t=16$) & $51.4$ ($12.85$) & $1.2$ ($0.3$) & $2.0$ ($0.5$) & $2.6\cdot10^{-3}$ ($6.5\cdot10^{-4}$) & $0.10$  \\
		3 ($t=32$) & $472.3$ ($94.4$)  & $4.1$ ($0.82$) & $2.0$ ($0.4$) & $4.3\cdot10^{-3}$ ($8.6\cdot10^{-4}$ ) & $0.22$ \\
		\hline
	\end{tabular}
\end{table}

%TODO in progress from here on

%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{0.49\textwidth}
%		\includegraphics[width=\textwidth]{graphics/nimpact}
%	\end{minipage}\begin{minipage}{0.49\textwidth}
%		\includegraphics[width=\textwidth]{graphics/Nimpact}
%	\end{minipage}
%
%\caption{Effect of larger $\LWE$ dimension and ring order, and decomposition base of the packing key}
%\label{fig:impact}
%\end{figure}


%To conclude this discussion, we analyse how altering other parameters affects the timing of our bootstrapping procedure. To this
%end we fix the first parameter set and vary the $\LWE$ dimension $n$ and the order $N$ of the Ring. The results are depicted in %Figure~\ref{fig:impact}. As predicted by Subsection~\ref{ssec:theo-eval}, an increase the LWE dimensions seems to only have a linear impact on the %execution time, as can be expected since it only determines the number of iterations required by the bootstrapping algorithm.


==> sections/long-integer-operations.tex <==
 
 
  
With previous bit-based fully homomorphic schemes such as TFHE or FHEW, one could emulate integers by using their binary representation and by storing each bit within an individual ciphertext. In
the context of our new bootstrapping technique, we can apply a similar reasoning to extend the range of integer far beyond our original message space.

Note that the bootstrap operation we rely on here is the half domain bootstrap from Section~\ref{sec:applications}.  Let us instantiate our scheme with appropriate parameters and let $t = 2^k, k = 1 \pmod{2}$ be the original message space and set $\digspace = \sqrt{\frac{t}{2}}$.  Long integers $\LongInteger = \LIDigit{LI}_{r}...\LIDigit{LI}_1$  are simply represented as a list of $r$ LWE ciphertexts $\LIDigit{LI}_i, i \in [r]$
with  $\LIDigit{LI}_i = \LWE_{\errDist_{\bound}, n, q}(\Delta_{q,t}\cdot d_i), d_i \in \ZZ_{\digspace}$. 
We start by describing our addition procedures:

\begin{definition}[Long Integer Addition]
	The addition of two long integers requires the definition of two subroutines $\DigitHalfAdd$ and $\FullAdd$, which are analogous to the half and full adders in the binary setting:
	\label{dnf:dha}
	\begin{description}
		\item[$\DigitHalfAdd(\ct,\ct')$] Takes as an input two digits $\ct,\ct' \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\cdot)$ and outputs the sum $\ctvar{res}$ and the output carry $\ctvar{c}_{out}$
		\begin{enumerate}
			\item Set $\ctvar{s} \exec \ct + \ct'$
			\item Let $f(x) = \begin{cases}
			1, &\text{if } x \geq \digspace\\
			0, &\text{ else }
			\end{cases}$
			\item Construct  $\preRotPoly_{0}, \preRotPoly_{1} \exec \ConstPoly(f, \deg)$
			\item Run $\ctvar{c}_{out} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{s}, \preRotPoly_{0}, \preRotPoly_{1},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Set $\ctvar{res} \exec \ctvar{s} - \ctvar{c}_{out} \cdot \digspace$
			\item Output $\ctvar{res},\ctvar{c}_{out}$
		\end{enumerate}
	\end{description}
	\label{dnf:dfa}
	\begin{description}
		\item[$\FullAdd(\ct,\ct',\ctvar{c}_{in})$] Takes as an input two digits $\ct,\ct' \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\cdot)$ and the input carry $\ctvar{c}_{in}$ and outputs the sum $\ctvar{res}$ and the output carry $\ctvar{c}_{out}$
		\begin{enumerate}
			\item Run $\ctvar{s}, \ctvar{c} \exec \DigitHalfAdd(\ct, \ct')$
			\item Run $\ctvar{res}, \ctvar{c}' \exec \DigitHalfAdd(\ctvar{s}, \ctvar{c}_{in})$
			\item Let $\ctvar{c}_{out} \exec \ctvar{c} + \ctvar{c}'$
			\item Output $\ctvar{res},\ctvar{c}_{out}$
		\end{enumerate}
	\end{description}
	The addition of two $r$-digit long integers is then defined by the following algorithm.
	\label{dnf:rbitadder}
	\begin{description}
		\item[$\LongAdd(\LongInteger, \LongInteger')$] Takes as an input two $r$-digit long integers $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1$ ,$\LongInteger' =\LIDigit{LI}'_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ and outputs a long integer $\LongIntegerA{S} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ representing the sum of the two inputs.
		\begin{enumerate}
			\item Set $\LongIntegerA{S} = \LIDigit{S}_r,...,\LIDigit{S}_1$ with $\vec{S}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Set $\ctvar{c}_{in} = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item For $i=1$ to $r$ do \begin{enumerate}
				\item Run $ \ctvar{t},\ctvar{c}_{out} \exec \FullAdd(\LIDigit{LI}_i,\LIDigit{LI}'_i,\ctvar{c}_{in})$
				\item Set $\LIDigit{S}_i = \ctvar{t}$
				\item Set $\ctvar{c}_{in} = \ctvar{c}_{out}$
			\end{enumerate}
			\item Output $\LongIntegerA{S}$
		\end{enumerate}
	\end{description}
\end{definition}

Correctness follows quickly. If the sum in $\DigitHalfAdd$ overflows, the bootstrap operation correctly computes the
carry, while the fifth step shifts the sum back into the appropriate slots. Then, the remaining algorithm follows. We note that the scaling
by $\digspace$ in Step 5 of $\DigitHalfAdd$ may induce a lot of noise. To prevent damaging the plaintext, the ciphertext should be scaled during bootstrapping,
either by scaling the sample before modulus switching or by using a functional keyswitch as in \cite{AC:CGGI17}.

While not as easily as in a binary setting, we can define the subtraction algorithm in a similar manner.
\begin{definition}[Long Integer Subtraction]
	Analogously to the case of addition, we first define a half and full subtractor, $\DigitHalfSub$ and $\FullSub$.
	\label{dnf:dhs}
	\begin{description}
		\item[$\DigitHalfSub(\ct,\ct')$] Takes as an input two digits $\ct,\ct' \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\cdot)$ and outputs the difference $\ctvar{res}$ and the output carry $\ctvar{c}_{out}$
		\begin{enumerate}
			\item Set $\ctvar{s} \exec \ct \cdot \digspace + \ct'$
			\item Let $f(a \cdot \digspace + b) = \begin{cases}
			1, &\text{ if } b > a\\
			0, &\text{ else }
			\end{cases}$
			\item Construct  $\preRotPoly_{0}, \preRotPoly_{1} \exec \ConstPoly(f, \deg)$
			\item Run $\ctvar{c}_{out} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{s}, \preRotPoly_{0}, \preRotPoly_{1},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Set $\ctvar{res} \exec \ctvar{c}_{out} \cdot \digspace + \ct - \ct'$
			\item Output $\ctvar{res},\ctvar{c}_{out}$
		\end{enumerate}
	\end{description}
	\label{dnf:dfs}
	\begin{description}
		\item[$\FullSub(\ct,\ct',\ctvar{c}_{in})$] Takes as an input two digits $\ct,\ct' \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\cdot)$ and the input carry $\ctvar{c}_{in}$ and outputs the difference $\ctvar{res}$ and the output carry $\ctvar{c}_{out}$
		\begin{enumerate}
			\item Run $\ctvar{d}, \ctvar{c} \exec \DigitHalfAdd(\ct', \ctvar{c}_{in})$
			\item Run $\ctvar{res}, \ctvar{c}' \exec \DigitHalfSub(\ct, \ctvar{d})$
			\item Let $\ctvar{c}_{out} \exec \ctvar{c} + \ctvar{c}'$
			\item Output $\ctvar{res},\ctvar{c}_{out}$
		\end{enumerate}
	\end{description}
	Then, the subtraction of two long integers $\LongSub$ is achieved by chaining $\FullSub$ operations.
	\label{dnf:rbitsubber}
	\begin{description}
		\item[$\LongSub(\LongInteger, \LongInteger')$] Takes as an input two $r$-digit long integers $\LongInteger=\LIDigit{LI}_r...\LIDigit{LI}_1,\LongInteger' = \LIDigit{LI}'_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ and outputs a long integer $\LongIntegerA{S} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ representing the sum of the two inputs.
		\begin{enumerate}
			\item Set $\LongIntegerA{S} = \LIDigit{S}_r...\LIDigit{S}_1$ with $\LIDigit{S}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Set $\ctvar{c}_{in} = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item For $i=1$ to $r$ do \begin{enumerate}
				\item Run $ \ctvar{t},\ctvar{c}_{out} \exec \FullSub(\LIDigit{LI}_i,\LIDigit{LI}'_i,\ctvar{c}_{in})$
				\item Set $\LIDigit{S}_i \exec \ctvar{t}$
				\item Set $\ctvar{c}_{in} \exec \ctvar{c}_{out}$
			\end{enumerate}
			\item Output $\LongIntegerA{S}$
		\end{enumerate}
	\end{description}
\end{definition}

Here, correctness follows by how $\DigitHalfSub$ and $\FullSub$ are defined. The former first computes the carry  by comparing two digits, and accordingly perform subtraction modulus $\digspace$. The latter, adds the input carry to the digit to subtract using $\DigitHalfAdd$, and then performs the actual subtraction. At most one output carry can be one, and the sum of both is then the output carry.

For the long integer multiplication, we start by describing a (left) shift operation on long integers. We note
that in practice, an equivalent operation can be achieved by appropriate indexing.
\begin{definition}[Long Integer Left Shift]
	The procedure to shift a long integer to the left $\LILeftShift$ is defined as follows:
	\label{dfn:lshift}
	\begin{description}
		\item[$\LILeftShift(\LongInteger, v)$] Takes as an input a long integer $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ and a number $v \in \NN$. Outputs a long integer $\LongIntegerA{S} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r $ which contains $\LongInteger$ shifted to the left by $v$ digits. The result is truncated to $r$ digits.
		\begin{enumerate}
			\item Set $\LongIntegerA{S} = \LIDigit{S}_r...\LIDigit{S}_1$ with $\LIDigit{S}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item For $i = v$ to $r$ \begin{enumerate}
				\item Set $\LIDigit{S}_i = \LIDigit{LI}_{i - v}$
			\end{enumerate}
			\item Output $\LongIntegerA{S}$
		\end{enumerate}
	\end{description}
\end{definition}  

Now, we show how to compute the product long integers in two steps. First we describe two subroutines, one to 
multiply two digits, another to multiply a digit and a long integer. Then utilize them together with $\LILeftShift$
to compute the product of two $r$-digit long integers.

\begin{definition}[Long Integer Multiplication]
	The product $\SmallProduct$ of two digits is achieved as follows:
	\label{dfn:smallprod}
	\begin{description}
		\item[$\FullProd(\ct,\ct')$] Takes as input two ciphertexts $\ct_a \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\msg), \ct_b \in \LWE_{\errDist_{\bound}, n, q}(\vec{s},\msg')$  and outputs two LWE ciphertext $\ctvar{hi} = \LWE_{\errDist_{\bound}, n, q}(\vec{s},\msg_{hi})$,$\ctvar{lo} = \LWE_{\errDist_{\bound}, n, q}(\vec{s},\msg_{lo})$ such that $\msg \cdot \msg' = \msg_{hi} \cdot \digspace + \msg_{lo}$
		\begin{enumerate}
			\item Define $f_{hi}(a \cdot \digspace + b) = \left\lfloor \frac{ab}{\digspace} \right\rfloor$
			\item Define $f_{lo}(a \cdot \digspace + b) = ab - \left\lfloor \frac{ab}{\digspace} \right\rfloor \cdot \digspace$
			\item Construct $\preRotPoly_{0,hi}, \preRotPoly_{1,hi} \exec \ConstPoly(f_{hi}, \deg)$
			\item Construct $\preRotPoly_{0,lo}, \preRotPoly_{1,lo} \exec \ConstPoly(f_{lo},\deg)$
			\item Set $\ctvar{c} \exec \ct \cdot \digspace + \ct'$
			\item Run $\ctvar{hi} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{c}, \preRotPoly_{0, hi}, \preRotPoly_{1, hi},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Run $\ctvar{lo} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{s}, \preRotPoly_{0, lo}, \preRotPoly_{1, lo},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Output $\ctvar{hi},\ctvar{lo}$
		\end{enumerate}
	\end{description}
	Then we can multiply a long integer and a digit by the following procedure $\LIDigitProd$:
	\label{dfn:longdigit}
	\begin{description}
		\item[$\LIDigitProd( \LongInteger, \ct)$] Takes as a input a long integer $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ and a digit $\ct \in \LWE_{\bound, n, q}(\vec{s}, \cdot)$. Outputs a long integer $\LongIntegerA{P} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ and 
		a digit ciphertext $\ctvar{hi} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)$ such that $\ctvar{hi} || \LIDigit{P}_r,...,\LIDigit{P}_1$ contains the product of $\LongInteger$ and $\ct$
		\begin{enumerate}
			\item Set $\LongIntegerA{P} = \LIDigit{P}_r...\LIDigit{P}_1$ with $\LIDigit{P}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Set $\ctvar{c} = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Run $\ctvar{hi},\ctvar{lo} \exec \FullProd(\LIDigit{LI}_1, \ct)$
			\item $\LIDigit{P}_1 = \ctvar{lo}$
			\item For $i=2$ to $r$ \begin{enumerate}
				\item Run $\ctvar{hi'}, \ctvar{lo} \exec \FullProd(\LIDigit{LI}_i, \ct)$
				\item Run $\ctvar{r}, \ctvar{c'} \exec \FullAdd(\ctvar{hi}, \ctvar{lo}, \ctvar{c})$
				\item Set $\LIDigit{P}_i = \ctvar{r}$
				\item Set $\ctvar{hi} = \ctvar{hi'}$ 
				\item Set $\ctvar{c} = \ctvar{c'}$
			\end{enumerate}
			\item Output $\LongIntegerA{P}, \ctvar{hi}$
		\end{enumerate}
	\end{description}
	Finally, we describe the (truncated) product $\LIMult$ of two long integers:
	\label{dfn:longmult}
	\begin{description}
		\item[$\LIMult(\LongInteger, \LongInteger')$] takes as input two long integer $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$, $\LongInteger' = \LIDigit{LI'}_r...\LIDigit{LI'}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$.
		Outputs a long integer $\LongIntegerA{M} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$ containing the $r$ low order digits of the $r \times r$-digit product of $\LongInteger$ and $\LongInteger'$
		\begin{enumerate}
			\item Set $\LongIntegerA{M} = \LIDigit{M}_r...\LIDigit{M}_1$ with $\LIDigit{M}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item For $i=1$ to $r$ \begin{enumerate}
				\item Run $\LongIntegerA{T}, \text{\textunderscore} \exec \LIDigitProd(\LongInteger, \LIDigit{LI'}_i)$
				\item Run $\LongIntegerA{S} \exec \LILeftShift(\LongIntegerA{T}, i)$
				\item Run $\LongIntegerA{M} \exec \LongAdd(\LongIntegerA{M}, \LongIntegerA{S})$
			\end{enumerate}
			\item Output $\LongIntegerA{M}$
		\end{enumerate}
	\end{description}
\end{definition}
Under the constraints specified, $\ctvar{c}$ in step 5 of $\SmallProduct$ is unique and correctness follows. 

To conclude this part of the supplementary material, we show how to compute the remainder and quotient of
a pair of long integer by describing a homomorphic variant of long division. We start by defining three subroutines.

\begin{definition}[Long Integer IsLessEqual]
	We describe the process to compare two long integers:
	\label{dfn:greater}
	\begin{description}
		\item[$\LILessEq(\LongInteger,\LongInteger')$] takes as an input two long integers $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$, $\LongInteger' = \LIDigit{LI'}_r...\LIDigit{LI'}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$.
		Outputs a LWE digit $\ctvar{le} \in \LWE_{\bound, n, q}(\vec{s}, b \cdot \Delta_{q, t} ), b \in \BB $, with $b = 1$ when $\LongInteger \leq \LongInteger'$ and $0$ otherwise.
		\begin{enumerate}
			\item Define $f(a \cdot \rho + b) = \begin{cases} 
			0, & \text{ if } a = b\\
			1, & \text{ if } a > b\\
			2, & \text{ else }\\
			\end{cases}$
			\item Define $g(a \cdot \sqrt{\frac{t}{2}} + b) = \begin{cases}
			b\cdot \rho, &\text{ if } a = 0\\
			a\cdot \rho, &\text{else}
			\end{cases}$
			\item Compute $\preRotPoly_{0,f}, \preRotPoly_{1,f} \exec \ConstPoly(f, \deg)$ and $\preRotPoly_{0,g}, \preRotPoly_{1,g} \exec \ConstPoly(g, \deg)$ 
			\item Set $\ctvar{p} = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item For $i=r$ to $1$ \begin{enumerate}
				\item Compute $\ctvar{d} \exec \LIDigit{LI}_i \cdot \rho + \LIDigit{LI'}_i$
				\item Run $\ctvar{c} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{d}, \preRotPoly_{0,f}, \preRotPoly_{1,f},  \basis_{\boot}, \packKey, \keySwitchKey)$
				\item Compute $\ctvar{t} \exec \ctvar{c} + \ctvar{p}$
				\item Compute $\ctvar{p} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{t}, \preRotPoly_{0,g}, \preRotPoly_{1,g},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\end{enumerate}
			\item Define $h(x) = \begin{cases}
			1, &\text{ if } x = 2 \rho \lor x = 0\\
			0, &\text{ else }
			\end{cases}$
			\item Construct $\preRotPoly_{0,h}, \preRotPoly_{1,h} \exec \ConstPoly(h, \deg)$ 
			\item Run $\ctvar{le} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{p}, \preRotPoly_{0,h}, \preRotPoly_{1,h},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Output $\ctvar{le}$
		
		\end{enumerate}
	\end{description}
	
\end{definition}

At a high level, we compare long integers by first packing two digits into a single half-domain ciphertext. Then $f$ is used the determine the relation between the digits, and $g$ is used to propagate it from highest to lowest order digit. Finally $h$
maps the result of the comparison to $\BB$. Next, we define a long integer variant of the MUX gate.

\begin{definition}[Long Integer Mux]
	\label{dfn:imux}
	\begin{description} 
		\item[$\LIMux(\ct, \LongInteger, \LongInteger')$] Takes as input a LWE ciphertext $\ct \in \LWE_{\bound, n, q}(\vec{s}, b \; \cdot \Delta_{q, t} ), b \in \BB$ and two long integers $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$,$\LongInteger' = \LIDigit{LI'}_r...\LIDigit{LI'}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$. Outputs $\LongIntegerA{R} = \LongInteger$ when $b = 1$ and $\LongIntegerA{R} = \LongInteger'$ otherwise.
		\begin{enumerate}
			\item Set $\LongIntegerA{R} = \LIDigit{R}_r...\LIDigit{R}_1$ with $\LIDigit{R}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Set $\overline{\ct} = \LWE_{\bound, n, q}(\vec{s}, \Delta_{q, t}) - \ct$
			\item Let $f(2 \cdot a + b) = \begin{cases}
			a, & \text{ if } b = 1\\
			0, &\text{ else }
			\end{cases}$
			\item Construct $\preRotPoly_{0,f}, \preRotPoly_{1,f} \exec \ConstPoly(f, \deg)$
			\item For $i = 1$ to $r$ \begin{enumerate}
				\item Compute $\ctvar{p} \exec 2 \cdot \LIDigit{LI}_i + \ct$
				\item Compute $\ctvar{n} \exec 2 \cdot \LIDigit{LI}'_i + \overline{\ct}$
				\item Run $\ctvar{p'} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{p}, \preRotPoly_{0,f}, \preRotPoly_{1,f},  \basis_{\boot}, \packKey, \keySwitchKey)$
				\item Run $\ctvar{n'} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{n}, \preRotPoly_{0,f}, \preRotPoly_{1,f},  \basis_{\boot}, \packKey, \keySwitchKey)$
				\item Set $\LIDigit{R}_i = p' + n'$
			\end{enumerate}
		\item Output $\LongIntegerA{R}$
		\end{enumerate}
	\end{description}
\end{definition}
Here, $\overline{\ct}$ acts as the complement of $\ct$. Then at most one of two values in step 5.5, can be non-zero and 
correctness follows.
Alternatively, if we are willing to sacrifice performs for simplicity, step 4 can be replaced by two $\LIDigitProd$ operations and by using the identity $$f(b,\ctvar{A},\ctvar{B}) = b\ctvar{A} + (1 - b)\ctvar{B} = \begin{cases}
A, &\text{if } b = 1\\
B, &\text{if } b = 0
\end{cases}$$ 

The purpose of next subroutine may be difficult to understand at first glance. It is used to detect whether the result $(\LongInteger, \ct)$ of a $\LIDigitProd$, shifted by $v$ digits, fits within a $r$-digit
long integer.

\begin{definition}[Long Integer Shift Overflow Detection]
	Overflow detection is achieved by the following procedure $\LIOverflow$:
	\label{dfn:detectOverflow}
	\begin{description}
		\item[$\LIOverflow(\LongInteger, \ct, v)$] Takes as input a long integer $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$, a LWE ciphertext $\ct \in \LWE_{\bound, n, q}(\vec{s}, d)$ and a shift amount $v$.
		Outputs a LWE ciphertext $\ctvar{o} \in \LWE_{\bound, n, q}(\vec{s}, \Delta_{Q, t} b), b \in \BB$, with $b=0$ when $d > 0$ or when $\LILeftShift(\LongInteger, v)$ would overflow non-zero terms
		\begin{enumerate}
			\item Define $f(x) = [x > 0]$ and $\preRotPoly_{0,f}, \preRotPoly_{1,f} \exec \ConstPoly(f,\deg)$
			\item Define $g(x) = [x = 0]$ and $\preRotPoly_{0,g}, \preRotPoly_{1,g} \exec \ConstPoly(f,\deg)$
			\item Run $\ctvar{p} \exec \Bootstrap(\brKey, \brKey_{F}, \vec{u}, \ct, \preRotPoly_{0,f}, \preRotPoly_{1,f},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item For $i=r$ to $r - (v - 1)$ \begin{enumerate}
				\item Run $\ctvar{o} \exec \Bootstrap(\brKey,  \vec{u}, \LIDigit{LI}_r, \preRotPoly_{0,f}, \preRotPoly_{1,f},  \basis_{\boot}, \packKey, \keySwitchKey)$
				\item Compute $\ctvar{p} \exec \ctvar{p} + \ctvar{o}$
			\end{enumerate}
			\item Run $\ctvar{o} \exec \Bootstrap(\brKey, \vec{u}, \ctvar{p}, \preRotPoly_{0,g}, \preRotPoly_{1,g},  \basis_{\boot}, \packKey, \keySwitchKey)$
			\item Output $\ctvar{o}$
		\end{enumerate}
	\end{description}
\end{definition}
We are finally able to define the combined division-modular reduction method $\LIDivMod$:
\begin{definition}[Long Integer Division and Remainder]
	\label{dfn:longdiv}
	\begin{description}
		\item[$\LIDivMod(\LongInteger,\LongInteger')$] takes as input two long integers $\LongInteger = \LIDigit{LI}_r...\LIDigit{LI}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$,$\LongInteger' = \LIDigit{LI'}_r...\LIDigit{LI'}_1 \in \LWE_{\bound, n, q}(\vec{s}, \cdot)^r$.
		Outputs two long integer $\LongIntegerA{Quot}$ and $\LongIntegerA{Mod}$ which contain the quotient and modulus respectively.
		\begin{enumerate}
			\item Set $\LongIntegerA{Quot} = \LIDigit{Quot}_r...\LIDigit{Quot}_1$ with $\LIDigit{Quot}_i = \LWE_{\bound, n, q}(\vec{s}, 0)$
			\item Set $\LongIntegerA{Mod} = \LongInteger$
			\item Let $\LongIntegerA{Pdig} = \LongIntegerA{Pdig}_{\frac{k-1}{2}},...,\LongIntegerA{Pdig}_1$ be a list of long integers with $k-1$ slots and $\ctvar{Phi} = \ctvar{phi}_{\frac{k-1}{2}},...,\ctvar{phi}_1 $ be a list of long integer \textit{digits} with $\frac{k-1}{2}$ slots.
			\item For $i=0$ to $\frac{k-1}{2}-1$ \begin{enumerate}
				\item Let $\ctvar{po2} \in \LWE_{\bound, n, q}(\vec{s}, \cdot)$ be a trivial LWE sample containing $\Delta_{q, t} \cdot 2^i$
				\item Run $\LongIntegerA{T}, \ctvar{hi} \exec \LIDigitProd(\LongInteger', \ctvar{po2})$
				\item Set $\LongIntegerA{Pdig}_{i+1} = \LongIntegerA{T}$ and $\ctvar{phi}_{i+1} = \ctvar{hi}$
			\end{enumerate}
			\item For $v = r - 1$ to $0$ \begin{enumerate}
				\item For $u = \frac{k - 1}{2} - 1$ to $0$ \begin{enumerate}
					\item Let $\LongIntegerA{Pow}$ be a long integer storing $2^{v (\frac{k-1}{2}) + u}$
					\item Run $\ctvar{ovf} \exec \LIOverflow(\LongIntegerA{Pdig}_{u+1}, \ctvar{phi}_{u+1}, v)$ 
					\item Run $\LongIntegerA{S} \exec \LILeftShift(\LongIntegerA{Pdig}_{u+1}, v)$
					\item Run $\ctvar{le} \exec \LILessEq(\LongIntegerA{S},\LongIntegerA{Mod})$
					\item Run $ \text{\textunderscore}, \ctvar{toggle} \exec \SmallProduct(\ctvar{le},\ctvar{ovf})$
					\item Run $\LongIntegerA{Dif} \exec \LongSub(\LongIntegerA{Mod}, \LongIntegerA{S})$
					\item Run $\LongIntegerA{Sum} \exec \LongAdd(\LongIntegerA{Quot}, \LongIntegerA{Pow})$
					\item Run $\LongIntegerA{Mod} \exec \LIMux(\ctvar{toggle}, \LongIntegerA{Dif}, \LongIntegerA{Mod})$
					\item Run $\LongIntegerA{Quot} \exec \LIMux(\ctvar{toggle}, \LongIntegerA{Sum}, \LongIntegerA{Quot})$
				\end{enumerate}
			\end{enumerate}
			\item Output $\LongIntegerA{Quot}, \LongIntegerA{Mod}$
	\end{enumerate}
	\end{description}
\end{definition}




\begin{table} 
	\centering
	\caption{Number of bootstrapping operations per long integer operation}
		\label{tbl:bsperop}
	\begin{tabular}{ c | c | c}
		& Operation & Bootstraps  \\
		\hline
		1 & \textit{DigitHalfAdder} & $1$ \\
		2 & \textit{DigitHalfSubber} & $1$ \\
		3 & \textit{DigitFullAdder} & $2$ \\
		4 & \textit{DigitFullSubber} & $2$ \\
		5 & \textit{LongAdd} & $2r$  \\
		6 & \textit{LongSub} & $2r$  \\
		7 & \textit{FullProduct} & $2$  \\
		8 & \textit{LongDigitProduct} & $ 4 \, r - 2 $  \\
		9 &\textit{LongLeftShift} & $0$ \\
		10 & \textit{LongMultiplication} & $6 \, r^{2} - 2 \, r$\\
		11 & \textit{IsLessEq} & $2 \, r + 1$ \\
		12 & \textit{LongMux} & $2 \, r$  \\
		13 & \textit{DetectNoOverflow} & $v + 2$ \\
		14 &\textit{LongDivMod} & $\frac{21}{4} \, {\left(k - 1\right)} r^{2} + \frac{17}{4} \, {\left(k - 1\right)} r - k + 1$ 
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{Number of bootstrapping operations per equivalent binary integer operation to the methods in Table~\ref{tbl:bsperop}}
		\label{tbl:bsperopbin}
	\begin{tabular}{c | c | c }
		& Equivalent operation & Bootstraps \\
		\hline
		 1 & Half-Adder & $2$\\
		 2 & Half-Subtractor & $2$\\
		 3 & Full-Adder & $5$\\
		 4 & Full-Subtractor & $5$\\
		 5 & $r(\frac{k-1}{2})$-bit Adder & $\frac{5}{2} \, {\left(k - 1\right)} r$ \\
		 6 & $r(\frac{k-1}{2})$-bit Subtractor & $\frac{5}{2} \, {\left(k - 1\right)} r$ \\
		 7 & $\frac{k-1}{2}$-bit Sequential Multiplier & $\frac{11}{4} \, k^{2} - \frac{21}{2} \, k + \frac{31}{4}$\\
		 8 & $(\frac{k-1}{2}) \times r (\frac{k-1}{2})$ Sequential Multiplier & $\frac{1}{2} \, {\left(3 \, k^{2} - 11 \, k + 8\right)} r + \frac{5}{4} \left(k-1\right)\left(k-3\right)$ \\
		 9 & Left Shift by a multiple of $k-1$ & $0$\\
		 10 & $r(\frac{k-1}{2})$-bit Sequential Multiplier & $\frac{11}{8} \, {\left(k^{2} - 2 \, k + 1\right)} r^{2} + \frac{1}{4} \, {\left(k - 1\right)} r$\\
		 11 & $r(\frac{k-1}{2})$-bit Comparator & $\frac{5}{2} \, {\left(k - 1\right)} r - 3$\\
		 12 & $1$ to $r(\frac{k-1}{2})$-bit MUX & $\frac{3}{2} \, {\left(k - 1\right)} r$ \\
		 13 & Chained OR gates & $v(\frac{k-1}{2}) + O(k)$ \\
		 14 & $r(\frac{k-1}{2})$-bit combined division and modular reduction& $\frac{45}{8} \, {\left(k^{2} - 2 \, k + 1\right)} r^{2} - \frac{5}{4} \, {\left(k - 1\right)} r$
	\end{tabular}
\end{table}



From a high level Definition~\ref{dfn:longdiv} describes a homomorphic variant of the long division. Initially, using $\LIDigitProd$, we compute all products of the divisor $\LongInteger'$ and the powers of 2 which fit into a single digit. Every other power which fits
into a $r$-digit long integer can then be computed through shifting. Then, going from the largest to the lowest power of 2, we subtract the product of the current power and the divisor from the remainder (initialized with the dividend), provided that the current product
fits into a $r$-bit long integer and given that it is smaller than the current remainder. Analogously, we add the current power of two to the quotient.

In order to compare our approach to previous binary schemes, we show the amount of bootstrapping operations of our long integer based approach and of equivalent operations implemented using binary numbers, in Table~\ref{tbl:bsperop} and Table~\ref{tbl:bsperopbin} respectively. 
We observe that the amount of bootstraps in the case of long integers is in most parts independent of the digit message space We note that in case of the binary schemes, NOT gates do not require any bootstrapping. Moreover, in both cases, some operations can be optimized depending on the setting. Per example, the binary equivalent of the $\LIDigitProd$ may be replaced
by multiple AND gates, provided that one side encrypts a binary value.


 
%\subsection{Applications to Discretized Neural Networks.}\label{sec:application-discretized-neural-network}
% 
%In this section, we discuss how to utilize our bootstrapping 
%procedure to evaluate neural networks.
%
%	 A neural network is a function $f^{\ast}:\RR^{\lwidth{1}} \mapsto \RR^{\lwidth{n}}$   which approximates a function $f:\RR^{\lwidth{1}} \mapsto \RR^{\lwidth{n}}$. 
%	That is given an approximation factor $\epsilon > 0$ we have that
%	for all $x \in \RR^{\lwidth{1}}$ 
%	it holds that $|f^{\ast}(x) - f| \leq \epsilon$.  
%	Furthermore, a neural network can be represented as a circuit of bounded fan-in, where
%	the gates of the circuit are defined by the a function 
%	$g_f(\vec{x}) = \psi(\sum_{i=1}^m \vec{w}_f[i] \cdot \vec{x}[i] + b_f)$
%	where $\vec{x} \in \RR^m$, $\vec{w} \in \RR^m$ is called the weight vector, $b_f \in \RR$ the bias and
%	$\phi:\RR \mapsto \RR$ is a non-linear activation function. Finally, we call gates of a neural network neurons.
%
% 
%In Table~\ref{tbl:act} we show popular choices for activation functions according to \cite{nwankpa2018activation}. 
% As we base our work on schemes that do not trivially support floating-point operations, we focus on neural networks with integer coefficients. 
%%TODO Ask Leo about this sentence 
% In the past, it has been demonstrated that neural networks with fixed precision perform similarly to their floating-point counterpart according to \cite{wu2018training,861451,10.5555/3045118.3045303}. 
% Moreover, one can easily transition from a floating-to a fixed point model. For example, Bourse et al. \cite{C:BMMP18} transforms the neural network by rounding each coefficient to the closest multiple of a chosen parameter and  Dowlin et al. \cite{10.5555/3045390.3045413} scales each coefficient by a fixed factor. In both cases, the authors report only a small drop in accuracy. 
% 
% A major difficulty in oblivious evaluation of neural networks is the computation of activation functions, as in most cases, they cannot be represented accurately by (finite) polynomials. Prior works presented many ways to circumvent these issues. For example 
%in  \cite{NIPS2019_9194,ACM:CGHPS18} the outputs rely on binary representations of integers and
%in \cite{C:BMMP18,10.5555/3045390.3045413} the authors use uncommon activation functions namely $\sig$ and $x^2$. Additionally, Boura et al. \cite{boura2018chimera} demonstrates a way to evaluate arbitrary negacyclic functions. 
%Such solutions introduce some shortcomings, however; alternative representations of integers require additional computations and
% may degrade the efficiency, and non-standard activation functions can restrict the class of functions, which can be approximated by neural networks \cite{leshno1993multilayer}.
% \begin{table}
% 	\centering
% 		\setlength{\tabcolsep}{7pt}
% 	\begin{tabular}{ c | c }
% 		\hline
% 		\textbf{Name} & \textbf{Formula}\\
% 		\hline 
% 		Rectified Linear Unit & $\mathsf{ReLu}(x) = \max\{0,x\}$\\[0.1cm]
% 		Sigmoid & $\mathsf{S}(x) = \frac{1}{1 + e^{-x}}$ \\[0.1cm]
% 		Hyperbolic Tangent & $\mathsf{tanh}(x) = \frac{e^{x} - e^{-x}}{e^{x} + e^{-x}}$\\[0.1cm]
% 		Softmax & $\mathsf{\sigmoid}(\vec{x}_i) = \frac{e^{\vec{x}_i}}{\sum_{j=1}^{\lwidth{i+1}} e^{\vec{x}_j}}$\\
% 		
% 		\hline
% 	\end{tabular}
% 	\caption{Popular choices for activation functions according to \cite{nwankpa2018activation}}
% 	\label{tbl:act}
% \end{table}
%Besides the requirement for a discrete network, our bootstrapping technique removes the need for any adaptations. The evaluation of a complete neural network with univariate activation functions using our proposed bootstrapping method is defined inductively over the evaluation of a single neuron.
% 
% We note that there are other activation functions or specialized neural networks that utilize multiple ciphertexts. 
% However, our bootstrapping technique will be able to handle such constructs as long as such functions can be decomposed into univariate maps. For instance, convolutional neural networks rely on pooling operations, which may compute the maximum of several values. By using
% the identity from the previous section, $\max(x, y) = \max(x-y,0) + y$, we are still  able to compute the result.
%

%TODO Comented out for space reasons
%\begin{definition}[Oblivious Evaluation of a Single Neuron]
%	\label{def:eval-nn}
%	\begin{description}
%		\item[$\EvalNeuron(\rKey, \vec{v}, \vec{w}, B, \phi)$]  
%Takes as input a bootstrapping key generated as in theorem \ref{thm:bootstrapping-pre-rotation}, a vector
%of LWE samples $\vec{v} \in \LWE_{\errDist_{\vec{v}}, n, q}(\vec{s}, .)^{m}$, a vector $\vec{w} \in \ZZ_q^m$ of weights,
%a vector bias $B \in \ZZ_q$ and an activation function $\phi$. 
%		\begin{enumerate}
%			\item Set $\BootsFunction$ such that for all $x \in \ZZ_q$ we have $\BootsFunction(x) = \phi(x)$.
%			\item Set $\preRotPoly \exec \ConstPoly(\BootsFunction, t, q, Q, N, \bound_{\ct})$ 
%			\item For $ j = 1 $ to $j = \lwidth{i+1}$ do,
%			\item Compute $\ct_{\out} \exec \sum_{i=1}^m \vec{w}[i] \cdot \vec{v}[i]$.
%			\item Output $\ct_{\out}$.
%		\end{enumerate} 
%	\end{description}
%\end{definition}


 

==> sections/lwe-estimator-scripts.tex <==

We evaluated security of our parameter sets via the following script for the LWE estimator \cite{albrecht2015concrete}.
In the example below we run the estimator as for the LWE samples in our parameter set 1.


\lstset{language=Python}

\begin{lstlisting}
sage: N = 704
sage: Q = 2**(56) - 286719
sage: stddev = float(2**(32))
sage: h = 64
sage: alpha = alphaf(sigmaf(stddev), Q)
sage: set_verbose(1)
sage: _ = estimate_lwe(
      N, 
      alpha, 
      Q, 
      secret_distribution=((0,1), h), 
      reduction_cost_model=BKZ.sieve)
\end{lstlisting}


 
In case no restrictions on the Hamming weight or distribution are given (e.g., in case of our RLWE parameters), 
we omit the \texttt{secret\_distribution} argument. 
%Note that for the LWE samples we set the modulus $q$ instead of $Q$, and the dimension $n$ instead of $N$. 
%But we stress that the change is only notational. 
The code to run the sparse LWE estimator  \cite{EPRINT:CheSonYhe21} we initialize all variables
as for the LWE estimator   \cite{albrecht2015concrete}, but instead of
calling the \texttt{estimate\_lwe} function we %call \verb+hybrid_dual+ or 
\texttt{hybrid\_primal}. 

==> sections/packing-techniques.tex <==
 
 
In this section, we give a precise specification of the ring packing technique where we can "load" LWE encrypted messages
into arbitrary coefficients of an RLWE encrypted messages. 
Then we show how to efficiently perform cyclic shifts of the coefficients of RLWE encrypted message.

 
\subsection*{Packing and Vector Packing.}
Below, we specify the packing technique. 
 
\begin{definition}[Packing LWE to RLWE]
We define the key generation algorithm $\PackSetup$ and  LWE to RLWE switching $\LWEtoRLWE$ as follows.

\begin{description} 
\item[$\PackSetup(\bound_{\packKey}, n, \deg, q, \vec{s}, \fr{s}, \basis_{\packKey}):$]
Takes as input 
bound $\bound_{\packKey} \in \NN$, a dimension $n \in \NN$, a degree $\deg \in \NN$ and
a modulus $q \in \NN$ that define $\R_{\deg, q}$, a vector  $\vec{s} \in \ZZ_q^n$,  
a polynomial $\fr{s} \in \R_{\deg, q}$ and a basis $\basis_{\packKey} \in \NN$.  
\begin{enumerate}
\item Set $\ell_{\packKey} = \roundUp{\log_{\basis_{\packKey}}{q}}$. 
\item For $i \in [n]$,  $j \in [\ell_{\packKey}]$ and $k \in [\basis_{\packKey}]$ set  
\begin{align*}
\packKey[i,j, k] \exec \RLWE_{\bound_{\packKey}, \deg, q}(\fr{s}, \vec{s}[i] \cdot \basis_{\packKey}^{j-1} \cdot (k-1)).
\end{align*}

\item Output $\packKey \in \RLWE_{\bound_{\packKey}, \deg, q}(\fr{s}, .)^{n \times \ell_{\packKey} \times \basis_{\packKey}}$. 
\end{enumerate}

\item[$\LWEtoRLWE(\vec{c}, \packKey, d):$]
Takes as input a  LWE ciphertext $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \LWE_{\bound_{\vec{c}}, n, q}(\vec{s}, .)$, a packing key $\packKey \in \RLWE_{\bound_{\packKey}, \deg, q}(\fr{s}, .)^{n \times \ell_{\packKey} \times \basis_{\packKey}}$, and an index $d$. 
\begin{enumerate}
\item Denote $\ell_{\packKey} = \roundUp{\log_{\basis_{\packKey}}{q}}$.
\item  Set $\fr{b}' \exec b \cdot X^{d - 1} \in \R_{\deg, q}$.   
\item Compute $\ma{A} \exec \Decomp_{\basis_{\packKey}, q}(\vec{a}) \in \R_{\basis_{\packKey}}^{n \times \ell_{\packKey}}$.    
\item Compute $c_{\out} \exec [\fr{b}', 0]^{\top} - X^{d-1} \cdot \sum_{i=1}^n \sum_{j=1}^{\ell_{\packKey}} \packKey[i,j, \ma{A}[i,j] + 1]$.  
\end{enumerate}
\end{description} 
 \end{definition}
  
  We note that we may define a different version of the packing procedure, where the packing key doesn't include precomputed values of $\ma{A}[i,j]$, but instead we multiply the RLWE sample with $\ma{A}[i,j]$ in step 4. 
  This way we can reduce the size of the packing key from $n \cdot \ell_{\packKey} \cdot (\basis_{\packKey} - 1)$ to $n \cdot \ell_{\packKey}$ RLWE tuples,
   but
  slightly increase the complexity and error growth rate of the packing algorithm. 
  We give the
  alternative version in supplementary material~\ref{sec:alternative-packing}, but state its correctness lemma
  below.
  

\begin{lemma}[Correctness of LWE to RLWE Packing (Precomp.)]
\label{lemma:correctness-lwe-to-rlwe-packing}
Let  $\basis_{\packKey} \in \NN$, $q \in \NN$, $\vec{s} \in \ZZ_q^{n \times 1}$ and
  $\vec{c} \in \LWE_{\bound_{\vec{c}}, n, q}(\vec{s}, \msg)$. 
Furthermore, let $\bound_{\packKey} < q$ be a bound on the packing key error. 
If we execute $\packKey \exec \PackSetup(\bound_{\packKey}, n, \deg, q, \vec{s}, \fr{s}, \basis_{\packKey})$  
and $c_{\out} \exec \LWEtoRLWE(\vec{c}, \packKey, k)$ for some $k \in [\deg]$,
then $c_{\out} \in \RLWE_{\bound, \deg, q}(\fr{s}, \msg_{\out})$,
where $\msg_{\out} = \msg \cdot X^{k} \in \R_{\deg, q}$, 
\begin{itemize}
\item $\bound \leq  \bound_{\vec{c}} + n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$ for the precomputed version, 

\item $\bound \leq   \bound_{\vec{c}} + (\frac{7}{12}) \cdot n \cdot \ell_{\packKey} \cdot \basis_{\packKey}^2 \cdot  \bound_{\packKey}$ for the ordinary version given in supplementary material~\ref{sec:alternative-packing}
\end{itemize}
and
$\ell_{\packKey} = \roundUp{\log_{\basis_{\packKey}}{q}}$.
\end{lemma}
 
 
 
%
%\begin{proof}[of lemma \ref{lemma:correctness-lwe-to-rlwe-packing} - Correctness of LWE to RLWE Packing]
%Note that the packing algorithm proceeds similarly as the keyswitch algorithm from LWE to LWE, with the exception 
%that we represent
%$\vec{c}$ as a polynomial of degree $X^{d-1}$ in $\R_{\deg, q}$.
%For completeness we will mostly restate the proof for this case.
% 
%Let $\vec{c}_i = \sum_{j=1}^{\ell_{\packKey}}  \packKey[i,j, \ma{A}[i,j]+1]$. We have that:
%\begin{align*}
%	\vec{c}_i &= \sum_{j=1}^{\ell_{\packKey}}  \packKey[i,j, \ma{A}[i,j]+1] \\
%	&= \sum_{j=1}^{\ell_{\packKey}}  \RLWE_{\bound_{\packKey}, \deg, q}(\fr{s}, \vec{s}[i] \cdot \basis_{\packKey}^{j-1} \cdot \ma{A}[i,j]) \\
%	&=  \RLWE_{\bound_{1}, \deg, q}(\fr{s}, \vec{a}[i] \cdot \vec{s}[i])
%\end{align*}
%where %$\errDist_{\bound_{1}}$ is a $\bound_1$-Bounded distribution with 
%$\bound_1 \leq \ell_{\packKey} \cdot \bound_{\packKey}$.
%Then  note that
%\begin{align*}
%[\fr{b}'', \fr{a}'']^{\top} &= X^{d-1} \sum_{i=1}^{n} \vec{c}_i \\
%&= \sum_{i=1}^{n} \RLWE_{\bound_{1}, \deg, q}(\fr{s},  \vec{a}[i] \cdot X^{d-1} \cdot \vec{s}[i]) \\ 
%&=  \RLWE_{\bound_{2}, \deg, q}(\fr{s}, \sum_{i=1}^{n} \vec{a}[i] \cdot X^{d-1} \cdot \vec{s}[i])  \\
%&= \RLWE_{\bound_{2}, \deg, q}(\fr{s},  \vec{a}^{\top}  \cdot \vec{s}  \cdot X^{d-1}),
%\end{align*} 
%where %$\errDist_{\bound_{2}}$ is a $\bound_{2}$-Bounded distribution with 
%$\bound_{2} \leq n \cdot \bound_1 \leq n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%Let us denote $\fr{b}' = X^{d-1} \cdot (\vec{a}^{\top} \cdot \vec{s} + \msg + e)$ and
%$\fr{b}'' = \fr{a}'' \cdot \fr{s} + \vec{a}^{\top} \cdot \vec{s} \cdot X^{d-1} + \fr{e}''$,
%then
%\begin{align*}
%\vec{c}_{\out}^{\top} = [\fr{b}', 0] - [\fr{b}'', \fr{a}''] = [- \fr{a}'' \cdot \fr{s} + X^{d-1} \cdot \msg +  e \cdot X^{d - 1} - \fr{e}'', - \fr{a}''].
%\end{align*}
%Hence, $\vec{c}_{\out}$ is a valid RLWE sample of $X^{d-1} \cdot \msg$ with respect to key $\fr{s}$ 
%and $\norm{\Error(c)}_2  \leq \bound \leq \norm{e \cdot X^{d - 1} - \fr{e}''}_2 \leq \bound_{\vec{c}} + \bound_{2} \leq
% \bound_{\vec{c}} + n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%\end{proof}




\begin{definition}[Vector Packing]
The packing algorithm $\PackLWEtoRLWE$ is defined as follows.
\begin{description}
\item[$\PackLWEtoRLWE(\vec{v}, \packKey):$]
Takes as input vector  $\vec{v} \in \LWE_{\bound_{\vec{v}}, n, q}(\vec{s}, .)^{m \times 1}$, and a packing key $\packKey$.
\begin{enumerate}
\item For $k \in [m]$ set $\vec{d}[k] \exec \LWEtoRLWE(\vec{v}[k], \packKey, k)$.
\item Output $\ct_{\out} \exec \sum_{i=1}^{m} \vec{d}[i]$.
\end{enumerate} 
\end{description}
\end{definition}
 

\begin{lemma}[Correctness of Vector Packing]
\label{lemma:correctness-of-vector-packing}
Let us define the packing key $\packKey \exec \PackSetup(\bound_{\packKey}, n, \deg, q, \vec{s}, \fr{s}, \basis_{\packKey})$,
where $n \in \NN$, $\deg \in \NN$ is
the a degree, $q \in \NN$,  $\bound_{\packKey} < q$, $\vec{s} \in \ZZ_q^{n \times 1}$, $\fr{s} \in \R_{\deg, q}$ and $\basis_{\packKey} \in \NN$. 
Let $\vec{v} \in \LWE_{\bound_{\vec{v}}, n, q}(\vec{s}, .)^{m \times 1}$ be a vector of 
$m \leq \deg$ LWE ciphertexts of $[\msg_1, \dots, \msg_m]$. 
If $\vec{c}_{\out} \exec \PackLWEtoRLWE(\vec{v}, \packKey)$,
then $\vec{c}_{\out} \in \RLWE_{\bound, \deg, q}(\fr{s}, \msg_{\out})$,
where 
$\msg_{\out} = \sum_{i=1}^{m}  \msg_{i} \cdot X^{i-1} \in \R_{\deg, q}$
and $\msg_{i} = 0$ for all $m \le i \leq N$.
Furthermore we have  
\begin{itemize}
\item $\bound \leq \bound_{\vec{v}} + m \cdot n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$  for the precomputed packing version, 

\item $\bound \leq  \bound_{\vec{v}} + (\frac{7}{12}) \cdot m \cdot n \cdot \ell_{\packKey} \cdot \basis_{\packKey}^2 \cdot \bound_{\packKey}$ for the ordinary packing version given in supplementary material~\ref{sec:alternative-packing}, 
\end{itemize}
and
$\ell_{\packKey} = \roundUp{\log_{\basis_{\packKey}}{q}}$.
\end{lemma}


%
%\begin{proof}[of lemma \ref{lemma:correctness-of-vector-packing} - Correctness of Vector Packing]
%For $i \in [m]$ us denote $\vec{v}[i] = [b_i, \vec{a}_i] \in \ZZ_q^{(n+1) \times 1}$,
%where $b_i = \vec{a}_1^{\top}\cdot \vec{s} + \msg_i + e_i$, 
%and let $\vec{d}[i] = [\fr{b}_i, \fr{a}_i]$.
%Then from the the proof of lemma \ref{lemma:correctness-lwe-to-rlwe-packing}, we can write
%$\fr{b}_i'' = \fr{a}_i'' \cdot \fr{s} + X^{i-1} \cdot \msg_i + \fr{e}_i'' + X^{i-1} \cdot e_i$,
%for some $\fr{a}''_i \in \R_{\deg, q}$ and $\fr{e}_i''$ from the packing key.
%Note also that, as in the proof of lemma  \ref{lemma:correctness-lwe-to-rlwe-packing},
%for all $i \in [m]$
%we have  $\norm{\fr{e}_i''}_2 \leq \bound_{2} \leq n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$.
%Now we can denote
%$
%\ct_{\out} = \begin{bmatrix}
%\fr{a}_{\out} \\
%\fr{b}_{\out}
%\end{bmatrix}
%$
%where $\fr{a}_{\out} = \sum_{i=1}^m \fr{a}''_i$ and 
%\begin{align*}
%\fr{b}_{\out} = \sum_{i=1}^m \fr{b}_i'' = \fr{a}_{\out}^{\top} \cdot \fr{s} + \sum_{i=1}^m \msg_{i} \cdot X^{i-1} + \sum_{i=1}^m \fr{e}_i'' + \sum_{i=1}^{m} e_i \cdot X^{i-1}.
%\end{align*}
%Furthermore we have
%that $\norm{\Error(\ct_{\out})} = \norm{\sum_{i=1}^m \fr{e}_i'' + \sum_{i=1}^{m} e_i \cdot X^{i-1}}_2 = \norm{\sum_{i=1}^m \fr{e}_i''}_2 + \norm{\sum_{i=1}^{m} e_i \cdot X^{i-1}}_2 \leq \bound \leq m \cdot \bound_{2} + \bound_{\vec{v}} \leq \bound_{\vec{v}} + m \cdot n \cdot \ell_{\packKey} \cdot \bound_{\packKey}$. 
%
%To conclude the proof we have that $\ct_{\out} \in \RLWE_{\bound, \deg, q}(\msg_{\out})$, 
%where $\msg_{\out} = \sum_{i=1}^m \msg_{i} \cdot X^{i-1}$.
%% and $\errDist_{\bound}$ is a $\bound$-Bounded distribution.
%\end{proof}



==> sections/parameters-correctness-previous-work.tex <==



\begin{table}[t]%[!htb] 
	\centering 
	\begin{tabular}{c | c | c | c | c | c}
		\hline
		Parameter  & Bourse et al. \cite{C:BMMP18} & \cite{EPRINT:ChiJoyPai21} Set 1 & \cite{EPRINT:ChiJoyPai21} Set  2 & \cite{EPRINT:ChiJoyPai21} Set 3 & Carpov et al. \cite{RSA:CarIzaMol19} \\
		\hline  	
 $n$ &  $2^{10}, 450$ & $542$ & $592$ &  $938$ &  $803$ \\
 $u$ &  $1$  & $1$  &   $1$   &  $1$  & $1$ \\ 
 $\deg$ & $2^{10}$  & $2^{10}$ &   $2^{11}$  &  $2^{12}$ & $2^{14}$ \\ 
 $q$ &  $2^{32}$ & $2^{64}$ &  $2^{64}$  & $2^{64}$ & $2^{64}$ \\
 $Q$ & $2^{32}$  & $2^{64}$ &  $2^{64}$ & $2^{64}$ & $2^{64}$ \\ 
 $\basis_{\RGSW}$ &  $2^{10}$ & $?, (2)$  & $?, (2)$  & $?, (2)$  & $2^{6}$ \\ 
 $\basis_{\keySwitchKey}$ &  $2^3$  & $?, (2)$  & $?, (2)$  & $?, (2)$ & $2^4$ \\ 
$\stddev$ & $4, 2^{15}, 0.0625$ & $2^{43}, 2^{24}$  &  $2^{41}, 8$  & $2^{41}, 4$ & $2^{44},2^{14}$\\
 $\vec{s}$ &  $[0, 1], -$  & $[0, 1], -$ & $[0, 1], -$  & $[0, 1], -$ &   $[0, 1], 63$ \\
 $\fr{s}$ & $[0, 1], -$ & $[0, 1], -$  & $[0, 1], -$   & $[0, 1], -$ &  $[0, 1], -$  \\
\end{tabular}  
\caption{Parameter sets from literature. 
%The first column gives the parameters from Bourse et al. \cite{C:BMMP18}. The other columns give the parameter sets given in \cite{EPRINT:ChiJoyPai21}.
Unfortunately, some parameters are not given.
We took the liberty to set the missing parameters such that to maximize correctness in favor of the previous schemes.
 Values in parentheses are the values we took for our noise estimation.
 The $\stddev$ row contains the standard deviations.
 For Bourse et al. \cite{C:BMMP18} we have $n=2^{10}$ for fresh ciphertexts, and $450$ for key switching keys with standard deviations
 $4$ and $2^{15}$ respectively. For \cite{EPRINT:ChiJoyPai21} and \cite{RSA:CarIzaMol19}  there are two standard deviation values. The first is for $\LWE$ samples and the second is for $\RLWE$ samples. 
% For Carpov et al. \cite{RSA:CarIzaMol19} the error standard deviation $2^{44}$ is for all $\LWE$ samples (including the key switching key), whereas $2^{14}$ is for all $\RLWE$ samples.
 }\label{tbl:parameter-sets-from-literature}
\end{table}


\begin{table}[t] 
 %\setlength{\tabcolsep}{7pt}
 \centering 
 \begin{tabular}{| c | c | c | c | c | c | c | c |}
 \hline
 Parameter Set & $t=2^{4}$  & $t=2^{5}$ & $t=2^{6}$ &  $t=2^{7}$ & $t=2^{8}$ & $t=2^{9}$  &  Key \\  
 \hline   
Bourse et al. \cite{C:BMMP18} &  $2^{-13}$ &  $2^{-5}$ & $0.34$  &   $0.63$ & $0.81$ & $0.90$ & 99\% \\  
\cite{EPRINT:ChiJoyPai21} Set 1 &  $2^{-23}$  &   $2^{-7}$ & $0.19$ & $0.51$ & $0.74$ &  $0.87$ & 100\% \\ 
\cite{EPRINT:ChiJoyPai21} Set 2 &  $0.0$  &  $2^{-21}$ & $2^{-7}$ & $0.21$ & $0.53$ & $0.75$ & 100\% \\ 
\cite{EPRINT:ChiJoyPai21} Set 3 &  $0.0$  &   $2^{-49}$ & $2^{-14}$ & $0.04$ & $0.32$ & $0.62$ & 100\% \\  
Carpov et al. \cite{RSA:CarIzaMol19} &  $2^{-38}$  &   $2^{-11}$ & $0.08$ & $0.38$ & $0.66$ & $0.82$ & 0\% \\ 
\hline
\end{tabular} 
\caption{Correctness for different plaintext spaces. The plaintext space is $\ZZ_t$.
However, we need to keep in mind that to compute any function the plaintexts must be $< \roundDown{t/2}$. 
The key column gives the contribution of the secret key in the error.}\label{tbl:parameter-sets-correctness-from-literature}
\end{table}


\begin{table}[!htb]
	%\setlength{\tabcolsep}{7pt}
	\centering 
	\begin{tabular}{|c | c | c | c | c | c | c | c | c |}
		\hline
	 \multirow{2}{*}{Set}     & \multicolumn{3}{c|}{RLWE} & \multicolumn{4}{c|}{LWE}  \\
		   & uSVP & dec & dual  &  uSVP & dec & dual  &    Hyb. Primal \\ 
		\hline   
Bourse et al. \cite{C:BMMP18} &  82.1 & 88.0 & 91.5 & 81.4 (78.9) & 192.7   & 87.1 (77.8) &  88.0 (81.0) \\  
\cite{EPRINT:ChiJoyPai21} Set 1 & 81.1  &  148.1 & 84.1 &  80.2 (77.5) &  321.3   &  84.7 (75.1) & 80.8 (80.3) \\  
\cite{EPRINT:ChiJoyPai21} Set 2 &  108.0 & 123.5 & 111.4 &  80.0 (77.6) &  286.9   &  83.9 (74.7) & 86.6 (81.0)  \\  
\cite{EPRINT:ChiJoyPai21} Set 3 &  231.2 & 261.6 & 236.8 &  128.0 (119.0) &  490.8   &  135.9 (108.3) &  139.8 (90.3) \\  
Carpov et al. \cite{RSA:CarIzaMol19} &   1445.8 & 2302.8 & 1465.1 &  116.4 & 569.6 &  106.8 & 80.9  \\  
\hline
\end{tabular} 
 \caption{Security of the parameter sets.
Out of curiosity, we ran the estimations with Hamming weight of $64$ and included the security in parentheses.
The estimates further ensure us that the keys for the LWE samples were not considered to be sparse.
 }\label{tbl:parameter-sets-size-and-security-from-literature}
\end{table}


In this section, we revisit the parameters from Bourse et al. \cite{C:BMMP18}, Chillotti, Joye, and Paillier \cite{EPRINT:ChiJoyPai21},
and Carpov, Izabach\'ene, and Mollimard \cite{RSA:CarIzaMol19}.
We summarize the parameters at Table~\ref{tbl:parameter-sets-from-literature}.
We show the correctness of these parameter sets when using TFHE to
compute functions over larger message spaces.
We summarize our correctness estimations at Table~\ref{tbl:parameter-sets-correctness-from-literature}.
Note that we calculate the correctness based on the $\bound_{\deg}$ bound from Theorem~\ref{thm:correctness-tfhe-bootstrapping}.
We give the correctness estimates for different plaintext spaces $\ZZ_t$ with $t=2^{k}$. Remind that to compute any function via the TFHE bootstrapping algorithm correctly, the plaintext space must be smaller than $t=2^{k-1}$.
Importantly, this restriction rules out computing affine functions on the LWE ciphertexts without bootstrapping.
At Table~\ref{tbl:parameter-sets-size-and-security-from-literature} we estimate the security of the parameters.
 

Unfortunately, some parameters were not listed in the papers. Therefore, we choose the most favorable ones in terms of correctness.
We stress that these parameters do not influence security.
Also, we note that we use the error estimation from this paper. We omit, for instance, approximate gadget matrices used by some of the previous work. Hence our estimations may be more optimistic.
Nevertheless, we show that non-sparse keys play a significant role in the correctness of bootstrapping.
Finally, we note that our analysis of the error is in favor of the previous work.
In particular, if there is no bound on the Hamming weight of the secret key, then we take the expected hamming weight for the given key distribution calculated as $\round{\frac{(b-a)\cdot \deg}{b - a + 1}}$,
 where the secret key coefficients are from $[a,b]$. 
 Concretely, for a binary secret key and $n=2^{10}$, we take the Hamming weight $512$.  
 Note that the actual Hamming weight may be smaller or higher.
 Previous work described their systems over the torus, i.e., real numbers modulo 1.
 The standard deviation parameter is then given as a number between  $[0, 1)$.
 However, all works implement their schemes over an integer modulus which is either $2^{32}$ or $2^{64}$.
 Hence all random variables over the torus are scaled by the modulus $Q$.
Let $\alpha$ denote the standard deviation over the torus. Then we translate the standard deviation
over the integers as $\stddev = \alpha \cdot Q$.
 For instance, for the parameter set by Bourse et al. \cite{C:BMMP18} we set the standard deviation to $0.0625$.
 In \cite{C:BMMP18}, they work over the torus that is implemented with 32-bit integers\footnote{We established that the torus is scaled by $2^{32}$ based on the implementation provided at \texttt{https://github.com/mminelli/dinn}. The $\TFHE$ library is instantiated over \texttt{Torus32}.}.
 The error variance is given as a fraction of the torus, which is $\alpha = 2^{-36}$ for the bootstrapping key (see Table~4 at page 23 \cite{C:BMMP18}).
 At Table~\ref{tbl:parameter-sets-size-and-security-from-literature} we list the correctness
 for $\bound_{\deg} \leq (\frac{2 \cdot \deg}{q})^2 \cdot \bound_{\ct} + \frac{2}{3}  + \frac{2}{3} + \hamming(\vec{s}) \cdot (\norm{\Var(\vec{s})}_{\infty} + \norm{\E(\vec{s})}_{\infty}^2)$,
 where $\bound_{\ct} = \bound_{\out}$ and $q=Q$.
 Additionally, we took into account some controlled leveled operations performed between blind rotation and key switching. 
 In particular, we estimated for $\bound_{\ct} = \bound_{\out} + \bound_{\out} \cdot \sqrt(t/2)$. Such operations
 can be done given that the effective plaintext space is $\sqrt(t/2)$ and is used when computing two variate functions using TFHE bootstrapping.
 furthermore we estimated the error of leveled computation as performed by Carpov, Izabach\'ene, and Mollimard \cite{RSA:CarIzaMol19},
 and which we recall in an paragraph below.
 However, the leveled operations had only a marginal influence on the correctness.
 
 
 As we see, correctness for larger plaintext spaces is relatively low. 
For all parameter sets with non-sparse keys, the error is overwhelmingly dominated by the error of the secret key.\
From Table~\ref{tbl:parameter-sets-correctness-from-literature} we conclude that the parameter sets from \cite{EPRINT:ChiJoyPai21} 
are incapable of computing correctly for reasonable input plaintext. 
For instance, if we take a 6-bit input plaintext, we return an incorrect value with probability $0.59$ with Set 2 and
$0.70$ with Set 1. Furthermore, as hinted above, because we cannot correctly compute affine functions without bootstrapping,
to compute multivariate functions using TFHE, we need to restrict the effective plaintext space to $3$ bits instead of $6$. 
Finally, we note that certain input plaintext may tolerate the error better than others.
For instance, to compute the sign function as in \cite{C:BMMP18}, the rotation polynomial is set
to return $1$ for $\tilde{\msg} \in [0, \deg)$ and $-1$ for $\tilde{\msg} \in [\deg, 2\cdot \deg)$.
Given that the message is in the middle of any of the intervals, several shifts should not interfere with the output.
The problem is with corner cases where any perturbation of the message results in an incorrect outcome of the bootstrapping.
 
%
%
%Finally, as we can see from Table~\ref{tbl:parameter-sets-size-and-security-from-literature}, 
%parameters from \cite{C:BMMP18,EPRINT:ChiJoyPai21} offer much smaller security than the authors report.

\paragraph{Why computing leveled operations in \cite{EPRINT:ChiJoyPai21} is incorrect?}

As we already noted on numerous occasions, we cannot easily perform leveled operations when using the half domain functional bootstrapping algorithm.
It is easy to see for example when inspecting computation of the max function according to the formula $\max(x, y) = \max(0, x-y) + y$.
The idea is to compute the max with a single bootstrapping operation to compute $\max(0, z)$ where $z = x-y$.
However, the problem appears when $y>x$, in which case the phase of the ciphertext holding $z$ is in $[\deg, 2 \cdot \deg]$.
In this case, the bootstrapping algorithm will output $- f(\deg - z)$. 



\paragraph{Multiple invocations of the LUT from Carpov et al. \cite{RSA:CarIzaMol19}.}

Carpov et al. \cite{RSA:CarIzaMol19} propose a bootstrapping method that mainly follows $\TFHE$, with the exception that after the blind rotation step, we multiply the accumulator with a rotation polynomial.
In this paper, we call these polynomials post-rotation polynomials $\mathsf{TV}_F^{(1)}$.
The rotation polynomial used during blind rotation $\mathsf{TV}_F^{(0)}$ is independent of the function that is being computed,
but multiplying the blind rotated polynomial by $\mathsf{TV}_F^{(1)}$ results in having the outcome of a function
encoded in the constant coefficient.
Specifically we have that the constant coefficient of $\mathsf{TV}_F^{(0)} \cdot X^{b - \inner{a}{s}} \cdot \mathsf{TV}_F^{(1)} \in \R_{\deg, Q}$ encodes
the outcome of $F(b - \inner{a}{s})$ where $F$ is determined by $\mathsf{TV}_F^{(1)}$.
Since $\mathsf{TV}_F^{(1)}$ is applied after blind rotation, and blind rotation itself is independent of the computed function, the idea is
that we may apply many post-rotation polynomials to compute many functions on the same input with only a single blind rotation.
One caveat is that multiplying with the polynomial $\mathsf{TV}_F^{(1)}$ induces a rather large error; hence we limit the functions to functions with domain over $\{0, 1\}$.
Finally, it is important to note that, to compute any function, we must limit the plaintext space such that the phase of the input ciphertext is in $[0, \deg)$ because of the negacyclicity problem of $\TFHE$.

Nevertheless, we can compute $k$-to-$k$ bit LUTs, by bootstrapping a ciphertext encoding a $k$-bit plaintext in an $k+1$-plaintext space,
and applying $k$ post-rotation polynomials computing all output bits.
Specifically, the input ciphertexts have a phase $\tilde{\msg} = \frac{2 \cdot \deg}{t} \cdot \msg + e$, where $t = 2^{k+1}$
and $\msg \in \ZZ_{2^k}$.
After bootstrapping, we get $k$ ciphertexts with phases $\tilde{m_i} = \frac{Q}{t} \cdot m_i + e_i$,
where $m_i = F_i(\msg)$ and $F_i: \ZZ_{2^{k}} \mapsto \{0, 1\}$. 
To be able to use functional bootstrapping again, we must compose these bits back to an integer.
Carpov et al. \cite{RSA:CarIzaMol19} suggest to compute a linear combination (see Section~4.2 in \cite{RSA:CarIzaMol19}).
While Carpov et al. \cite{RSA:CarIzaMol19} rightfully identify that such linear combinations induce a significant error,
they do not give any error analysis, nor do they state the error rate for their parameters.
Below we estimate the error rate.
Let $\bound_{BR}$ be the variance of the error induced by blind rotation.
Before we extract the LWE sample encoding the constant coefficient we multiply the
outcome RLWE sample with $\mathsf{TV}_{F_i}^{(1)}$. 
Denote $\bound_{BR, \mathsf{TV}}$ the bound on the variance of the resulting RLWE sample. 
From 
linear homomorphism we have $\bound_{BR, \mathsf{TV}} \leq \bound_{BR} \cdot \bound_{\mathsf{TV}}^{2} \cdot \deg$ where
$\norm{\mathsf{TV}_{F_i}^{(1)}}_{\infty} \leq \bound_{\mathsf{TV}}$. 
Let $[\ct_i]_{i=1}^{k}$ denote the LWE ciphertexts obtained by extracting 
the constant coefficient of the RLWE sample. From correctness of the extraction 
we have that the bound on the error variance stays the same.
In particular, we have $\ct_i = \LWE_{\bound_{BR, \mathsf{TV}}, \deg, Q}(\KeyExtract(\fr{s}), \Delta_{Q, t} \cdot F_{i}(m_i))$. 
Now we compute the  $\ct_{F} = \sum_{i=1}^k \ct_{i} \cdot 2^{i-1}$.
From linear homomorphism of LWE samples, we have  
\begin{align*}
\Var(\Error(\ct_{F})) \leq \sum_{i=1}^k \bound_{BR, \mathsf{TV}} \cdot  (2^{i-1})^2  
\leq \bound_{BR, \mathsf{TV}} \cdot \sum_{i=1}^k  2^{2(k-1)}  
\leq k \cdot   2^{2(k - 1)} \bound_{BR, \mathsf{TV}} 
\end{align*}
Then we key switch from $\KeyExtract(\fr{s})$ to $\vec{s}$, 
obtaining $\ct_{F, n} = \LWE_{\bound_{F, n}, n, Q}(\vec{s}, \Delta_{Q, 2^{k+1}} \cdot \sum_{i=1}^k F_{i}(m_i) \cdot 2^{i-1})$.
From correctness of key switching
we have $\bound_{F, n} \leq k \cdot \cdot 2^{2(k - 1)} \bound_{BR, \mathsf{TV}}  + (\frac{1}{3}) \cdot \deg \cdot \ell_{\keySwitchKey} \cdot \basis_{\keySwitchKey}^2 \cdot \bound_{\keySwitchKey}$.
Finally, before blind rotating we switch the modulus from $Q$ to $2 \cdot \deg$.
Let $\bound_{\deg}$ denote the bound on the LWE sample after modulus switching.
From correctness of modulus switching we have
\begin{align*}
\bound_{\deg} \leq \frac{(2\cdot \deg)^2}{Q^2} \cdot \bound_{F, n} + \frac{2}{3} + \frac{2}{3} \cdot \hamming(\vec{s}) \cdot \big(\norm{\Var(\vec{s})}_{\infty} + \norm{\E(\vec{s})}_{\infty}^2\big).
\end{align*}

 

\paragraph{Correctness of the Experiments in Bourse et al. \cite{C:BMMP18}.}
In Bourse et al. \cite{C:BMMP18}, the authors test two neural networks that are as follows.
\begin{align*}
x_i = \sum_{j=1}^{W} \sgn(\sum_{k=1}^{784} m_k \cdot w_{k, j}^{(1)}) \cdot w_{j, i}^{(2)},
\end{align*} 
where $[m_k]_{k=1}^{784}$ are the input messages, $[w_{k, j}^{(1)}]_{k=1,j=1}^{784,W}$ are weights of the first layer,
 $[w_{j, i}^{(2)}]_{j=1,i=1}^{W,10}$ are weights of the second layer, and $[x_i]_{i=1}^{10}$ are outputs of the network.
The vector $[x_i]_{i=1}^{10}$ is computed over encrypted data, and returned to the client. 
Bourse et al. \cite{C:BMMP18} perform two tests for $W=30$ and $W=100$.
Unfortunately, they did not provide an error analysis. 
Below we calculate the correctness errors and show that the correctness
of the experiments is low for the chosen parameters. We present the estimates at Table~\ref{tbl:correctness-bourse}.

The homomorphic evaluation is as follows.
First we encode $[m_k]_{k=1}^{784}$ in the coefficients of a RLWE sample $\vec{c} = \RLWE_{\bound, \deg, Q}(\fr{s}, \Delta_{Q, t_1} \cdot \sum_{k=1}^{784} m_k \cdot X^{k-1})$,
where $\deg = 2^{10}$ and $t_1 < Q$ defines the message space $\ZZ_{t_1}$.
Then for each $j \in [W]$ we multiply $\vec{c}_j = \vec{c} \cdot \fr{w}_j = \RLWE_{\bound_{j}, \deg, Q}(\fr{s}, \Delta_{Q, t_1} \cdot \fr{w}_j \cdot \sum_{k=1}^{784} m_k \cdot X^{k-1})$, where $\fr{w}_j$ is a polynomial such that the constant coefficient
of $\fr{w}_j \cdot \sum_{k=1}^{784} m_k \cdot X^{k-1} \in \R_{\deg, Q}$
is equal $\sum_{k=1}^{784} m_k \cdot w_{k, j}^{(1)}$.
From linear homomorphism of GLWE samples we have that $\bound_j \leq 784 \cdot \bound_{\fr{w}}^2 \cdot \bound$,
where $\norm{\fr{w}}_{\infty} \leq \bound_{\fr{w}}$.
Then we extract the LWE samples encoding the constant coefficient from $\vec{c}_j$
and we key switch obtaining $\vec{c}'_j = \LWE_{\bound'_j, n, Q}(\vec{s}, \Delta_{Q, t_1} \cdot \sum_{k=1}^{784} m_k \cdot w_{k, j}^{(1)})$.
From correctness of sample extraction and key switching we have
$\bound'_j \leq \bound_j + (\frac{1}{3}) \cdot \deg \cdot \ell_{\keySwitchKey} \cdot \basis_{\keySwitchKey}^2 \cdot \bound_{\keySwitchKey}$.
We compute the sign function by blind rotating $\vec{c}'_j$ for each $j \in [W]$.
For blind rotation we first switch the modulus from $Q$ to $2 \cdot \deg$, obtaining
$\vec{c}''_j = \LWE_{\bound''_j, n, 2 \cdot \deg}(\vec{s}, \Delta_{2 \cdot \deg, t_1} \cdot \sum_{k=1}^{784} m_k \cdot w_{k, j}^{(1)})$.
From correctness of modulus switching we have
\begin{align*}
\bound''_j \leq \frac{(2\cdot \deg)^2}{Q^2} \cdot \bound'_{j} + \frac{2}{3} + \frac{2}{3} \cdot \hamming(\vec{s}) \cdot \big(\norm{\Var(\vec{s})}_{\infty} + \norm{\E(\vec{s})}_{\infty}^2\big).
\end{align*} 

Denote $\vec{c}_{BR, j} = \LWE_{\bound_{BR}, \deg, Q}(\vec{s}, \Delta_{Q, t_2} \cdot y_j)$ the LWE tuple obtained by blind rotation and extracting the LWE sample
encoding the constant coefficient. Note that $\bound_{BR}$ is the error induced by the blind rotation algorithm and
$t_2 < Q$ defines the plaintext space $\ZZ_{t_2}$. 
The last step before returning the ciphertext is to compute the
affine functions $\vec{c}_{i, \out} = \sum_{j=1}^{W} \vec{c}_{BR, j} \cdot w_{j, i}^{(2)}$.
From linear homomorphism of GLWE samples we have $\vec{c}_{i, \out} =   \LWE_{\bound_{i, \out}, \deg, Q}(\Delta_{Q, t_2} \cdot x_i)$,
where $\bound_{i, \out} \leq W \cdot \bound_{BR} \cdot \bound_{w^{(2)}}^2$ and
$w_{j, i}^{(2)} \leq \bound_{w^{(2)}}^2$ for all $i \in [10]$ and $j \in [W]$.

\begin{table}[t]  
 \centering 
 \begin{tabular}{| c | c | c | c | c | c | c|}
 \hline
$W$ & $t_1$  & $t_2$ & $\bound_{\fr{w}}$ &  $\bound_{w^{(2)}}$ & $Corr(\bound''_j)$ & $Corr(\bound_{i, \out})$  \\  
 \hline   
$30$ & $4676$  & $796$ & $2338$ &  $399$ & $0.985$ & $0.986$  \\  
$30$ & $2500$  & $800$ & $2338$ &  $399$ & $0.973$ & $0.986$  \\  
$100$ & $2744$  & $976$ & $1372$ &  $488$ & $0.975$ & $0.994$  \\  
$100$ & $1800$  & $1000$ & $1372$ &  $488$ & $0.962$ & $0.995$  \\  
\hline
\end{tabular} 
\caption{Correctness of the experiments from Bourse et al. \cite{C:BMMP18}. Here $CorrErr(\bound) = \erf(\frac{q}{2 \cdot t \cdot \sqrt{\bound} \cdot \sqrt{2}})$, where $t$ is the message space and $q$ the modulus. $CorrErr(\bound)$ gives us the probability of having an incorrect output.}\label{tbl:correctness-bourse}
\end{table}

Finally, we note that when computing, for instance, the sign function, even incorrect bootstrapping has a fair chance of returning
a correct outcome. For instance if we bootstrap $\Delta_{2 \cdot \deg, t} \cdot msg$ and $\msg \approx t/4$. Then
even if the error perturbs the message resulting in a ``correct'' encryption of $\Delta_{2 \cdot \deg, t} \cdot (msg + 1)$, then the outcome may still be correct from $\msg$. Low correctness error is problematic for corner cases when $\msg \approx t/2$, and a perturbation flips the message to $\msg' > t/2$, consequently flipping the sign.




%TODO Commented out Guimar\~aes
%\paragraph{Guimar\~aes et al. \cite{CHES:GuiBorAra21}.}
%
%Guimar\~aes et al. \cite{CHES:GuiBorAra21} propose two methods: A tree method and a chaining method.  
%In the case of the tree method, the authors claim it is capable of computing any function in linear time in the size of the input 
%(see page 1, page 2, and Table 1 at page 13 of \cite{CHES:GuiBorAra21}). 
%Unfortunately, the authors do not provide correctness proofs of any of their methods. Furthermore, it is unclear how to choose the rotation polynomials (in \cite{CHES:GuiBorAra21} they call it LUTs) to compute any function as claimed.
%Nevertheless, it turns out that the tree-based algorithm as specified by Algorithm~6 in \cite{CHES:GuiBorAra21} is incorrect, as acknowledged by the authors (see page 9 of \cite{CHES:GuiBorAra21}). 
%In particular, the algorithm cannot process more than a single loop, effectively reducing the algorithm to a single invocation of the multivalue bootstrapping algorithm of Carpov et al. \cite{RSA:CarIzaMol19}.  
%The problem is that a single invocation returns a set of $\RLWE$ encryptions of rotation polynomials that are supposed
%to be multiplied by the accumulator after the next blind rotation.
%As acknowledged in \cite{CHES:GuiBorAra21} that is not possible with Algorithm~6, but the algorithm could potentially
%be extended, for example, as in \cite{AC:CGGI17}, to return a $\RGSW$ after bootstrapping. 
%While implementations of such extensions are available (\cite{AC:CGGI17} claims these extentions are implemented in the TFHE library\footnote{\texttt{https://github.com/tfhe/tfhe}}) and are relatively efficient, Guimar\~aes et al. \cite{CHES:GuiBorAra21} claims these implementations are not efficient and refrain from implementing them.
%
%For the experiments, the authors build custom algorithms for each application (see Appendix~A in \cite{CHES:GuiBorAra21}).
%They show algorithms to compute 8-bit integer comparison, ReLU, max, and addition of two numbers.
%All implementations are applications of the multi-value bootstrap algorithm of Carpov et al. \cite{RSA:CarIzaMol19}, but the methods as specified and claimed to be main contributions, i.e., Algorithm~6 and the chain based method that is not formally specified, are not implemented. 
%
%Unfortunately, the lack of a correctness analysis, specification on how to choose the rotation polynomials, and the lack of an implementation of the main claimed contribution make it impossible to validate results reported in \cite{CHES:GuiBorAra21}. 
%To clarify, we do not count the applications in Appendix~A of \cite{CHES:GuiBorAra21} as the tree-based method since these applications do not follow Algorithm~6 to compute any function but instead show custom algorithms that use  Carpov et al. \cite{RSA:CarIzaMol19} bootstrapping.
% 

==> sections/performance-of-subroutines.tex <==
 At Table~\ref{tbl:prelim-cost} we summarize the cost of all algorithms that constitute
our bootstrapping algorithm.  
In general the formula for the amount of operations in our functional bootstrapping 
is given by
\begin{align*}
 \Bootstrap =~~ &\ell_{\boot} \cdot \big(\BlindRotate  + \SampleExtract \big) + \BuildAcc \\
 &+ \BlindRotate  + \SampleExtract  + \ModSwitch  + \KeySwitch.
\end{align*} 
It is crucial to note that the first $\ell_{\boot}$ blind rotations are over the ring $\R_{\deg, Q}$,
and then starting from the $\BuildAcc$ procedure we compute over the ring $\R_{\deg_{F}, Q}$.
$\SampleExtract$, $\KeySwitch$ $\ModSwitch$ perform operations in $\ZZ_Q$, and are cheap relatively to other operations. 
Therefore, at Table~\ref{tbl:bootstrap-cost} we summarize costs for operations
in $\R_{\deg, Q}$ and $\R_{\deg_{F}, Q}$. 
At Table~\ref{tbl:variance} we summarize the variance after bootstrapping according to Theorem~\ref{thm:correctness-of-functional-bootstrapping}.

\begin{table}[!htb]
	%\setlength{\tabcolsep}{7pt}
	\centering 
	\begin{tabular}{c | c | c | c}
		\hline
		Algorithm & $\add$ & $\mul$ & $\mul_{\mono}$ \\
		\hline
 $\extProd$ & $(n+1)^2 \cdot \ell$ &  $(n+1)^2 \cdot \ell$ & $0$ \\
 $\CMux$ &  $(n+1)^2 \cdot \ell  + 2(n+1)$ & $(n+1)^2 \cdot \ell$ & $0$ \\
 $\ModSwitch$ & $0$ & $0$ & $n+1$ \\
 $\SampleExtract$ & $0$ & $\deg \cdot \in \ZZ_q$ & $0$ \\
% $\KeySwitch$ & $n \cdot (n+1) \cdot \ell_{\keySwitchKey} \in \ZZ_q$ &  $n^2 \cdot \ell_{\keySwitchKey} \in \ZZ_q$ & $0$ \\
 $\KeySwitch$ & $(n'+ 1) \cdot n \cdot \ell_{\packKey} + 1$ & $0$  & $(n'+ 1) \cdot n \cdot \ell_{\packKey}$ \\
%  $\KeySwitch$ (Precomp.) & $(n'+ 1) \cdot n \cdot \ell_{\packKey} + 1$ & $0$ & $2$ \\
% $\PackLWEtoRLWE$ & $2 \cdot m \cdot n \cdot \ell_{\packKey} + 3 \cdot m$ & $0$ & $2 \cdot m \cdot n \cdot \ell_{\packKey}$ \\
 %$\PackLWEtoRLWE$ (Precomp.) & $2 \cdot m \cdot n \cdot \ell_{\packKey} + 3 \cdot m$ & $0$ & $2 \cdot m$ \\
 $\BlindRotate_{\TFHE}$ &  $4 \cdot n \cdot u \cdot (\ell_{\RGSW} + 1)$ & $4 \cdot n \cdot u  \cdot \ell_{\RGSW}$ & $2$ \\
 $\PubMux$ & $(2 + \ell) \cdot (n+1)$ & $\ell \cdot (n+1)$ & $0$ \\ 
 $\BuildAcc$ & $\ell \cdot (2 \cdot n \cdot \ell_{\packKey} + 3) + 4$ & $2 \cdot \ell$ & $ 2 \cdot \ell \cdot n \cdot \ell_{\packKey}$ \\
 $\BuildAcc$ (Precomp.) & $\ell \cdot (2 \cdot n \cdot \ell_{\packKey} + 3) + 4$ & $2 \cdot \ell$ & $2 \cdot \ell_{\packKey}$ \\ 
 \hline
\end{tabular}  
\caption{Complexity of individual algorithms. Note that the notation for the variables is the same as in the respective algorithm description.}\label{tbl:prelim-cost}
\end{table}




\begin{table}[!htb]
	%\setlength{\tabcolsep}{7pt}
	\centering 
	\label{tbl:bootstrap-cost}
	\begin{tabular}{c | c }
		\hline 
   Type & Complexity \\
   \hline
 $\add$ &  $\ell_{\boot} \cdot (2 \cdot \deg \cdot \ell_{\packKey} + 3) + 4 + 4 \cdot n \cdot u \cdot (\ell_{\RGSW, F} + 1)$  \\  
 		& $+ \ell_{\boot} \cdot  4 \cdot n \cdot u \cdot (\ell_{\RGSW} + 1)$ \\
 $\mul$ &  $2 \cdot \ell_{\boot} +   4 \cdot n \cdot u  \cdot \ell_{\RGSW, F} + \ell_{\boot} \cdot 4 \cdot n \cdot u  \cdot \ell_{\RGSW}$  \\  
  $\mul_{\mono}$ & $2 \cdot \ell_{\boot} \cdot \deg \cdot \ell_{\packKey} + 2 + 2 \cdot \ell_{\boot}$ \\
%   $\mul_{\mono}$ (Precomp) & $2 \cdot \ell_{\packKey} + 2$   \\ 
   \hline
\end{tabular}  
\caption{Complexity of the bootstrapping algorithm.}
\end{table}



In this section we estimate the theoretical performance, choose the parameters, 
estimate the correctness error and security.

To estimate the theoretical performance we calculate the amount of additions and multiplication of ring elements,
and multiplications of ring elements by a monomial.
We denote these operations with $\add$, $\mul$ and $\mul_{\mono}$ respectively.




\begin{table}%[!htb]
	%\setlength{\tabcolsep}{7pt}
	\centering 
	\label{tbl:variance}
	\begin{tabular}{c | c }
		\hline
		Bound & Error \\
		\hline 
		$\bound_{\deg}$ & $(\frac{2 \deg}{q})^{2} \cdot \bound_{\out}  + \frac{2}{3} + \frac{2}{3} \cdot \hamming(\vec{s}) \cdot (\norm{\Var(\vec{s})}_{\infty} + \norm{\E(\vec{s})}_{\infty})$ \\ 
	$\bound_{\out}$	& $ (\frac{q^2}{Q^2}) \cdot (\bound_{F} + \bound_{\BR} + \bound_{KS}) + \frac{2}{3} + \frac{2}{3} \cdot \hamming(\vec{s}_F) \cdot (\norm{\Var(\vec{s}_{F})}_{\infty} + \norm{\E(\vec{s}_{F})}_{\infty})$   \\
	$\bound_{F}$  &  $(\frac{7}{12}) \cdot \deg_{F} \cdot \ell_{\boot} \cdot  \basis_{\boot}^2  \cdot \big(\bound_{\BR} +  \bound_{P}\big)$  \\ 
	$\bound_{P}$ & $(\frac{7}{12}) \cdot \deg \cdot \ell_{\packKey} \cdot \basis_{\packKey}^2 \cdot \bound_{\packKey}$ \\
	%$\bound_{P}$ (Precomp.) & $ \deg \cdot \ell_{\packKey} \cdot \bound_{\packKey}$  \\
	$\bound_{\BR}$ & $(\frac{7}{6}) \cdot n \cdot u \cdot  \deg \cdot \ell_{\RGSW} \cdot \basis_{\RGSW}^2 \cdot \bound_{\brKey}$ \\ 
	$\bound_{KS}$  & $(\frac{7}{12}) \cdot \deg \cdot \ell_{\keySwitchKey} \cdot \basis_{\keySwitchKey}^2 \cdot \bound_{\keySwitchKey}$ \\
	\hline
\end{tabular} 
	\caption{Variance on the error for different parts of the bootstrapping procedure.}
\end{table}
 
  
  
  


\begin{table}[!htb]
	%\setlength{\tabcolsep}{7pt}
	\centering 
	\begin{tabular}{c | c | c | c}
		\hline
		Parameter Set &  $\add$ & $\mul$ &  $\mul_{\mono}$  \\ 
		\hline  
Set 1  &  835588  & 270344  & 524298 (18)  \\ 
Set 2  &  614404  & 245768 & 327690  (20)  \\ 
Set 3  &  450564  & 245768 & 163850 (20)  \\ 
\hline
\end{tabular} 
 \caption{Complexity for the parameter sets. The key and ciphertext column contain the size of the bootstrapping keys and ciphertexts. The public key includes $\brKey$ as well as the key switching keys  $\packKey$ and $\keySwitchKey$. The last column contain the amount a monomial multiplications for precomputed keys.}\label{tbl:parameter-sets-cost}
\end{table}  
  
  


==> sections/pk-mm.tex <==
Using the packing key construction presented earlier, the LWE to RLWE transform as a matrix multiplication. Using the packing key $\packKey$ 
we construct a matrix $M_{\packKey} \in \ZZ_Q^{2\cdot N \times N \cdot \ell{\packKey}}$ where $M_{\packKey}[*,i \cdot \basis_{\packKey} + j] = \coefs(\packKey[i,j,2])$. To transform a LWE sample $c = [\vec{a},b]  \in  \LWE_{\bound_{\ct}, \deg, Q}(\msg)$ into $c' = [a',b'] \in \RLWE_{\bound_{\brKey}, \deg, Q}(\msg)$ we create a vector $v \in \ZZ^{N \cdot \ell_{\packKey}}_Q$ with:
\begin{equation}\label{eqn:decvec}
	v[i \cdot \ell_{\packKey} + j] = \coefs({\Decomp_{\basis_{\packKey}, Q}}(\vec{a})_j)[i]
\end{equation}
 In other words, we decompose each coefficient of $\vec{a}$ with regards to $\basis_{\packKey}$ and concatenate all digits.
To calculate $c'$ we finally compute
\begin{equation}
	v' = \left[ 0^\deg | b | 0^{\deg-1} \right]^T - M_{\packKey} \cdot v
\end{equation}
and interpret $v'[0:\deg-1]$ as the coefficients of $a'$ and $v'[\deg:2\deg-1]$ as the coefficients of $b'$.
This can be arbitrarily extended to multiple vectors. As an intermediate step, $\PackLWEtoRLWE$ computes up to $\frac{N}{2}$ transformations.
This can still be achieved using a single matrix multiplication. 

To transform $k$ samples, let $c_i$, be the $i$-th $\LWE$ sample to be processed and 
$v_i$ be the corresponding decomposed vector as in Equation~\ref{eqn:decvec}. We denote by $V$ the $N\cdot\ell_{\packKey} \times k$ matrix whose columns are composed of all $v_i$'s. We compute:
\begin{equation}
	V' = [0^N|b_0,...,b_{k-1}|0^{N-k}]^T - M_{\packKey} \cdot V
\end{equation}
The columns of $V'$ constitute the coefficients of the transformed samples.

==> sections/post-rotation-bootstrapping.tex <==
 
 
 
 
 
\subsection{Post-Rotation Bootstrapping Algorithm.}
 
Here we describe the post-rotation bootstrapping algorithm.
 Similarly, as in the previous section, we will actually use both pre- and post-rotation polynomials.
 At a high level the algorithm follows the same principles as the algorithm from Def. \ref{def:pre-rotation-bootstrapping},
however we will compute all the powers of $\basis_{\boot}$ using the blind rotation.
Then having the powers of $\basis_{\boot}$, we can multiply it with a $\basis_{\boot}$ decomposition of the
post rotation polynomial.

 \begin{definition}[Post-Rotation Bootstrapping]
The bootstrapping procedure is defined as follows:
\begin{description}
\item[$\BootstrapPostRot(\brKey, \vec{u}, \ct, \preRotPoly, \postRotPolyList, \basis_{\boot}, \packKey, \keySwitchKey):$]
Takes as input a bootstrapping key $\brKey = \RGSW_{\errDist_{\brKey}, \deg, Q, \basis_{\brKey}}(\fr{s}, .)^{n \times u}$, 
a vector $\vec{u} \in \ZZ^{u}$,
a LWE sample $\ct = \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)(\msg) = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$, 
a polynomial  $\preRotPoly \in \R_Q$ and a list of polynomials $\postRotPolyList \in \R_Q^{m}$, 
a packing key $\packKey \in \RLWE_{\errDist_{\packKey}, \deg, Q}(\fr{s}, .)^{\deg \times \ell_{\packKey} \times \basis_{\packKey}}$, and a keyswitch key $\keySwitchKey \in \LWE_{\errDist_{\keySwitchKey}, n, q}(\vec{s}, .)^{\deg \times \ell_{\keySwitchKey} \times \ell_{\keySwitchKey}}$.
\begin{enumerate}
\item Cyclic shift the coefficients of $\preRotPoly$ by $b$ positions, resulting in $\preRotPoly_b \in \R_Q$.
\item Let $\ell_{\boot} = \roundUp{\log_{\basis_{\boot}}{Q}}$
\item For $i=1$ to $\ell_{\boot}$ do, 
\begin{enumerate} 
\item  Set $\acc_i \exec \RLWE_{\errDist_{\acc}, \deg, Q}(\fr{s}, 0) + [2^{i-1} \cdot \preRotPoly_b, 0]^{\top}$.  
\item  Run $\acc_{\BR, i} \exec \BlindRotate(\acc_i, \bootstrapKey, \ct)$.   
\end{enumerate}
\item For $i=1$ to $m$ do,
\begin{enumerate}
\item Compute $\vec{d}_{i} \exec \Decomp_{\basis_{\boot}, Q}(\postRotPoly[i])$.
\item Compute $\vec{c}_i \exec \sum_{j=1}^{\ell_{\boot}} \acc_{\BR, j} \cdot \vec{d}_i[j]$.
\item Run $\vec{c}_{Q, i} \exec \SampleExtract(\fr{c}_i, 1)$.
\item Run $\vec{c}_{q, i} \exec \ModSwitch(\vec{c}_{Q, i}, Q, q)$.
\item Run $\ct_{\out, i} \exec \KeySwitch(\vec{c}_{q, i}, \keySwitchKey)$.
\end{enumerate} 
\item Return $\ct_{\out} \exec [\ct_{\out, i}]_{i=1}^m$.  
\end{enumerate}
\end{description}
\end{definition}
 
 
 
\begin{theorem}[Correctness of the Post-Rotation Bootstrapping]
\label{thm:bootstrapping-post-rotation}
Let  $\vec{u} \in \ZZ^u$ be a vector 
 that for all $y \in \ZZ_q$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod q$.
 Let $\ct = \LWE_{\errDist_{\ct}, n, q}(\vec{s}, .)(\msg) = [b, \vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$.
 Let $\deg, Q \in \NN$ and $\basis_{\RGSW}, \basis_{\brKey}, \basis_{\packKey}, \basis_{\keySwitchKey} \in \NN$.
 Let
 and $\fr{s} \in \skDist$ and $\vec{s}_{\fr{s}} \exec \KeyExtract(\fr{s})$.
 Let $\errDist_{\bound_{\brKey}}$, $\errDist_{\bound_{\packKey}}$ and $\errDist_{\bound_{\keySwitchKey}}$,
 be respectively $\bound_{\brKey}$, $\bound_{\packKey}$ and $\bound_{\keySwitchKey}$-Bounded distributions.
  Let
 $\brKey \exec \BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \errDist_{\bound_{\brKey}}, \deg, Q, \basis_{\RGSW}, \fr{s})$, 
 $\packKey \exec \PackSetup(\errDist_{\bound_{\packKey}}, \deg, \deg, q, \vec{s}_{\fr{s}}, \fr{s}, \basis_{\packKey})$, 
 and  $\keySwitchKey \exec \KeySwitchSetup(\errDist_{\bound_{\keySwitchKey}}, \deg, \deg, q, \vec{s}_{\fr{s}}, \vec{s}, \basis_{\keySwitchKey})$.
 Finally, let $\preRotPoly \in \R_Q$ and $\postRotPolyList \in \R_Q^{m}$ be two polynomials.
 
 If $\ct_{\out} \exec \BootstrapPreRot(\brKey, \vec{u}, \ct, \preRotPoly, \postRotPoly, \packKey, \keySwitchKey)$, then
 for $i \in [m]$ we have
 $\ct_{\out}[m] \in \LWE_{\errDist_{\bound}, \deg, q}(\vec{s}, \msg_{\out, i})$, 
where
 $\msg_{\out, i} = (\frac{q}{t}) \cdot \msg_{F, i}$ and 
 $\msg_{F, i} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)) \cdot \postRotPolyList[i])[1]$ for $Q = q = 0 \mod t$,   
 and $\errDist_{\bound}$ is a $\bound$-Bounded distribution with
 \begin{align*} 
\bound \leq (\frac{q}{Q}) \cdot \sqrt{\deg} \cdot  \bound_{\BR} \cdot \postRotPoly  + \skDist + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1),
\end{align*}
where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$
and  
 $\bound_{\BR}$ is the bound on RLWE accumulator after blind rotation according to lemma \ref{lemma:correctness-shift-based-blind-rotate}.
 Furthermore, we have that
 if $\bound \leq \frac{q}{2 \cdot t}$, then
 $\round{\Phase(\ct_{\out, i})}_t^q = \msg_{F, i}$.
\end{theorem}
 
 
  

\begin{proof}[of theorem \ref{thm:bootstrapping-post-rotation} - Correctness of the Post-Rotation Bootstrapping] 
The correctness of the bootstrapping follows from the correctness of the underlying algorithms.
In particular, on the beginning we set the accumulator $\acc$ to the $\preRotPoly$ shifted by $b$.
From correctness of blind rotation for $i \in [\ell_{\boot}]$ we have
$\acc_{\BR, i} \in \RLWE_{\bound_{\BR}}(\fr{s}, \msg_{\BR} \cdot 2^{i-1})$, where
$\msg_{\BR} = \Shift(\preRotPoly, \Phase(\ct)) \in \R_Q$
and $\errDist_{\bound_{\BR}}$ is a $\bound_{\BR}$-Bounded distribution
where the bound is given by lemma \ref{lemma:correctness-shift-based-blind-rotate}
Then for $i \in [m]$ we compute
$\vec{d}_i \exec \Decomp_{\basis_{\boot}, Q}(\postRotPoly[i])$, and
 $\vec{c}_i \exec \sum_{j=1}^{\ell_{\boot}} \acc_{\BR, j} \cdot \vec{d}_i[j]$,
so so we have  that
\begin{align*}
\vec{c}_i &= \sum_{j=1}^{\ell_{\boot}} \acc_{\BR, j} \cdot \vec{d}_i[j] \\
	&= \sum_{j=1}^{\ell_{\boot}} \RLWE_{\errDist_{\bound_{\BR}}, \deg, Q}(\fr{s}, \msg_{\BR} \cdot 2^{i-1}) \cdot \vec{d}_i[j] \\
	&= \RLWE_{\errDist_{\bound_{\vec{c}}}, \deg, Q}(\fr{s}, \msg_{\BR} \sum_{j=1}^{\ell_{\boot}} \vec{d}_i[j] \cdot 2^{i-1}) \\
	&= \RLWE_{\errDist_{\bound_{\vec{c}}}, \deg, Q}(\fr{s}, \msg_{\BR} \cdot \postRotPoly[i]) \\
	&= \RLWE_{\errDist_{\bound_{\vec{c}}}, \deg, Q}(\fr{s}, \msg_{\vec{c}_i})
\end{align*}
where
$\errDist_{\bound_{\vec{c}}}$ is a $\bound_{\vec{c}}$-Bonded distribution with 
$\bound_{\vec{c}} \leq \expFact_{\R_Q} \cdot  \bound_{\BR} \cdot (\basis_{\boot} - 1) \cdot \ell_{\boot} 
\leq \sqrt{\deg} \cdot  \bound_{\BR} \cdot (\basis_{\boot} - 1) \cdot \ell_{\boot}$.
Then from correctness of sample extract we have that $\vec{c}_{Q, i} \in \LWE_{\errDist_{\bound_{\vec{c}}}, \deg, Q}(\vec{s}_{\fr{s}}, \msg_{\vec{c}_{Q, i}})$, where $\msg_{\vec{c}_{Q, i}} = \coefs(\msg_{\vec{c}_i})[1]$.
From correctness of modulus switching we have that 
$\vec{c}_{q, i} \in \LWE_{\errDist_{\bound_{\vec{c}_q}}, \deg, q}(\vec{s}_{\fr{s}}, (\frac{q}{Q}) \cdot \msg_{\vec{c}_{Q, i}})$,
where $\errDist_{\bound_{\vec{c}_q}}$ is a $\bound_{\vec{c}_q}$-Bounded distribution
with $\bound_{\vec{c}_q} \leq (\frac{q}{Q}) \cdot  \sqrt{\deg} \cdot  \bound_{\BR} \cdot (\basis_{\boot} - 1) \cdot \ell_{\boot} + \bound_{\skDist}$.
Finally from correctness of key switching
we have that $\ct_{\out, i} \in \LWE_{\errDist_{\bound}, \deg, q}(\vec{s}, \msg_{\out, i})$,
where
$\msg_{\out, i} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_{Q, i}}$ and
 $\errDist_{\bound}$ is a $\bound$-Bounded distribution
with 
\begin{align*}
\bound &\leq \bound_{\vec{c}_q} + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1) \\
 &\leq (\frac{q}{Q}) \cdot  \sqrt{\deg} \cdot  \bound_{\BR} \cdot (\basis_{\boot} - 1) \cdot \ell_{\boot} + \bound_{\skDist} + \deg \cdot \ell_{\keySwitchKey} \cdot \bound_{\keySwitchKey} \cdot (\basis_{\keySwitchKey}-1),
\end{align*}
where 
$\ell_{\keySwitchKey} = \roundUp{\log_{\basis_{\keySwitchKey}}{q}}$. 

Finally, denote $\msg_{\vec{c}_{Q, i}} = (\frac{Q}{t}) \cdot \msg_{F, i}$, so that $\msg_{F, i} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)) \cdot \postRotPolyList[i])[1]$.
Then we have 
$\msg_{\out, i} = (\frac{q}{Q}) \cdot \msg_{\vec{c}_{Q, i}} = (\frac{q}{Q}) \cdot  (\frac{Q}{t}) \cdot \msg_{F, i} = (\frac{q}{t}) \cdot \msg_{F, i}$.
What follows is that if $\bound \leq \frac{q}{2\cdot t}$, then 
$\round{\Phase(\ct_{\out, i})}_t^q = \msg_{F, i} = (\frac{t}{Q}) \cdot \coefs(\Shift(\preRotPoly, \Phase(\ct)) \cdot \postRotPolyList[i])[1]$.
\end{proof}

 

==> sections/tfhe-blind-rotate.tex <==
 
 
 Below we recall the blind rotation introduced by Chillotti et al. \cite{AC:CGGI16}.
 Let  $\vec{u} \in \ZZ^u$ be a vector 
 that for all $y \in \ZZ_{2 \cdot \deg}$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod 2 \cdot \deg$.

\begin{definition}[TFHE Blind Rotation]
Blind rotation consists of a key generation algorithm $\BRKeyGen_{\TFHE}$,
and blind rotation algorithm $\BlindRotate_{\TFHE}$.

\begin{itemize}

\item $\BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \bound_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s}):$ 
Takes as input a dimension $n$, a secret key $\vec{s} \in \ZZ_t^{n \times 1}$ and a vector $\vec{u} \in \ZZ^{u}$, an bound $\bound_{\brKey}$,
 a degree $\deg$ and a modulus $Q$ defining the ring $\R_{\deg, Q}$, 
 a basis $\basis_{\RGSW} \in \NN$, and a secret key $\fr{s} \in \R_{\deg, Q}$.
The algorithm outputs a blind rotation key $\brKey$.
%TODO Commented and put into appendix
%\begin{enumerate}
%\item  Set a matrix $\ma{Y} \in \BB^{n \times u}$ as follows:  
%\begin{enumerate}
%\item For $i \in [n]$ set the $i$-th row of $\ma{Y}$, to satisfy 
%$\vec{s}[i] = \sum_{j=1}^{u} \ma{Y}[i, j] \cdot \vec{u}[j]$, 
%\end{enumerate} 
%\item For $i \in [n]$, $j \in [u]$ set $\brKey[i,j] = \RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, \ma{Y}[i,j])$. 
%\item Output  $\brKey$. 
%\end{enumerate}

\item $\BlindRotate_{\TFHE}(\brKey, \acc, \ct, \vec{u}):$ 
Takes as input a blind rotation key $\brKey$ $=$ $\RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\RGSW}}(\fr{s}, .)^{n \times u}$,  
  an accumulator $\acc \in \RLWE_{\bound_{\acc}, \deg, Q}(\fr{s}, .)$, 
 a ciphertext $\ct \in  \LWE_{\bound_{\ct}, n, 2\cdot \deg}(\vec{s}, .)$, where $\vec{s} \in \ZZ_t^{n}$ with $t \leq 2 \cdot \deg$, and a vector $\vec{u} \in \ZZ^{u}$. The algorithm outputs $\acc_{\out}$.
 %TODO Commented and put into appendix
%\begin{enumerate}
%\item $\vec{c} \exec \ModSwitch(\ct, q, 2 \cdot \deg)$.
%\item Let $\vec{c} = [b, \vec{a}^{\top}]^{\top} \in \ZZ_{2 \cdot \deg}^{(n+1) \times 1}$. 
%\item For $i \in [n]$ do: 
%\begin{enumerate}
%\item  For $j \in [u]$ do:
% \begin{align*}
% \acc \exec \CMux(\brKey[i, j], \acc \cdot X^{-\vec{a}[i] \cdot \vec{u}[j]}, \acc)
%\end{align*}   
%\end{enumerate} 
%\item Output $\acc$.  
%\end{enumerate} 
\end{itemize} 
\end{definition}
 
 
 
\begin{lemma}[Correctness of TFHE-Style Blind-Rotation]
\label{lemma:correctness-tfhe-blind-rotate} 
 Let   $\ct$ $\in$ $\LWE_{\bound_{\ct}, n, 2 \cdot \deg}(\vec{s}$, $.)$ be a LWE sample and denote $\ct$ $=$ $[b$, $\vec{a}^{\top}]^{\top} \in \ZZ_{2 \cdot \deg}^{(n+1) \times 1}$.
%Let $\deg$ $\in$ $\NN$ be the degree and $Q$ $\in$ $\NN$ be the modulus defining the ring $\R_{\deg, Q}$.
%Furthermore, let $\fr{s}$ $\in$ $\R_{\deg, Q}$,  $\basis_{\RGSW}$ $\in$ $\NN$,  $\bound_{\brKey}$ $\le$ $Q$  
Let $\acc$ $\in$ $\RLWE_{\bound_{\acc}, \deg, Q}(\fr{s}$, $\msg_{\acc})$. 
If $\brKey \exec \BRKeyGen_{\TFHE}(n, \vec{s}, \vec{u}, \bound_{\brKey}, \deg, Q, \basis_{\RGSW}, \fr{s})$
and $\acc_{\out}$ $\exec$ $\BlindRotate_{\TFHE}(\brKey$, $\acc$, $\ct$, $\vec{u})$,
then $\acc_{\out}$ $\in$ $\RLWE_{\bound_{\out}, \deg, Q}(\fr{s}$, $\msg_{\acc}^{\out})$,
where $\msg_{\acc}^{\out}$ $=$ $\msg_{\acc}$ $\cdot$ $X^{b - \vec{a}^{\top} \cdot \vec{s} \mod 2 \cdot \deg}$ $\in$ $\R_{\deg, Q}$ and  
\begin{align*} 
\bound_{\out}  \leq  \bound_{\acc} +  (\frac{2}{3}) \cdot  n \cdot u \cdot \deg \cdot \ell_{\RGSW} \cdot \basis_{\RGSW}^2 \cdot \bound_{\brKey}
\end{align*} 
\end{lemma}



 \begin{definition}[Bootstrapping]\label{def:tfhe-bootstrapping}
The bootstrapping procedure is as follows:
\begin{itemize}
\item $\Bootstrap(\brKey,  \vec{u}, \ct, \preRotPoly, \keySwitchKey):$
Takes as input a blind rotation key $\brKey$ $=$  $\RGSW_{\bound_{\brKey}, \deg, Q, \basis_{\brKey}}(\fr{s}$, $.)^{n \times u}$, 
a vector $\vec{u} \in \ZZ^{u}$,
a LWE sample $\ct$ $=$ $\LWE_{\bound_{\ct}, n, q}(\vec{s}$, $.)$ $=$ $[b$, $\vec{a}^{\top}]^{\top} \in \ZZ_q^{(n+1) \times 1}$, 
a polynomial  $\preRotPoly \in \R_{\deg, Q}$, and a LWE to LWE key switching key $\keySwitchKey$.
the algorithm outputs $\ct_{\out}$.
 %TODO Commented and put into appendix
%\begin{enumerate} 
%
%\item Set $b_{\deg} \exec \lfloor \frac{2\cdot\deg \cdot b}{q} \rceil$
%  
%\item Set $\preRotPoly' \exec \preRotPoly \cdot X^{b_{\deg}} \in \R_{\deg, Q}$.
%
%\item Run $\acc_{F} \exec [\preRotPoly', 0]^{\top}$
%
%\item Run $\acc_{\BR, F} \exec \BlindRotate( \brKey, \acc_{F}, \ct, \vec{u})$.   
%
%\item Run $\vec{c}_{Q} \exec \SampleExtract(\acc_{\BR, F}, 1)$.
%   
%\item Run $\vec{c}_{Q, \keySwitchKey} \exec \KeySwitch(\vec{c}_{Q}, \keySwitchKey)$.
% 
%\item Run $\ct_{\out} \exec \ModSwitch(\vec{c}_{Q, \keySwitchKey}, Q, q)$.
%
%\item Return $\ct_{\out}$.  
%\end{enumerate}
\end{itemize}
\end{definition}
  
   
  \begin{theorem}[Correctness of TFHE-Style Bootstrapping]
\label{thm:correctness-tfhe-bootstrapping}
%Let  $\vec{u} \in \ZZ^u$ be a vector 
% that for all $y \in \ZZ_q$ there exists $\vec{x} \in \BB^u$ such that $y = \sum_{i=1}^u \vec{x}[i] \cdot \vec{u}[i] \mod q$.
 Let   $\ct \in \LWE_{\bound_{\ct}, n, q}(\vec{s}, \Delta_{q, t} \cdot \msg)$.
%Let $\deg \in \NN$ be the degree and $Q \in \NN$ be the modulus defining the ring $\R_{\deg, Q}$.
%Furthermore, let $\fr{s} \in \R_{\deg, Q}$,  $\basis_{\RGSW} \in \NN$, and  $\bound_{\brKey} \le Q$.
Let $\brKey$ $\exec$ $\BRKeyGen_{\TFHE}(n$, $\vec{s}$, $\vec{u}$, $\bound_{\brKey}$, $\deg$, $Q$, $\basis_{\RGSW}$, $\fr{s})$,
$\vec{s}_{F} \exec \KeyExtract(\fr{s})$, 
and
$\keySwitchKey$ $\exec$ $\KeySwitchSetup(\bound_{\keySwitchKey}$, $\deg$, $n$, $q$, $\vec{s}_{F}$, $\vec{s}$, $\basis_{\keySwitchKey})$.
%, where  $\basis_{\keySwitchKey} \in \NN$ and $\bound_{\keySwitchKey} \le q$.
Let $\ct_{\deg} \exec \ModSwitch(\ct, q, 2 \cdot \deg) \in \LWE_{\bound_{\deg}, n, 2 \cdot \deg}(\vec{s}, \Delta_{2 \cdot \deg, t} \cdot \msg)$.
Let $\tilde{\msg} \exec \Phase(\ct_{\deg})$, $\msg = \round{\tilde{\msg}}_{t}^{2 \cdot \deg}$ and
 $\preRotPoly \in \R_{\deg, Q}$ be such that if $\tilde{\msg} \in [0,\deg)$, then
 $\coefs(X^{\tilde{\msg}} \cdot \preRotPoly)[1] = \Delta_{Q, t} \cdot F(\msg)$, where $F:\ZZ_t \mapsto \ZZ_t$.
If $\ct_{\out} \exec \Bootstrap(\brKey,  \vec{u}, \ct, \preRotPoly, \keySwitchKey)$
and $\msg \leq \frac{t}{2} - 1$,
then $\ct_{\out} \in \RLWE_{\bound_{\out}, \deg, q}(\vec{s}, \msg_{\out})$,
where $\msg_{\out} = \Delta_{Q, t} \cdot F(\msg)$ and  
\begin{align*}
\bound_{\out} \leq& (\frac{q^2}{Q^2}) \cdot  (\bound_{\BR} + \bound_{KS}) \\
 &+ \frac{2}{3} + \frac{2}{3} \cdot \hamming(\vec{s}_{F}) \cdot  (\norm{\Var(\vec{s}_{F})}_{\infty} + \norm{\E(\vec{s}_{F})}_{\infty}^2), 
\end{align*}
where  $\bound_{\BR} \leq (\frac{2}{3}) \cdot  n \cdot u \cdot \deg \cdot \ell_{\RGSW} \cdot \basis_{\RGSW}^2 \cdot \bound_{\brKey}$
and $\bound_{KS} \leq  (\frac{1}{3}) \cdot \deg \cdot \ell_{\keySwitchKey} \cdot \basis_{\keySwitchKey}^2 \cdot  \bound_{\keySwitchKey}$.
If $Q = q$, then $\bound_{\out} \leq \bound_{\BR} + \bound_{KS}$.
%\begin{align*}
%\bound_{\BR} \leq (\frac{7}{6}) \cdot  n \cdot u \cdot \deg \cdot \ell_{\RGSW} \cdot \basis_{\RGSW}^2 \cdot \bound_{\brKey}, \text{ and} \\
%\bound_{KS} \leq  (\frac{7}{12}) \cdot \deg \cdot \ell_{\keySwitchKey} \cdot \basis_{\keySwitchKey}^2 \cdot  \bound_{\keySwitchKey}.
%\end{align*}
Finally we have,
\begin{align*}
\bound_{\deg} \leq& (\frac{2 \cdot \deg}{q})^2 \cdot \bound_{\ct} \\
 &+ \frac{2}{3}  + \frac{2}{3} + \hamming(\vec{s}) \cdot (\norm{\Var(\vec{s})}_{\infty} + \norm{\E(\vec{s})}_{\infty}^2)
\end{align*} 
if $\deg \neq 2 \cdot q$, and $\bound_{\deg} = \bound_{\ct}$ otherwise, where
$\bound_{\ct} = \max(\bound_{\fresh}, \bound_{\out})$ and $\bound_{\fresh}$ is the bound in the error variance
of a fresh ciphertext.
\end{theorem}

